AndesVL Technical Report: An Efficient Mobile-side Multimodal Large Language Model

In recent years, while cloud-based MLLMs such as QwenVL, InternVL, GPT-4o, Gemini, and Claude Sonnet have demonstrated outstanding performance with enormous model sizes reaching hundreds of billions of parameters, they significantly surpass the limitations in memory, power consumption, and computing capacity of edge devices such as mobile phones. This paper introduces AndesVL, a suite of mobile-side MLLMs with 0.6B to 4B parameters based on Qwen3's LLM and various visual encoders. We comprehensively outline the model architectures, training pipeline, and training data of AndesVL, which achieves first-tier performance across a wide range of open-source benchmarks, including fields such as text-rich image understanding, reasoning and math, multi-image comprehension, general VQA, hallucination mitigation, multilingual understanding, and GUI-related tasks when compared with state-of-the-art models of a similar scale. Furthermore, we introduce a 1+N LoRA architecture alongside a Quantization-Aware LoRA Fine-Tuning (QALFT) framework to facilitate efficient task adaptation and model compression during mobile-side deployment of AndesVL. Moreover, utilizing our cache eviction algorithm -- OKV -- along with customized speculative decoding and compression strategies, we achieve a 6.7x peak decoding speedup ratio, up to 30.9% memory reduction, and 1.8 bits-per-weight when deploying AndesVL-4B on MediaTek Dimensity 9500 chips. We release all models on https://huggingface.co/OPPOer.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> section/experiments/benchmark/visual_grounding_benchmark.tex <==
\subsection{Visual Grounding}
\subsubsection{Benchmarks}
To evaluate the visual grounding and reference capability of AndesVL, we assess it on referring expression comprehension (REC) tasks on the RefCOCO, RefCOCO+, and RefCOCOg datasets, where the model identifies target objects in images from given descriptions.

\textbf{RefCOCO}~\cite{kazemzadeh2014referitgame}: RefCOCO consists of 19,994 images from COCO with 142,210 referring expressions for 50,000 objects. Its test A is people-focused, and test B is for other objects on REC tasks. 

\textbf{RefCOCO+}~\cite{kazemzadeh2014referitgame}: RefCOCO+ emphasizes attribute-based descriptions without absolute location cues, in contrast to RefCOCO. It contains 19,992 images and 141,564 expressions as descriptive attributes.

\textbf{RefCOCOg}~\cite{mao2016generation}: RefCOCOg has more complex and longer descriptive attributions for objects and requires models to handle intricate REC tasks. It contains 25,799 images and 95,010 expressions.

==> section/experiments/experiment_results/UI_understanding_experiment.tex <==
\begin{table}[tb]
    \centering
    \begin{tabular}{c|c|c|c|c|c|c|c}
        \toprule
        Model &  MMMU&  MathVista&    OCRBench& AI2D& BLINK& POPE&RealworldQA\\
        \midrule
        AndesVL-4B         & 54.7& 71.0& 81.6& 82.0& 53.2& 88.9&67.6\\
        AndesVL-4B-UI      & 51.9& 68.8& 79.8& 79.8& 51.3& 87.9&64.8\\
        \hline
        AndesVL-2B         & 46.7& 61.4& 78.4& 75.9& 46.0& 88.3&63.9\\
        AndesVL-2B-UI      & 45.3& 62.2& 77.0& 75.3& 43.7& 87.3&62.0\\
        \hline
        AndesVL-0.6B       & 40.1& 47.9& 70.3& 66.3& 41.6& 83.9&54.8\\
        AndesVL-0.6B-UI    & 39.3& 52.0& 67.6& 66.0& 40.2& 85.1&54.5\\ 
        \bottomrule
    \end{tabular}
    \caption{Comparison of AndesVL-UI and AndesVL on different general benchmarks}
    \label{tab:ablation_}
\end{table}

==> section/experiments/experiment_results/baselines.tex <==
\subsection{Results}

\subsubsection{Baselines}

==> section/experiments/experiment_results/overall_benchmark_results.tex <==
\subsubsection{Evaluation Results}

\begin{table}
    \small
    \centering
    \begin{tabular}{l|ccccccccc}
        \hline
         Model & MMMU & MathVista & AI2D & HallBench  & OCRBench & MMStar & MMVet & MMBv1.1 & Overall\\
         \hline
         AndesVL-4B  & \textbf{55.4} & \textbf{70.2}  & 80.6 & \textbf{50.3} & 80.1 & 60.7 & 56.4 & 75.7 & \textbf{66.2} \\
         Qwen2.5-VL-3B ~\cite{bai2025qwen2_5}  & 51.2 & 60.9 & 81.4 & 46.6 & 82.6 & 56.3 & 60 & 76.8 & 64.5\\
         InternVL2.5-4B ~\cite{chen2024expanding}  & 51.8 & 60.8 & 81.4 & 46.6 & 82 & 58.6 & 61.5 & 78.2 & 65.1 \\
         Gemma3-4B ~\cite{gemmateam2025gemma3}  &  47.3 & 46.3 & 70.7 & 40.8 & 66 & 47.9 & 57.8 & 66.4 & 55.4\\
         Phi-3.5-Vision ~\cite{abdin2024phi3}  & 44.6 & 43.3 & 77.8 & 40.5 & 59.9 & 47.5 & 43.2 & 67.4 & 53\\
         MM1.5-3B ~\cite{zhang2024mm1_5}  & 37.1 & 44.4 & 65.7 & - & 65.7 & - & 41 & - & - \\
         BlueLM-V-3B ~\cite{lu2024bluelm}  & 45.1 & 60.9 & \textbf{85.3} & 48 & \textbf{82.9} & \textbf{62.3} & \textbf{61.8} & \textbf{82.7} & 66.1\\
         \hline
         AndesVL-2B  & 47.2 & 54.9 & 75.6 & 45.4 & 79 & 50.6 & 43.8 & 71.9 & 58.5 \\
         Qwen2-VL-2B ~\cite{wang2024qwen2vl}  & 42.2 & 48 & 74.7 & 42.4 & 79.7 & 47.5 & 51.5 & 42.2 & 57.3  \\
         InternVL2.5-2B ~\cite{chen2024expanding}  & 43.2 & 51.1 & 74.9 &  42.6 & 80.2 & 53.7 & 62.6 & 70.9 & 59.9 \\
         InternVL3-2B ~\cite{zhu2025internvl3}  & 48.6 & 57 & 78.7 & 42.5 & 83.5 & 60.7 & 64.6 & 78 & 64.2 \\
         Ovis2-2B ~\cite{lu2024ovis}  & 45.6 & 64.1 & 82.7 & 50.2 & 87.3 & 56.7 & 58.3 & 76.9 & 65.2 \\
         SAIL-VL-1.5-2B  ~\cite{dong2025scalable}  & 46.7 & 67.3 & 83.7 & 49.8 & 88.5 & 62.8 & 61.4 & 78.4 & 67.3 \\
         MiniCPM-V-2B ~\cite{yao2024minicpm}  & 38.2 & 39.8 & 62.9 & 36.1 & 60.5 & 39.1 & 41 & 65.7 & 47.9 \\
         \hline
         AndesVL-1B  & 41.3 & 47.2  & 68 & 35.2 & 76.4 & 46.6 & 36.7 & 65.1 & 52.4\\
         InternVL2.5-1B ~\cite{chen2024expanding}  & 47.1 & 60.9 & 69.3 & 39 & 78.5 & 50.1 & 47.6 & 66.5 & 
         54.9 \\
         InternVL3-1B ~\cite{zhu2025internvl3}  & 45.8 & 60.8 & 69.4 & 41.4 & 79 & 51.5 & 58.7 & 43.4 & 57.2 \\
         Ovis2-1B ~\cite{lu2024ovis}  & 49 & 59.4 & 76.4 & 45.2 & 89 & 52.1 & 50 & 68.3 & 59.6 \\
         MM1.5-1B ~\cite{zhang2024mm1_5}  & 35.8 & 37.2 & 59.3 & - & 60.5 & - &  37.4 & - &- \\
         \hline
    \end{tabular}
    \caption{Performance of AndesVL and other MLLMs on OpenCompass academic benchmarks. The best results are in bold.}
    \label{tab:benchmark_1}
\end{table}

Table \ref{tab:benchmark_1} illustrates the detailed evaluation results of different MLLMs on OpenCompass academic benchmarks. Some results are sourced from the benchmark papers and the OpenCompass leaderboard~\cite{opencompass2023}. 

As indicated in the table, our proposed model, AndesVL, demonstrates significant improvements in various multimodal tasks when compared to prior models of similar parameter size. This enhancement highlights the effectiveness of our advanced training strategies and the quality of the training corpus utilized.

AndesVL-4B achieves an overall score of 66.2 on the OpenCompass academic benchmarks, the highest among all evaluated models. This result underscores the model's proficiency in addressing a range of real-world tasks that require multimodal perception, understanding, and reasoning.

Notably, our model attains an impressive score of 55.4 on the general multimodal benchmark, MMMU, surpassing all other leading models. This exceptional performance reflects AndesVL's capability in handling complex multimodal tasks effectively. 

Furthermore, AndesVL-4B scores 70.2 on the MathVista benchmark, significantly advancing the state-of-the-art performance by nearly 10 points. This improvement illustrates the model's superior capabilities in multimodal mathematics and reasoning scenarios.




==> section/experiments/experiment_results/visual_grounding_benchmark_results.tex <==
\subsubsection{Evaluation Results}
\begin{table}
    \centering
    \begin{tabular}{l|ccc|ccc|cc|c}
        \hline
         Model &  \multicolumn{3}{c|}{RefCOCO} &\multicolumn{3}{c|}{RefCOCO+} &  \multicolumn{2}{c|}{RefCOCOg} & overall  \\
         & val & test-A & test-B & val & test-A & test-B & val & test & \\
         \hline
         AndesVL-4B &  \textbf{90} & \textbf{92.5} & \textbf{86.2} & \textbf{82.8} & \textbf{88} & \textbf{77} & \textbf{87.4} & \textbf{86.5} & \textbf{86.3}\\
         Qwen2.5-VL-3B ~\cite{bai2025qwen2_5} & 89.1 & 91.7 & 84 & 82.4 & 88 & 74.1 & 85.2 & 85.7 & 85 \\
         InternVL2-4B ~\cite{chen2024expanding} &  84.4 & 91.2 & 83.9 & 81.2 & 87.2 & 73.8 & 84.6 & 84.6 & 84.4 \\
         MM1.5-3B ~\cite{zhang2024mm1_5} & - & 92 & 86.1 & - & 87.7 & 75.9 & - & 86.4 & -\\
         \hline
         AndesVL-2B &   &  &  &  &  &   &  &  &  \\
         Qwen2-VL-2B ~\cite{wang2024qwen2vl} & 87.6 &  90.6 & 82.3 & 79 & 84.9  & 71 & 81.2& 80.3 & 82.1 \\
         InternVL2-2B ~\cite{chen2024expanding} & 82.3 & 88.2 & 75.9 &  73.5 & 82.8 & 63.3  & 77.6 & 78.3 & 77.7 \\
         InternVL3-2B ~\cite{zhu2025internvl3} &  89.8 & 92.6 & 86.4 & 84 & 89.2 & 76.5  & 87.6 & 87.2 & 86.7 \\
         \hline
         AndesVL-1B &  &  &  &  &  &  & & & \\
         InternVL3-1B ~\cite{zhu2025internvl3} & 85.8 & 90.1 & 81.7 & 76.6 & 84.1 & 69.2 & 82.8 & 82.6 & 81.6 \\
         MM1.5-1B ~\cite{zhang2024mm1_5} & - & 89.3 & 81.9 & - & 83.7 & 69.3 &  - & 82.8 &-\\
         \hline
    \end{tabular}
    \caption{Comparison of visual grounding performance. The best results are in bold.}
    \label{tab:benchmark_grounding}
\end{table}

The detailed evaluation results on visual grounding benchmarks are presented in Table ~\ref{tab:benchmark_grounding}. Among existing advanced models, the proposed AndesVL-4B achieves the highest average score of 86.3. More specifically, AndesVL-4B demonstrates top performance in RefCOCO, RefCOCO+, and RefCOCO, among others, revealing its significant advantages over competing models in various visual grounding tasks. These results underscore the importance of our refined grounding corpus and model optimization strategies.


==> table/ablation_mpo.tex <==
\begin{table*}[t!]

\centering
\small
\setlength\tabcolsep{3pt}
% \renewcommand{\arraystretch}{0.9}
\begin{tabular}{l|c|ccccccc|l}
{Model}   & MPO    & {MMMU}        & {MathVista}        & {MathVision}        & {MathVerse}           & {DynaMath}        & {WeMath}        & {LogicVista}        & {Overall}    \\ 
\hline
% \rowcolor{gray!15}
\multirow{2}{*}{InternVL3-1B}   & \no   & 43.4          & 47.2               & 13.8                & 18.1                  & 4.2               & 14.7            & 31.1                & 24.6         \\
 &  \yes & 43.4          & 45.8               & 18.8                 & 18.7                   & 5.8             & 13.4            & 29.8             & 25.1 \gbf{+0.5}        \\

       % & \textcolor{red}{\textbf{+0.0}}          & \textcolor{red}{\textbf{-1.4}}               & \textcolor{red}{\textbf{+5.0}}                & \textcolor{red}{\textbf{+0.6}}                  & \textcolor{red}{\textbf{+1.6}}               & \textcolor{red}{\textbf{-1.3}}            & \textcolor{red}{\textbf{-1.3}}                & \textcolor{red}{\textbf{+0.5}}         \\
\hline
% \rowcolor{gray!15}
\multirow{2}{*}{InternVL3-2B}   & \no    & 49.1          & 59.0               & 22.0                & 23.2                  & 13.4              & 18.1            & 30.0                & 30.7         \\
 & \yes & 48.6           & 57.0               & 21.7                & 25.3                  & 14.6              & 22.4            & 36.9                & 32.4 \gbf{+1.7}        \\

       % & \textcolor{red}{\textbf{-0.5}}          & \textcolor{red}{\textbf{-2.0}}               & \textcolor{red}{\textbf{-0.3}}                & \textcolor{red}{\textbf{+2.1}}                  & \textcolor{red}{\textbf{+1.2}}               & \textcolor{red}{\textbf{+4.3}}            & \textcolor{red}{\textbf{+6.9}}                & \textcolor{red}{\textbf{+1.7}}         \\
\hline
% \rowcolor{gray!15}
\multirow{2}{*}{InternVL3-8B}   & \no       & 61.9          & 67.4               & 24.7                & 36.9                  & 22.8              & 32.7            & 43.2                & 41.4         \\
& \yes  & 62.7          & 71.6               & 29.3                & 39.8                  & 25.5              & 37.1            & 44.1                & 44.3 \gbf{+2.9}          \\
       % & \textcolor{red}{\textbf{+0.8}}          & \textcolor{red}{\textbf{+4.2}}               & \textcolor{red}{\textbf{+4.6}}                & \textcolor{red}{\textbf{+2.9}}                  & \textcolor{red}{\textbf{+2.7}}               & \textcolor{red}{\textbf{+4.4}}            & \textcolor{red}{\textbf{+0.9}}                & \textcolor{red}{\textbf{+2.9}}         \\
\hline
% \rowcolor{gray!15}
\multirow{2}{*}{InternVL3-9B}   & \no       & 59.0          & 68.8               & 28.9                & 32.2                  & 23.0              & 32.5            & 46.5                & 41.6         \\
& \yes  & 57.7          & 71.5               & 27.6                & 35.3                  & 26.7              & 33.8            & 49.2                & 43.1 \gbf{+1.5}          \\
       % & \textcolor{red}{\textbf{-1.3}}          & \textcolor{red}{\textbf{+2.7}}               & \textcolor{red}{\textbf{-1.3}}                & \textcolor{red}{\textbf{+3.1}}                  & \textcolor{red}{\textbf{+3.7}}               & \textcolor{red}{\textbf{+1.3}}            & \textcolor{red}{\textbf{+2.7}}                & \textcolor{red}{\textbf{+1.5}}         \\
\hline
% \rowcolor{gray!15}
\multirow{2}{*}{InternVL3-14B}   & \no       & 67.1          & 70.5               & 31.2                & 38.8                  & 27.9              & 38.1            & 49.9                & 46.2         \\
& \yes & 67.1          & 75.1               & 37.2                & 44.4                  & 31.3              & 43.0            & 51.2                & 49.9 \gbf{+3.7}          \\
       % & \textcolor{red}{\textbf{+0.0}}          & \textcolor{red}{\textbf{+4.6}}               & \textcolor{red}{\textbf{+6.0}}                & \textcolor{red}{\textbf{+5.6}}                  & \textcolor{red}{\textbf{+3.4}}               & \textcolor{red}{\textbf{+4.9}}            & \textcolor{red}{\textbf{+1.3}}                & \textcolor{red}{\textbf{+3.7}}         \\
\hline
% \rowcolor{gray!15}
\multirow{2}{*}{InternVL3-38B}   & \no       & 69.3          & 71.2               & 34.2                & 45.1                  & 22.2              & 41.7            & 54.4                & 48.3         \\
& \yes & 70.1          & 75.1               & 34.2                & 48.2                  & 35.3              & 48.6            & 58.4                & 52.8 \gbf{+4.5}         \\
       % & \textcolor{red}{\textbf{+0.8}}          & \textcolor{red}{\textbf{+3.9}}               & \textcolor{red}{\textbf{+0.0}}                & \textcolor{red}{\textbf{+3.1}}                  & \textcolor{red}{\textbf{+13.1}}               & \textcolor{red}{\textbf{+6.9}}            & \textcolor{red}{\textbf{+4.0}}                & \textcolor{red}{\textbf{+4.5}}         \\
\hline
% \rowcolor{gray!15}
\multirow{2}{*}{InternVL3-78B}   & \no       & 72.2          & 74.0               & 35.2                & 44.2                  & 31.7              & 42.5            & 53.5                & 50.5         \\ 
& \yes & 72.2          & 79.0               & 43.1                & 51.0                  & 35.1              & 46.1            & 55.9                & 54.6 \gbf{+4.1}         \\
       % & \textcolor{red}{\textbf{+0.0}}          & \textcolor{red}{\textbf{+5.0}}               & \textcolor{red}{\textbf{+7.9}}                & \textcolor{red}{\textbf{+6.8}}                  & \textcolor{red}{\textbf{+3.4}}               & \textcolor{red}{\textbf{+3.6}}            & \textcolor{red}{\textbf{+2.4}}                & \textcolor{red}{\textbf{+4.1}}         \\
\end{tabular}
\caption{{\textbf{Comparison of reasoning abilities before and after Mixed Preference Optimization (MPO).}
% \wwh{check}
% 突出差值
}
}
\label{tab:ablation_mpo}
\end{table*}

==> table/benchmark_alignment.tex <==

\begin{table*}[!t]
\centering

\resizebox{\linewidth}{!}{
\begin{tabular}{l|c|ccccc|c}
% \diagbox{Models}{Datasets }
\multirow{2}{*}{model name} & \multirow{2}{*}{\#param}  & {AlpacaEval} & {MTBench} & {CompassArena} & {AlignBench} & {IFEval} & \multirow{2}{*}{avg.} \\
& & (WinRate) & (0-10 Score) & (WinRate) & (0-10 Score) & (0-100 Acc) \\
\hline
% \multicolumn{7}{c}{\purplecolor{{\ding{72}API Models}}} \\
GPT-3.5 & - & 9.6 & 8.4 & 24.7 & 5.7 & - & - \\
\hline
% \multicolumn{7}{c}{\greencolor{{$\triangle$ $\sim7B\ Models$}}} \\

Llama2-7B-Chat & 7B & 5 & 6.3 & 6.5 & - & 44.6 & - \\
Llama2-13B-Chat & 13B & 7.7 & 6.7 & 9.8 & - & 46.1 & -\\

Mistral-7B-Instruct-v0.2 & 7.3B & {14.7} & - & 14.2 & -  & {{57.9}} & - \\
Mixtral-8x7B-Instruct-v0.1 & 46.7B & - & {{8.3}} & 18.9 & - & {56.5} & -\\

Baichuan2-7B-Chat & 7B & - & - & 16.1 & 5.1 & 42.1 & -\\
Baichuan2-13B-Chat & 13B & - & - & 20.5 & 5.3 & 42.5 & - \\

Qwen-7B-Chat & 7B & - & - & 15.8 & 4.7 & 37.3 & - \\
Qwen-14B-Chat & 14B & 7.5 & 7.0 & 24.8 & 5.4 & 43.8 & - \\

ChatGLM3-6B & 6.2B  & - & - & 17.2 & 5.0 & 33.7 & - \\
\hline
\rowcolor{gray!15}
InternLM2-Chat-7B-SFT & 7B & 6.9 & 7.1 & 14.1 & 4.9 & 48.5 & 16.3 \\
\rowcolor{gray!15}
InternLM2-Chat-7B & 7B & 11.3 & {7.7} & {28.7} & {6.1} & 45.9 & {19.9} \\
\rowcolor{gray!15}
InternLM2-Chat-20B-SFT & 20B & 8.0 & 7.3 & 15.2 & 5.3 & 48.7  & 16.9  \\
\rowcolor{gray!15}
InternLM2-Chat-20B & 20B & {{21.8}} & 7.9 & {{31.4}} & {{6.8}} & 42.2 & {{22.0}} \\
\end{tabular}}
\caption{\textbf{Comparison of models on alignment benchmarks}. }

\label{tab:alignment_model_results}
\end{table*}



==> table/benchmark_grounding.tex <==
\begin{table*}[t] 
\centering 
\renewcommand{\arraystretch}{0.95}
\setlength\tabcolsep{8pt}
{\fontsize{8}{10}\selectfont 
\begin{tabular}{l|ccc|ccc|cc|c}
\multirow{2}{*}{{Model Name}}           & \multicolumn{3}{c|}{{RefCOCO}} & \multicolumn{3}{c|}{{RefCOCO+}} & \multicolumn{2}{c|}{{RefCOCOg}} & \multirow{2}{*}{{Overall}} \\
                                        & val    & test-A    & test-B    & val    & test-A    & test-B     & val     & test                 &         \\
\hline
Grounding-DINO-L~\citep{grounding_dino} & 90.6   & 93.2      & 88.2      & 82.8   & 89.0      & 75.9       & 86.1    & 87.0                 & 86.6    \\
UNINEXT-H~\citep{uninext}               & 92.6   & 94.3      & 91.5      & 85.2   & 89.6      & 79.8       & 88.7    & 89.4                 & 88.9    \\
ONE-PEACE~\citep{one-peace}             & 92.6   & 94.2      & 89.3      & 88.8   & 92.2      & 83.2       & 89.2    & 89.3                 & 89.8    \\
\hline
Qwen2.5-VL-3B~\cite{bai2025qwen2}       & 89.1   & 91.7      & 84.0      & 82.4   & 88.0      & 74.1       & 85.2    & 85.7                 & 85.0    \\
\rowcolor{gray!15}
InternVL3-1B                             & 85.8   & 90.1      & 81.7      & 76.6   &	84.1	  & 69.2	   & 82.8    & 82.6                 & 81.6    \\
\rowcolor{gray!15}
InternVL3-2B                             & 89.8   & 92.6	     & 86.4      & 84.0	  & 89.2      & 76.5       & 87.6    & 87.2                 & 86.7    \\
Shikra-7B~\citep{chen2023shikra}        & 87.0   & 90.6      & 80.2      & 81.6   & 87.4      & 72.1       & 82.3    & 82.2                 & 82.9    \\
% Qwen-VL~\citep{bai2023qwenvl}           & 89.4   & 92.3      & 85.3      & 83.1   & 88.3      & 77.2       & 85.6    & 85.5                 & 85.8    \\ 
Ferret-v2-13B~\citep{ferretv2}          & 92.6   & 95.0      & 88.9      & 87.4   & 92.1      & 81.4       & 89.4    & 90.0                 & 89.6    \\
CogVLM-Grounding~\citep{wang2023cogvlm} 
                                        & 92.8   & 94.8      & 89.0      & 88.7   & 92.9      & 83.4       & 89.8    & 90.8                 & 90.3    \\
MM1.5~\cite{zhang2024mm1_5}             & --     & 92.5      & 86.7      & --     & 88.7      & 77.8       & --      & 87.1                 & --      \\
Qwen2-VL-7B~\cite{wang2024qwen2vl}      & 91.7   & 93.6      & 87.3      & 85.8   & 90.5      & 79.5       & 87.3    & 87.8                 & 87.9    \\
Qwen2.5-VL-7B~\cite{bai2025qwen2}       & 90.0   & 92.5      & 85.4      & 84.2   & 89.1      & 76.9       & 87.2    & 87.2                 & 86.6    \\
TextHawk2~\citep{yu2024texthawk2}       & 91.9   & 93.0      & 87.6      & 86.2   & 90.0      & 80.4       & 88.2    & 88.1                 & 88.2    \\
InternVL2-8B~\cite{chen2024far}         & 87.1   & 91.1      & 80.7      & 79.8   & 87.9      & 71.4       & 82.7    & 82.7                 & 82.9    \\

InternVL2.5-8B~\cite{chen2024expanding} & 90.3   & 94.5      & 85.9      & 85.2   & 91.5      & 78.8       & 86.7    & 87.6                 & 87.6    \\
\rowcolor{gray!15}
InternVL3-8B                            & 92.5   & 94.6      & 88.0      & 88.2   & 92.5      & 81.8       & 89.6    & 90.0                 & 89.6    \\
\rowcolor{gray!15}
InternVL3-9B                            & 91.8  & 93.2     & 86.6     & 86.4  & 91.0     & 79.9      & 88.0   & 88.5                & 88.2    \\  
\rowcolor{gray!15}
InternVL3-14B                           & 92.0  & 94.4     & 87.8     & 87.4  & 92.1     & 81.5      & 88.6   & 89.3                 & 89.1    \\  
\hline

Qwen2-VL-72B~\cite{wang2024qwen2vl}     & 93.2   & 95.3      & 90.7      & 90.1   & 93.8      & 85.6       & 89.9    & 90.4                 & 91.1    \\
Qwen2.5-VL-72B~\cite{bai2025qwen2}      & 92.7   & 94.6      & 89.7      & 88.9   & 92.2      & 83.7       & 89.9    & 90.3                 & 90.3    \\
InternVL2-Llama3-76B~\cite{chen2024far} & 92.2   & 94.8      & 88.4      & 88.8   & 93.1      & 82.8       & 89.5    & 90.3                 & 90.0    \\
InternVL2.5-78B~\cite{chen2024expanding}& 93.7   & 95.6      & 92.5      & 90.4   & 94.7      & 86.9       & 92.7    & 92.2                 & 92.3    \\
\rowcolor{gray!15}
InternVL3-38B                           & 93.2   & 95.1      & 90.2      & 89.8   & 93.2      & 85.2       & 91.4    & 91.5                 & 91.2    \\
\rowcolor{gray!15}  
InternVL3-78B                           & 93.4   & 95.4      & 90.3      & 90.1   & 93.8      & 85.3       & 91.5    & 91.5                 & 91.4    \\
% \rowcolor{gray!15}
% InternVL2.5-Pro                       &        &           &           &        &           &            &         &                      &         \\
\end{tabular}
}
\caption{\textbf{Comparison of visual grounding performance.}
We evaluate InternVL's visual grounding capability on RefCOCO, RefCOCO+, and RefCOCOg datasets~\cite{kazemzadeh2014referitgame, mao2016generation}. Parts of the results are collected from \cite{wang2024qwen2vl}.
} 
\label{tab:benchmark-grounding}
\end{table*}
%  91.9 93.0 87.6 86.2 90.0 80.4 88.2 88.1

==> table/benchmark_gui_grounding.tex <==
\begin{table*}[h]
\centering
\small
\footnotesize
% \resizebox{\textwidth}{!}
{\fontsize{8}{10}\selectfont 
\setlength\tabcolsep{4pt}
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
\textbf{Method} & GPT-4o & Gemini 2.0 & Claude & Aguvis-72B & Qwen2.5-VL-72B & UI-TARS-72B & InternVL3-8B & -38B & -72B\\ 
\midrule
ScreenSpot & 18.1 & 84.0 & 83.0 & \textbf{89.2} & 87.1 & 88.4 & 79.5 & 85.6 & 88.7 \\ 
ScreenSpot-V2 & $-$ & $-$ & $-$ & $-$ & $-$ & 90.3 & 81.4 & 88.3 & \textbf{90.9} \\  
% ScreenSpot Pro & - & - & 17.1 & 23.6 & 38.1 & \textbf{43.6} &  & 13.1 & 20.4 & 26.3 \\  
\bottomrule
\end{tabular}
}
\caption{\textbf{Performance of InternVL3 and other models on GUI grounding benchmarks.}}
\label{tab:gui_grounding}
\end{table*}

==> table/benchmark_in_cls.tex <==
\begin{table*}[t!]
\centering
{\fontsize{8}{10}\selectfont 
\renewcommand{\arraystretch}{1.1}
\setlength\tabcolsep{1.3pt}
\begin{tabular}{l|c|ccccccc|ccccccc|c}
                          &                        & \multicolumn{7}{c|}{Linear Probing} & \multicolumn{7}{c|}{Attention Pooling Probing} &   \\

\multirow{-2}{*}{Model Name}& \multirow{-2}{*}{res.} & IN-1K & IN-ReaL & IN-V2 & IN-A & IN-R & IN-Ske & avg.                      & IN-1K & IN-ReaL & IN-V2 & IN-A & IN-R & IN-Ske & avg.                     & \multirow{-2}{*}{$\Delta$} \\
\hline
\textcolor{gray}{InternViT-6B-224px}        & \textcolor{gray}{224}                    & \textcolor{gray}{88.2}  & \textcolor{gray}{90.4}    & \textcolor{gray}{79.9}  & \textcolor{gray}{77.5} & \textcolor{gray}{89.8} & \textcolor{gray}{69.1}   & \textcolor{gray}{82.5}                      & \textcolor{gray}{89.2}  & \textcolor{gray}{91.1}    & \textcolor{gray}{82.3}  & \textcolor{gray}{84.7} & \textcolor{gray}{93.1} & \textcolor{gray}{72.7}   & \textcolor{gray}{85.5}                     & \textcolor{gray}{3.0}    \\
InternViT-6B-224px        & 448                    & 87.8  & 90.2    & 79.8  & 77.2 & 87.1 & 65.8   & \cellcolor{gray!15} 81.3  & 88.8  & 91.0    & 82.0  & 85.4 & 91.3 & 70.5   & \cellcolor{gray!15} 84.8 & 3.5    \\
InternViT-6B-448px-V1.0   & 448                    & 87.0  & 90.0    & 78.8  & 77.2 & 85.5 & 65.1   & \cellcolor{red!15} 80.6 & 88.7  & 91.0    & 82.0  & 88.7 & 92.8 & 72.0   & \cellcolor{green!15} 85.9  & 5.3    \\
InternViT-6B-448px-V1.2   & 448                    & 87.0  & 89.9    & 78.5  & 77.1 & 83.9 & 59.7   & \cellcolor{red!15} 79.4 & 88.6  & 91.1    & 82.0  & 88.7 & 92.7 & 71.6   & \cellcolor{green!15} 85.8  & 6.4    \\
InternViT-6B-448px-V1.5   & 448                    & 86.5  & 89.9    & 78.1  & 69.8 & 82.9 & 60.1   & \cellcolor{red!15} 77.9 & 88.4  & 91.2    & 81.6  & 86.0 & 92.2 & 70.9   & \cellcolor{green!15} 85.1  & 7.2    \\
InternViT-6B-448px-V2.5   & 448                    & 86.6  & 90.1    & 77.8  & 73.7 & 82.7 & 60.0   & \cellcolor{red!15} 78.5 & 88.3  & 91.2    & 81.3  & 86.9 & 92.4 & 70.8   & \cellcolor{green!15} 85.2  & 6.7    \\
% \hline
% CLIP-ViT-Large-336px      & 336 &  \\
% InternViT-300M-448px-V1.0 & 448                    &       &         &       &      &      &        &                           &       &         &       &      &      &        &                          &        \\
% InternViT-300M-448px-V2.5 & 448                    &       &         &       &      &      &        &                           &       &         &       &      &      &        &                          &        \\
\end{tabular}
}
\caption{\textbf{Image classification performance across different versions of InternViT.}
We use IN-1K~\cite{deng2009imagenet} for training and evaluate on the IN-1K validation set as well as multiple ImageNet variants, including IN-ReaL~\cite{beyer2020imagenetreal}, IN-V2~\cite{recht2019imagenetv2}, IN-A~\cite{hendrycks2021imagenet_a}, IN-R~\cite{hendrycks2021imagenet_r}, and IN-Sketch~\cite{wang2019imagenet_sketch}.
Results are reported for both linear probing and attention pooling probing methods, with average accuracy for each method. 
$\Delta$ represents the performance gap between attention pooling probing and linear probing, where a larger $\Delta$ suggests a shift from learning simple linear features to capturing more complex, nonlinear semantic representations.
    }
\label{tab:benchmark_in_cls}
\end{table*}


==> table/benchmark_long_context.tex <==
\begin{table*}[t!]
\centering
\renewcommand{\arraystretch}{0.95}
\setlength\tabcolsep{3.2pt}
\newcommand{\MMLongBench}{\makecell{MMLong-Doc\\(Acc / F1)}}
\newcommand{\MPD}{\makecell{MPDoc\\(val)}}
\newcommand{\SlideVQA}{\makecell{SlideVQA-Mini\\(ANLS / EM / F1)}}
\newcommand{\DocGenome}{\makecell{DocGenome\\(SP Acc / MP Acc)}}
\newcommand{\MMNIAH}{\makecell{MM-NIAH\\(Short / Medium / Long / Overall)}}
{\fontsize{8}{10}\selectfont 
\begin{tabular}{l|ccccccc}
Model Name                              & \MPD& \MMLongBench & \SlideVQA          & \DocGenome & \MMNIAH \\
\hline
InternVL2-1B~\cite{chen2024far}         & 64.7 & 7.8 / 9.1    & 28.8 / 22.4 / 26.3 &            &         \\
\rowcolor{gray!15}
InternVL2.5-1B                          & 71.2 &              &                    &            &         \\
InternVL2-2B~\cite{chen2024far}         & 71.8 & 10.5 / 10.8  & 35.4 / 28.3 / 32.3 &            &         \\
\rowcolor{gray!15}
InternVL2.5-2B                          & 76.3 &              &                    &            &         \\
\hline
InternVL2-4B~\cite{chen2024far}         & 76.3 & 12.6 / 11.9  & 50.1 / 40.7 / 45.6 &            &         \\
\rowcolor{gray!15}
InternVL2.5-4B                          & 81.7 &              &                    &            &         \\
\hline
InternVL2-8B~\cite{chen2024far}         & 79.3 & 17.4 / 16.5  & 55.7 / 44.3 / 49.6 &            &         \\
\rowcolor{gray!15}
InternVL2.5-8B                          & 82.4 &              &                    &            &         \\
\hline
InternVL-Chat-V1.5~\cite{chen2024far}   & 77.7 & 12.7 / 12.5  & 51.3 / 41.1 / 46.8 &            &         \\
InternVL2-26B~\cite{chen2024far}        & 80.2 & 16.3 / 15.3  & 56.3 / 45.3 / 50.9 &            &         \\
\rowcolor{gray!15}
InternVL2.5-26B                         & 85.1 &              &                    &            &         \\
\hline
InternVL2-40B~\cite{chen2024far}        & 77.2 & 17.7 / 16.7  & 56.9 / 46.0 / 51.5 &            &         \\
\rowcolor{gray!15}
InternVL2.5-38B                         & 87.0 &              &                    &            &         \\
\hline
InternVL2-Llama3-76B~\cite{chen2024far} & 80.1 & 21.1 / 20.0  & 61.1 / 50.9 / 56.2 &            &         \\
\rowcolor{gray!15}
InternVL2.5-Llama3.1-76B                &      &              &                    &            &         \\
\rowcolor{gray!15}
InternVL2.5-Pro                         &      &              &                    &            &         \\

\end{tabular}
}
\caption{\textbf{Comparison of multimodal long context performance.}
We evaluate InternVL's long-context capabilities across 5 benchmarks, including MPDocVQA~\cite{tito2023hier}, MMDU~\cite{liu2024mmdu}, MMLongBench-Doc~\cite{ma2024mmlong}, DUDE~\cite{van2023document}, MM-NIAH~\cite{wang2024needle}, and DocGenome~\cite{xia2024docgenome}.
}
\label{tab:benchmark_long_context}
\end{table*}

==> table/benchmark_long_context_lm.tex <==
\begin{table*}[!t]
\centering

\resizebox{\linewidth}{!}{
\tablestyle{10pt}{1.2}
\begin{tabular}{l|c|ccc|ccccccc}

\multirow{2}{*}{model name} & \multirow{2}{*}{\#param} & \multicolumn{3}{c|}{L-Eval} & \multicolumn{7}{c}{LongBench} \\
& & Close & Open  & avg.  & Single & Multi & Summ & FSL & Syn & Code & avg. \\ 
\hline
% \multicolumn{11}{c}{\greencolor{\textit{ $\leq 7$B Models}}} \\ 
Llama2-7B-Chat & 7B & 20.0 & 33.1 & 29.4 & 23.1 & 17.0 & 18.5 & 7.0 & 5.0 & 15.4 & 14.3 \\
Llama2-13B-Chat & 13B & 27.3 & 34.4 & 32.5 & 18.2 & 9.9 & 18.5 & 6.7 & 10.0 & 18.1 & 13.6 \\

Mistral-7B-Instruct-v0.2 & 7.3B & 54.3 & 34.0 & 39.7 & 31.3 & 26.4 & 21.8 & 46.6 & 59.2 & 44.8 & 38.3 \\
Mixtral-8x7B-Instruct-v0.1 & 46.7B & 65.3 & 35.6 & 43.9 & 35.0 & 25.6 & 17.1 & 35.9 & 68.2 & 40.0 & 37.0 \\

Baichuan2-7B-Chat & 7B & 36.1 & 32.4 & 33.4 & 30.3 & 18.4 & 21.8 & 42.5 & 6.6 & 36.0 & 25.9 \\
Baichuan2-13B-Chat & 13B & 40.6 & 32.3 & 34.6 & 34.3 & 29.1 & 21.3 & 45.5 & 4.0 & 51.4 & 30.9 \\

Qwen-7B-Chat & 7B & 13.6 & 32.6 & 27.3 & 27.9 & 14.2 & 21.0 & 21.8 & 8.3 & 28.9 & 20.4 \\
Qwen-14B-Chat & 14B & 35.3 & 33.5 & 34.0 & 32.6 & 19.4 & 22.5 & 36.9 & 23.7 & 42.9 & 29.7 \\

% Qwen1.5-7B-Chat & 54.2 & 38.1 & 42.6 & 42.7 & 36.1 & 16.8 & 36.7 & 30.7 & 46.7 & 35.0 \\
% Qwen1.5-14B-Chat & 64.2 & 36.4 & 44.1 & 41.7 & 38.9 & 17.2 & 36.9 & 62.3 & {60.3} & 42.9 \\

ChatGLM3-6B & 6.2B & 59.1 & 35.0 & 41.7 & 40.9 & 45.0 & 26.0 & 56.5 & 65.0 & {57.1} & {48.4} \\

\hline
\rowcolor{gray!15}
InternLM2-Chat-7B & 7B & 68.6 & {40.8} & 48.5 & 45.7 & 43.1 & {26.5} & 58.3 & 66.3 & 36.4 & 46.1 \\
\rowcolor{gray!15}
InternLM2-Chat-7B-SFT & 7B & {68.7} & {40.8} & {48.6} & {47.3} & {45.2} & 25.3 & {59.9} & {67.2} & 43.5 & 48.1 \\
\rowcolor{gray!15}
InternLM2-Chat-20B & 20B & 68.6 & 40.6 & 48.4 & {46.9} & 46.7 & {26.0} & 49.1 & 67.3 & 32.6 & 44.8 \\
\rowcolor{gray!15}
InternLM2-Chat-20B-SFT & 20B & {68.8} & {42.0} & {49.4} & 46.8 & {48.7} & 25.6 & {51.2} & {67.9} & 40.4 & {46.8} \\ 
\end{tabular}}
\caption{\textbf{Comparison of chat models on long-context Benchmarks}. 
For each benchmark and task group, we report the average accuracies of intra-group subtasks.
\textbf{L-Eval abbrs}: Close $\rightarrow$ close-ended; Open $\rightarrow$ open-ended. 
\textbf{LongBench abbrs}: Single $\rightarrow$ single-document; Multi $\rightarrow$ multi-document; Summ $\rightarrow$ summarization; FSL $\rightarrow$ few shot learning; Syn $\rightarrow$ synthetic. 
All results are obtained with the OpenCompass~\cite{opencompass2023} evaluation toolkit. }
% \vspace{-2mm}
\label{tab:longtext_chat_results}
\end{table*}


==> table/benchmark_math_reasoning.tex <==
\begin{table*}[t!]
\centering
\fontsize{8}{10}\selectfont 
\setlength\tabcolsep{4pt}
\renewcommand{\arraystretch}{0.9}
\begin{tabular}{l|ccccccc|c}
{Model}                           & {MMMU} & {MathVista} & {MathVision} & {MathVerse} & {DynaMath} & {WeMath} & {LogicVista} & {Overall} \\ 
\hline
LLaVA-OV-0.5B~\cite{li2024llavaov}       & 31.4          & 34.8               & $-$                   & $-$                  & $-$                 & $-$               & $-$                   & $-$                \\
InternVL2.5-1B~\cite{chen2024expanding}  & 41.2          & 47.1               & 21.1                & 16.4               & 5.6               & 11.1            & 26.0                & 24.1             \\
\rowcolor{gray!15}
InternVL3-1B                             & 43.4          & 45.8               & 18.8                & 18.7               & 5.8               & 13.4            & 29.8                & 25.1             \\
\rowcolor{gray!15}
\emph{\textcolor{blue}{w/ VisualPRM-Bo8}}~\cite{wang2025visualprm}                              & 55.4          & 62.1               & 21.7                & 28.9               & 13.4              & 28.5            & 34.9                & 35.0             \\
\hline
Aquila-VL-2B~\cite{gu2024aquilavl}       & 46.9          & 59.1               & 17.9                & 17.4               & 5.0               & 15.9            & 30.6                & 27.5             \\
Qwen2.5-VL-3B~\cite{bai2025qwen2_5}      & 51.2          & 61.2               & 21.9                & 31.2               & 13.2              & 22.9            & 40.3                & 34.6             \\
Ovis-2B~\cite{lu2024ovis}                & 45.6          & 64.1               & 17.7                & 29.4               & 10.0              & 9.9             & 34.7                & 30.2             \\
Ovis-4B~\cite{lu2024ovis}                & 49.0          & 69.6               & 21.5                & 38.5               & 18.0              & 16.9            & 35.3                & 35.5             \\
InternVL2.5-2B~\cite{chen2024expanding}  & 43.2          & 51.1               & 14.0                & 22.3               & 4.4               & 8.0             & 27.3                & 24.3             \\
InternVL2.5-4B~\cite{chen2024expanding}  & 51.8          & 64.1               & 18.4                & 27.7               & 15.2              & 21.2            & 34.2                & 33.2             \\
\rowcolor{gray!15}
InternVL3-2B                             & 48.6          & 57.0               & 21.7                & 25.3               & 14.6              & 22.4            & 36.9                & 32.4             \\
\rowcolor{gray!15}
\emph{\textcolor{blue}{w/ VisualPRM-Bo8}}~\cite{wang2025visualprm}                              & 57.8          & 70.5               & 26.6                & 36.7               & 21.4              & 38.5            & 40.5                & 41.7             \\
\hline
LLaVA-OV-7B~\cite{li2024llavaov}         & 47.9          & 58.6               & 18.3                & 19.3               & 9.0               & 20.9            & 33.3                & 29.6             \\
MiniCPM-V2.6~\cite{yao2024minicpm}       & 49.8          & 60.8               & 23.4                & 18.9               & 9.8               & 16.4            & 27.5                & 29.5             \\
MiniCPM-o2.6~\cite{yao2024minicpm}       & 50.9          & 73.3               & 21.7                & 35.0               & 10.4              & 25.2            & 36.0                & 36.1             \\
Ovis-8B~\cite{lu2024ovis}                & 57.4          & 71.8               & 25.9                & 42.3               & 20.4              & 27.2            & 39.4                & 40.6             \\
Qwen2.5-VL-8B~\cite{bai2025qwen2_5}      & 55.0          & 67.8               & 25.4                & 41.1               & 21.0              & 35.2            & 44.1                & 41.4             \\
InternVL2.5-8B~\cite{chen2024expanding}  & 56.2          & 64.5               & 17.0                & 22.8               & 9.4               & 23.5            & 36.0                & 32.8             \\
\rowcolor{gray!15}
InternVL3-8B                             & 62.7          & 71.6               & 29.3                & 39.8               & 25.5              & 37.1            & 44.1                & 44.3             \\
\rowcolor{gray!15}
\emph{\textcolor{blue}{w/ VisualPRM-Bo8}}~\cite{wang2025visualprm}                              & 66.0          & 75.2               & 37.5                & 46.3               & 28.5              & 48.1            & 49.7                & 50.2             \\
\hline
\rowcolor{gray!15}
InternVL3-9B                             & 57.7          & 71.5               & 27.6                & 35.3               & 26.7              & 33.8            & 49.2                & 43.1             \\
\rowcolor{gray!15}
\emph{\textcolor{blue}{w/ VisualPRM-Bo8}}~\cite{wang2025visualprm}                              & 63.7          & 76.2               & 33.9                & 45.8               & 29.1              & 46.6            & 50.6                & 49.4             \\
\hline
Ovis2-16B~\cite{lu2024ovis}              & 60.7          & 73.7               & 30.1                & 45.8               & 26.3              & 45.0            & 47.4                & 47.0             \\
InternVL2.5-26B~\cite{chen2024expanding} & 60.7          & 68.2               & 23.4                & 24.0               & 11.4              & 30.9            & 39.6                & 36.9             \\
\rowcolor{gray!15}
InternVL3-14B                            & 67.1          & 75.1               & 37.2                & 44.4               & 31.3              & 43.0            & 51.2                & 49.9             \\
\rowcolor{gray!15}
\emph{\textcolor{blue}{w/ VisualPRM-Bo8}}~\cite{wang2025visualprm}                             & 69.3          & 77.9               & 40.1                & 47.7               & 33.1              & 52.0            & 56.2                & 53.8             \\
\hline
Cambrian-34B~\cite{tong2024cambrian}     & 49.7          & 53.2               & $-$                   & $-$                  & $-$                 & $-$               & $-$                   & $-$                \\
VILA-1.5-40B~\cite{lin2024vila}          & 55.1          & 49.5               & $-$                   & $-$                  & $-$                 & $-$               & $-$                   & $-$                \\
Ovis2-34B~\cite{lu2024ovis}              & 66.7          & 76.1               & 31.9                & 50.1               & 27.5              & 51.9            & 49.9                & 50.6             \\
InternVL2.5-38B~\cite{chen2024expanding} & 63.9          & 71.9               & 32.2                & 36.9               & 20.0              & 38.3            & 47.9                & 44.4             \\
\rowcolor{gray!15}
InternVL3-38B                            & 70.1          & 75.1               & 34.2                & 48.2               & 35.3              & 48.6            & 58.4                & 52.8             \\
\rowcolor{gray!15}
\emph{\textcolor{blue}{w/ VisualPRM-Bo8}}~\cite{wang2025visualprm}                              & 71.0          & 79.4               & 41.8                & 54.2               & 36.1              & 55.2            & 58.4                & 56.6             \\
\hline
GPT-4o-20241120~\cite{gpt4v}             & 70.7          & 60.0               & 31.2                & 40.6               & 34.5              & 45.8            & 52.8                & 47.9             \\
Claude-3.7-Sonnet~\cite{claude3series2024}& 75.0          & 66.8               & 41.9                & 46.7               & 39.7              & 49.3            & 58.2                & 53.9             \\
Gemini-2.0-Flash~\cite{gemini2_0}        & 72.6          & 70.4               & 43.6                & 47.8               & 42.1              & 47.4            & 52.3                & 53.7             \\
Gemini-2.0-Pro~\cite{gemini2_0pro}       & 69.9          & 71.3               & 48.1                & 67.3               & 43.3              & 56.5            & 53.2                & 58.5             \\
LLaVA-OV-72B~\cite{li2024llavaov}        & 55.7          & 67.1               & 25.3                & 27.2               & 15.6              & 32.0            & 40.9                & 37.7             \\
QvQ-72B-Preview~\cite{qvq-72b-preview}   & 70.3          & 70.3               & 34.9                & 48.2               & 30.7              & 39.0            & 58.2                & 50.2             \\
Qwen2.5-VL-72B~\cite{bai2025qwen2_5}     & 68.2          & 74.2               & 39.3                & 47.3               & 35.9              & 49.1            & 55.7                & 52.8             \\
InternVL2.5-78B~\cite{chen2024expanding} & 70.0          & 72.3               & 32.2                & 39.2               & 19.2              & 39.8            & 49.0                & 46.0             \\
\rowcolor{gray!15}
InternVL3-78B                            & 72.2          & 79.0               & 43.1                & 51.0               & 35.1              & 46.1            & 55.9                & 54.6             \\
\rowcolor{gray!15}
\emph{\textcolor{blue}{w/ VisualPRM-Bo8}}~\cite{wang2025visualprm}                              & 72.2          & 80.5               & 40.8                & 54.2               & 37.3              & 52.4            & 57.9                & 56.5             \\ 
\end{tabular}

\caption{\textbf{Comparison of multimodal reasoning and mathematical performance.}
MMMU~\cite{yue2023mmmu} is a multidisciplinary reasoning benchmark.
MathVista~\cite{lu2023mathvista}, MathVision~\cite{wang2024mathvision}, MathVerse~\cite{zhang2024mathverse}, DynaMath~\cite{zou2024dynamath}, and WeMath~\cite{qiao2024wemath} are mathematics benchmarks. For MathVerse, we report the performance on Vision-Only split.
LogicVista~\cite{xiao2024logicvista} is a logical reasoning benchmark.
Part of the results are collected from the OpenCompass leaderboard~\cite{opencompass2023}.
The overall score is the average score of the above benchmarks.
``w/ VisualPRM-Bo8'' denotes that the model is evaluated with Best-of-8 settings, where VisualPRM~\cite{wang2025visualprm} serves as the critic model.
}
\label{tab:benchmark_math_reasoning}
\end{table*}

==> table/benchmark_medical.tex <==
\begin{table*}[t!]
\scriptsize
\centering
\renewcommand{\arraystretch}{1.1}
\setlength\tabcolsep{4.5pt}
\newcommand{\MODELNAME}{\makecell{\\ model name}}
\newcommand{\PARAM}{\makecell{\\ \#param}}
\newcommand{\GMAIMMBench}{\makecell{\\GMAI-MMBench\\(val)}}
\newcommand{\WorldMedQABrazil}{\makecell{Brazil\\(t.only / t.\&i.)}}
\newcommand{\WorldMedQAIsrael}{\makecell{Israel\\(t.only / t.\&i.)}}
\newcommand{\WorldMedQAJapan}{\makecell{Japan\\(t.only / t.\&i.)}}
\newcommand{\WorldMedQASpain}{\makecell{Spain\\(t.only / t.\&i.)}}
\begin{tabular}{l|cccc|c}
\multirow{2}{*}{\MODELNAME}      & \multicolumn{4}{c|}{WorldMedQA-V}    & \multirow{2}{*}{\GMAIMMBench} \\
                                 & \WorldMedQABrazil & \WorldMedQAIsrael & \WorldMedQAJapan &  \WorldMedQASpain &  \\

\hline
InternVL2-1B                     &   &   &   &   & 36.3     \\
\rowcolor{gray!15}
InternVL2.5-1B                   &   &   &   &   & 39.3  \\
InternVL2-2B                     &   &   &   &   & 37.5 \\
\rowcolor{gray!15}
InternVL2.5-2B                   &   &   &   &   & 41.9 \\
\hline
InternVL2-4B                     &   &   &   &   & 38.7  \\
\rowcolor{gray!15}
InternVL2.5-4B                   &   &   &   &   & 45.4  \\
\hline
InternVL2-8B                     &   &   &   &   & 43.5  \\
\rowcolor{gray!15}
InternVL2.5-8B                   &   &   &   &   & 47.2  \\
\hline
InternVL-Chat-V1.5               &   &   &   &   & 38.9     \\
InternVL2-26B                    &   &   &   &   & 46.7  \\
\rowcolor{gray!15}
InternVL2.5-26B                  &   &   &   &   & 51.3  \\
\hline 
InternVL2-40B                    &   &   &   &   & 49.2  \\
\rowcolor{gray!15}
InternVL2.5-38B                  &   &   &   &   & 51.7  \\
\hline
InternVL2-Llama3-76B             &   &   &   &   &   \\
\rowcolor{gray!15}
InternVL2.5-Llama3.1-76B         &   &   &   &   &   \\
\end{tabular}
\caption{\textbf{Comparison of medical image understanding  performance.}
We evaluate InternVL's capabilities in medical image understanding across WorldMedQA-V~\cite{matos2024worldmedqa} and GMAI-MMBench~\cite{chen2024gmai}.
The two settings of WorldMedQA-V are text-only (t. only) and text and image (t. \& i.).
}
\label{tab:benchmark_medical}
\end{table*}
% worldmedqa-v https://www.arxiv.org/pdf/2410.12722 appendix5

==> table/benchmark_multi_image_real_world.tex <==
\begin{table*}[t!]
\scriptsize
\centering
{\fontsize{8}{10}\selectfont 
\renewcommand{\arraystretch}{0.95}
\setlength\tabcolsep{1.3pt}
\newcommand{\MMIU}{\makecell{MMIU}}
\newcommand{\Muir}{\makecell{Muir\\Bench}} % (test)
\newcommand{\BLINK}{\makecell{BLINK\\(val)}}
\newcommand{\Mantis}{\makecell{Mantis\\Eval}} % (test)
\newcommand{\RWQA}{\makecell{RealWorld\\QA}} % (test)
\newcommand{\MMERW}{\makecell{MME-RW\\(EN)}} % TODO
\newcommand{\RBench}{\makecell{R-Bench\\(test)}}
\newcommand{\TaskMe}{\makecell{TaskMe-\\Anything}}
\newcommand{\MMT}{\makecell{MMT\\(val)}}
\newcommand{\WILDV}{\makecell{WildVision\\(win rate)}}
\newcommand{\MIRB}{\makecell{MIRB\\(avg)}}
\newcommand{\RB}{\makecell{R-Bench\\(dis)}}
\newcommand{\TODO}{\textcolor{red}{TODO}}
\newcommand{\lsp}{--\ \ \ \ \ \ }
\newcommand{\rsp}{\ \ \ \ \ --~}
\begin{tabular}{l|ccccccc|ccccc}
Model Name                                 & \BLINK & \Mantis & \MMIU & \Muir & \MMT & \MIRB & Overall &\RWQA  & \MMERW & \WILDV  & \RB  & Overall \\
\hline
LLaVA-OneVision-0.5B~\cite{li2024llavaov}  & 52.1   & 39.6    & --    & 25.5  & --   & --    & --      & 55.6  & --     & --      & --   & --      \\
InternVL2-1B~\cite{chen2024far}            & 38.6   & 46.1    & 37.3  & 29.3  & 49.5 & 31.5  & 38.7    & 50.3  & 40.2   & 17.8    & 55.6 & 41.0    \\
InternVL2.5-1B~\cite{chen2024expanding}    & 42.0   & 51.2    & 38.5  & 29.9  & 50.3 & 35.6  & 41.3    & 57.5  & 44.2   & 43.4    & 59.0 & 51.0    \\
\rowcolor{gray!15}
InternVL3-1B                               & 42.9   & 50.2    & 39.3  & 31.2  & 52.9 & 36.1  & 42.1    & 58.2  & 46.0   & 43.8    & 60.4 & 52.1    \\
Qwen2-VL-2B~\cite{wang2024qwen2vl}         & 44.4   & --      & --    & --    & 55.1 & --    & --      & 62.6  & --     & --      & --   & --      \\
Qwen2.5-VL-3B~\cite{bai2025qwen2}          & 47.6   & --      & --    & 47.7    & -- & --    & --      & 65.4  & 53.1   & --      & --   & --      \\
% Aquila-VL-2B~\cite{gu2024aquilavl}       & --     & --      & --    & --    & 58.3 & --    & --      & 63.9  & --     & --      & --   & --      \\
InternVL2-2B~\cite{chen2024far}            & 43.8   & 48.4    & 39.8  & 32.5  & 50.4 & 32.1  & 41.2    & 57.3  & 47.3   & 31.8    & 56.8 & 48.3    \\
InternVL2.5-2B~\cite{chen2024expanding}    & 44.0   & 54.8    & 43.5  & 40.6  & 54.5 & 36.4  & 45.6    & 60.1  & 48.8   & 44.2    & 62.2 & 53.8    \\
\rowcolor{gray!15}
InternVL3-2B                               & 50.3   & 65.9    & 43.0  & 38.8  & 59.5 & 42.9  & 50.1    & 64.3  & 53.8   & 48.8    & 67.5 & 58.6    \\
\hline
Qwen2-VL-7B~\cite{wang2024qwen2vl}         & 53.2   & --      & --    & --    & 64.0 & --    & --      & 70.1  & 56.5   & --      & 64.0 & --      \\
Qwen2.5-VL-7B~\cite{bai2025qwen2}          & 56.4   & --      & --    & 59.6  & --   & --    & --      & 68.5  & 57.4   & --      & --   & --      \\
MiniCPM-V2.6~\cite{yao2024minicpm}         & 53.0   & 69.0    & --    & --    & 60.8 & --    & --      & 65.0  & --     & --      & --   & --      \\
InternVL2-8B~\cite{chen2024far}            & 50.9   & 65.4    & 42.0  & 48.7  & 60.0 & 50.0  & 52.8    & 64.4  & 53.5   & 54.4    & 67.9 & 60.1    \\
InternVL2.5-8B~\cite{chen2024expanding}    & 54.8   & 67.7    & 46.7  & 51.1  & 62.3 & 52.5  & 55.9    & 70.1  & 59.1   & 62.0    & 70.1 & 65.3    \\
\rowcolor{gray!15}
InternVL3-8B                               & 55.5   & 70.1    & 46.8  & 55.0  & 65.0 & 56.8  & 58.2    & 70.8  & 62.0   & 69.8    & 74.1 & 69.2    \\
\rowcolor{gray!15}
InternVL3-9B                               & 58.6   & 70.1    & 50.4  & 51.4  & 65.4 & 58.6  & 59.1    & 70.5  & 61.3   & 63.8    & 70.3 & 66.5    \\
\rowcolor{gray!15}
InternVL3-14B                              & 60.3   & 76.0    & 50.9  & 56.2  & 70.3 & 59.3  & 62.2    & 70.7  & 64.0   & 69.8    & 69.3 & 68.5    \\
\hline
InternVL-Chat-V1.5~\cite{chen2024far}      & 46.6   & 66.8    & 37.4  & 38.5  & 58.0 & 50.3  & 49.6    & 66.0  & 49.4   & 56.6    & 67.9 & 60.0    \\
InternVL2-26B~\cite{chen2024far}           & 56.2   & 69.6    & 42.6  & 50.6  & 60.6 & 53.7  & 55.6    & 68.3  & 58.7   & 62.2    & 70.1 & 64.8    \\
InternVL2.5-26B~\cite{chen2024expanding}   & 61.8   & 75.6    & 49.4  & 61.1  & 66.9 & 55.7  & 61.8    & 74.5  & 61.8   & 65.2    & 72.9 & 68.6    \\
Cambrian-34B~\cite{tong2024cambrian}       & --     & --      & --    & --    & --   & --    & --      & 67.8  & 44.1   & --      & --   & --      \\
InternVL2-40B~\cite{chen2024far}           & 57.2   & 71.4    & 47.9  & 54.4  & 66.2 & 55.2  & 58.7    & 71.8  & 61.8   & 63.2    & 73.3 & 67.5    \\
InternVL2.5-38B~\cite{chen2024expanding}   & 63.2   & 78.3    & 55.3  & 62.7  & 70.0 & 61.2  & 65.1    & 73.5  & 64.0   & 66.4    & 72.1 & 69.0    \\
\rowcolor{gray!15}
InternVL3-38B                              & 64.0   & 77.9    & 57.4  & 63.8  & 71.8 & 62.3  & 66.2    & 75.6  & 67.3   & 71.6    & 73.3 & 72.0    \\
\hline
GPT-4V~\cite{gpt4v}                        & 54.6   & 62.7    & --    & 62.3  & 64.3 & 53.1  & --      & 61.4  & --     & 71.8    & 65.6 & --      \\
GPT-4o-20240513~\cite{gpt4v}               & 68.0   & --      & 55.7  & 68.0  & 65.4 & --    & --      & 75.4  & 45.2   & 80.6    & 77.7 & 69.7    \\
% Claude-3-Opus~\cite{claude3series2024}   & 44.1   & --      & --    & --    & --   & --    & --      & 49.8  & --     & 53.0    & --   & --      \\
Claude-3.5-Sonnet~\cite{claude3series2024} & --     & --      & 53.4  & --    & --   & --    & --      & 60.1  & 51.6   & --      & --   & --      \\
Gemini-1.5-Pro~\cite{reid2024gemini1_5}    & --     & --      & 53.4  & --    & 64.5 & --    & --      & 67.5  & 38.2   & --      & --   & --      \\
LLaVA-OneVision-72B~\cite{li2024llavaov}   & 55.4   & 77.6    & --    & 54.8  & --   & --    & --      & 71.9  & --     & --      & --   & --      \\
Qwen2-VL-72B~\cite{wang2024qwen2vl}        & --     & --      & --    & --    & 71.8 & --    & --      & 77.8  & --     & --      & --   & --      \\
Qwen2.5-VL-72B~\cite{bai2025qwen2}         & 64.4   & --      & --    & 70.7  & --   & --    & --      & 75.7  & 63.2   & --      & --   & --      \\
InternVL2-Llama3-76B~\cite{chen2024far}    & 56.8   & 73.7    & 44.2  & 51.2  & 67.4 & 58.2  & 58.6    & 72.2  & 63.0   & 65.8    & 74.1 & 68.8    \\
InternVL2.5-78B~\cite{chen2024expanding}   & 63.8   & 77.0    & 55.8  & 63.5  & 70.8 & 61.1  & 65.3    & 78.7  & 62.9   & 71.4    & 77.2 & 72.6    \\
\rowcolor{gray!15}
InternVL3-78B                              & 66.3   & 79.3    & 60.4  & 64.5  & 73.2 & 64.3  & 68.0    & 78.0  & 65.4   & 73.6    & 77.4 & 73.6    \\
% \rowcolor{gray!15}
% InternVL2.5-Pro                            &        &         &       &       &      &       &       &         &        &         &      &         \\
\end{tabular}
}
\caption{\textbf{Comparison of multi-image and real-world understanding performance. }
Multi-image benchmarks include BLINK~\cite{fu2024blink}, Mantis-Eval~\cite{jiang2024mantis}, MMIU~\cite{meng2024mmiu}, MuirBench~\cite{wang2024muirbench}, MMT-Bench~\cite{mmtbench}, and MIRB~\cite{zhao2024mirb}.
Real-world benchmarks encompass RealWorldQA~\cite{realworldqa}, MME-RealWorld~\cite{zhang2024mme}, WildVision~\cite{lu2024wildvision}, and R-Bench~\cite{li2024r}.
Part of the results are sourced from the benchmark papers and the OpenCompass leaderboard~\cite{opencompass2023}.
}
\label{tab:benchmark_multi_image_real_world}
\end{table*}

==> table/benchmark_multilingual.tex <==
\begin{table*}[t!]
\scriptsize
\centering
\renewcommand{\arraystretch}{0.95}
{\fontsize{8}{10}\selectfont 
\setlength\tabcolsep{4.2pt}
\newcommand{\MMMB}{\makecell{MMMB}}
\newcommand{\MultiMMB}{\makecell{Multilingual MMBench}}
\begin{tabular}{l|cccccc|cccccc|c|c}
\multirow{2}{*}{Model Name}               & \multicolumn{6}{c|}{\MMMB}              & \multicolumn{6}{c|}{\MultiMMB}          & MTVQA   & \multirow{2}{*}{Overall} \\
                                          & en   & zh   & pt   & ar   & tr   & ru   & en   & zh   & pt   & ar   & tr   & ru   & (avg)   &                          \\
\hline
InternVL2-1B~\cite{chen2024far}           & 73.2 & 67.4 & 55.5 & 53.5 & 43.8 & 55.2 & 67.9 & 61.2 & 50.8 & 43.3 & 31.8 & 52.7 & 12.6    & 40.7                     \\
InternVL2.5-1B~\cite{chen2024expanding}   & 78.8 & 70.2 & 61.5 & 55.0 & 45.3 & 61.1 & 72.5 & 64.7 & 57.0 & 43.0 & 37.8 & 53.2 & 21.4    & 46.0                     \\
\rowcolor{gray!15}
InternVL3-1B                              & 79.4 & 70.1 & 62.3 & 58.0 &	47.6 & 61.9 & 72.6 & 66.2 & 62.3 & 48.0 & 39.5 & 60.3 & 22.2    & 47.9                     \\
Qwen2-VL-2B~\cite{wang2024qwen2vl}        & 78.3 & 74.2 & 72.6 & 68.3 & 61.8 & 72.8 & 72.1 & 71.1 & 69.9 & 61.1 & 54.4 & 69.3 & 20.0    & 52.6                     \\
Qwen2.5-VL-3B~\cite{bai2025qwen2}         & --   & --   & --   & --   & --   & --   & --   & --   & --   & --   & --   & --   & 24.8    & --                       \\
InternVL2-2B~\cite{chen2024far}           & 79.4 & 71.6 & 54.0 & 43.5 & 46.4 & 48.1 & 73.8 & 69.6 & 51.4 & 29.8 & 31.3 & 42.3 & 10.9    & 39.3                     \\
InternVL2.5-2B~\cite{chen2024expanding}   & 81.4 & 74.4 & 58.2 & 48.3 & 46.4 & 53.2 & 76.5 & 71.6 & 55.9 & 37.3 & 33.9 & 44.8 & 21.8    & 45.2                     \\
\rowcolor{gray!15}
InternVL3-2B                              & 81.9 & 78.3 & 75.4 & 68.6 & 62.9 & 74.6 & 81.3 & 77.8 & 75.9 & 66.4 & 59.5 & 70.7 & 26.7    & 57.4                     \\
% \hline
% InternVL2-4B~\cite{chen2024far}           & 82.0 & 76.1 & 75.6 & 54.3 & 51.2 & 67.4 & 77.3 & 72.4 & 72.6 & 43.6 & 46.5 & 61.2 & 15.3    & 48.4                     \\
% \rowcolor{gray!15}
% InternVL2.5-4B                            & 83.7 & 81.0 & 79.7 & 76.0 & 70.5 & 79.9 & 82.3 & 81.1 & 78.9 & 73.4 & 68.1 & 76.2 & 28.4    & 61.2                     \\
\hline
mPLUG-Owl2~\cite{ye2023mplug2}            & 67.3 & 61.0 & 59.7 & 45.8 & 45.4 & 62.6 & 66.2 & 59.4 & 58.2 & 37.9 & 47.7 & 60.4 & --      & --                       \\
Qwen2-VL-7B~\cite{wang2024qwen2vl}        & 83.9 & 82.4 & 81.2 & 79.0 & 74.7 & 82.4 & 81.8 & 81.6 & 79.1 & 75.6 & 74.5 & 79.3 & 25.6    & 61.6                     \\
Qwen2.5-VL-7B~\cite{bai2025qwen2}         & --   & --   & --   & --   & --   & --   & --   & --   & --   & --   & --   & --   & 29.2    & --                       \\
InternVL2-8B~\cite{chen2024far}           & 83.4 & 81.5 & 76.1 & 66.3 & 69.2 & 75.7 & 82.9 & 81.8 & 76.0 & 60.5 & 66.0 & 74.4 & 20.9    & 56.6                     \\ 
InternVL2.5-8B~\cite{chen2024expanding}   & 84.3 & 83.1 & 78.6 & 69.3 & 71.5 & 79.5 & 83.8 & 83.2 & 79.4 & 64.3 & 67.8 & 77.3 & 27.6    & 60.4                     \\
\rowcolor{gray!15}
InternVL3-8B                              & 85.1 & 83.1 & 82.5 & 81.6 & 76.2 & 83.4 & 85.5 & 85.6 &	83.2 & 79.2 & 75.9 & 82.6 & 30.2    & 64.7                     \\
\rowcolor{gray!15}
InternVL3-9B                              & 84.8 & 83.7 & 80.6 & 69.9 & 68.5 & 80.8 & 86.5 & 85.2 & 79.1 & 64.3 & 68.3 & 79.1 & 27.1    & 60.7                     \\
\rowcolor{gray!15}
InternVL3-14B                             & 85.7 & 84.7 & 83.1 & 83.7 &	79.3 & 83.6 & 86.7 & 85.8 & 83.2 & 81.1 & 80.7 & 83.8 & 31.6    & 66.2                     \\
\hline
InternVL-Chat-V1.5~\cite{chen2024far}     & 82.6 & 80.8 & 76.3 & 65.2 & 68.6 & 74.0 & 81.1 & 80.2 & 76.9 & 56.2 & 66.7 & 71.0 & 20.5    & 55.7                     \\
InternVL2-26B~\cite{chen2024far}          & 83.8 & 81.7 & 78.0 & 68.8 & 69.3 & 76.3 & 82.7 & 81.8 & 77.8 & 61.9 & 69.6 & 74.4 & 17.7    & 56.2                     \\
InternVL2.5-26B~\cite{chen2024expanding}  & 86.2 & 83.8 & 81.6 & 73.3 & 73.7 & 82.8 & 86.1 & 85.5 & 80.7 & 67.5 & 75.0 & 79.6 & 28.5    & 62.6                     \\
InternVL2-40B~\cite{chen2024far}          & 85.3 & 84.1 & 81.1 & 70.3 & 74.2 & 81.4 & 86.2 & 85.8 & 82.8 & 64.0 & 74.2 & 81.8 & 20.6    & 59.7                     \\
InternVL2.5-38B~\cite{chen2024expanding}  & 86.4 & 85.1 & 84.1 & 84.3 & 82.8 & 84.9 & 87.5 & 88.6 & 85.3 & 84.5 & 84.0 & 85.9 & 31.7    & 67.4                     \\
\rowcolor{gray!15}
InternVL3-38B                             & 86.7 & 85.6 & 84.5 & 84.8 &	82.6 & 85.1 & 89.0 & 89.3 & 87.1 & 84.6 & 84.3 & 87.4 & 32.4    & 68.1                     \\
\hline
GPT-4V~\cite{gpt4v}                       & 75.0 & 74.2 & 71.5 & 73.5 & 69.0 & 73.1 & 77.6 & 74.4 & 72.5 & 72.3 & 70.5 & 74.8 & 22.0    & 56.1                     \\
GPT-4o~\cite{gpt4v}                       & --   & --   & --   & --   & --   & --   & --   & --   & --   & --   & --   & --   & 27.8    & --                       \\
% Qwen-VL-Max~\cite{bai2023qwenvl}        & 77.2 & 75.3 & 72.2 & 70.8 & 66.0 & 74.2 & 76.8 & 77.6 & 74.6 & 75.0 & 69.1 & 75.0 & --      & --                       \\
Gemini-1.0-Pro~\cite{team2023gemini}      & 75.0 & 71.9 & 70.6 & 69.9 & 69.6 & 72.7 & 73.6 & 72.1 & 70.3 & 61.1 & 69.8 & 70.5 & --      & --                       \\
Qwen2-VL-72B~\cite{wang2024qwen2vl}       & 86.8 & 85.3 & 85.2 & 84.8 & 84.2 & 85.3 & 86.9 & 87.2 & 85.8 & 83.5 & 84.4 & 85.3 & 30.9    & 67.2                     \\
Qwen2.5-VL-72B~\cite{bai2025qwen2}        & --   & --   & --   & --   & --   & --   & --   & --   & --   & --   & --   & --   & 31.7    & --                       \\
InternVL2-Llama3-76B~\cite{chen2024far}   & 85.3 & 85.1 & 82.8 & 82.8 & 83.0 & 83.7 & 87.8 & 87.3 &	85.9 & 83.1 & 85.0 & 85.7 & 22.0    & 63.9                     \\
InternVL2.5-78B~\cite{chen2024expanding}  & 86.3 & 85.6 & 85.1 & 84.8 & 83.1 & 85.4 & 90.0 & 89.7 & 87.4 & 83.3 & 84.9 & 86.3 & 31.9    & 68.0                     \\
\rowcolor{gray!15}
InternVL3-78B                             & 87.2 & 86.6 & 85.5 & 86.5 & 84.6 & 86.1 & 89.4 & 90.3 &	88.7 & 86.1 & 86.6 & 88.1 & 32.5    & 68.9                     \\
% \rowcolor{gray!15}
% InternVL2.5-Pro                         &      &      &      &      &      &      &      &      &      &      &      &      &         & --                       \\
\end{tabular}
}
\caption{\textbf{Comparison of multimodal multilingual performance. }
We evaluate multilingual capabilities across 3 benchmarks, including MMMB~\cite{sun2024parrot}, Multilingual MMBench~\cite{sun2024parrot} and MTVQA~\cite{tang2024mtvqa}.
The languages evaluated are English (en), Chinese (zh), Portuguese (pt), Arabic (ar), Turkish (tr), and Russian (ru).
}
\label{tab:benchmark_multilingual}
\end{table*}



==> table/benchmark_multimodal_hallucination.tex <==
\begin{table*}[t!]
\centering
\renewcommand{\arraystretch}{0.95}
{\fontsize{7.5}{10}\selectfont 
\setlength\tabcolsep{1.5pt}
\newcommand{\MME}{\makecell{MME\\(sum)}}
\newcommand{\MMB}{\makecell{MMB\\(EN / CN)}}
\newcommand{\MMBV}{\makecell{MMBv1.1\\(EN)}}
\newcommand{\MMVet}{\makecell{MMVet\\(turbo)}}
\newcommand{\MMVetV}{\makecell{MMVetv2\\(0613)}}
\newcommand{\MMStar}{\makecell{MMStar}}
\newcommand{\POPE}{\makecell{POPE\\(avg)}}
\newcommand{\HallB}{\makecell{HallBench\\(avg)}}
\newcommand{\AMBER}{\makecell{AMBER\\(generative / discriminative / overall)}}
\newcommand{\ObjectHalBench}{\makecell{ObjectHal}}
\newcommand{\MMHal}{\makecell{MMHal\\(score)}}
\newcommand{\CRPE}{\makecell{CRPE\\(relation)}}
\begin{tabular}{l|ccccccc|ccccc}
Model Name                                & \MME   & \MMB        & \MMBV & \MMVet & \MMVetV & \MMStar & Overall & \HallB & \MMHal & \CRPE & \POPE & Overall \\
\hline
LLaVA-OneVision-0.5B~\cite{li2024llavaov} & 1438.0 & 61.6 / 55.5 & 59.6  & 32.2   & --      & 37.7    & --      & 27.9   & --     & --    & --    & --      \\
InternVL2-1B~\cite{chen2024far}           & 1794.4 & 65.4 / 60.7 & 61.6  & 32.7   & 36.1    & 45.7    & 51.7    & 34.0   & 2.25   & 57.5  & 87.3  & 45.3    \\
InternVL2.5-1B~\cite{chen2024expanding}   & 1950.5 & 70.7 / 66.3 & 68.4  & 48.8   & 43.2    & 50.1    & 58.9    & 39.0   & 2.49   & 60.9  & 89.9  & 48.1    \\
\rowcolor{gray!15}
InternVL3-1B                              & 1934.4 & 72.6 / 67.9 & 69.9  & 59.5   &  47.5   & 51.5    & 61.9    & 41.4   & 2.59   & 64.0  & 90.7  & 49.7    \\
Qwen2-VL-2B~\cite{wang2024qwen2vl}        & 1872.0 & 74.9 / 73.5 & 72.2  & 49.5   & --      & 48.0    & --      & 41.7   & --     & --    & --    & --      \\
Qwen2.5-VL-3B~\cite{bai2025qwen2}         &   2157 & 79.1 / 78.1 & 77.4  &  61.8  & --      & 55.9    & --      & 46.3   & --     & 73.6  & --    & --      \\
InternVL2-2B~\cite{chen2024far}           & 1876.8 & 73.2 / 70.9 & 70.2  & 39.5   & 39.6    & 50.1    & 58.0    & 37.9   & 2.52   & 66.3  & 88.3  & 48.8    \\
InternVL2.5-2B~\cite{chen2024expanding}   & 2138.2 & 74.7 / 71.9 & 72.2  & 60.8   & 52.3    & 53.7    & 65.3    & 42.6   & 2.94   & 70.2  & 90.6  & 51.6    \\
\rowcolor{gray!15}
InternVL3-2B                              & 2221.2 & 81.1 / 78.4 & 78.6  & 62.2   & 53.9    & 60.7    & 69.8    & 42.5   & 3.26   & 71.5  & 89.6  & 51.7    \\
\hline
Qwen2-VL-7B~\cite{wang2024qwen2vl}        & 2326.8 & 83.0 / 80.5 & 80.7  & 62.0   & --      & 60.7    & --      & 50.6   & 3.40   & 74.4  & 88.1  & 54.1    \\
Qwen2.5-VL-7B~\cite{bai2025qwen2}         & 2347   & 83.5 / 83.4 & 82.6  &  67.1  & --      & 63.9    & --      & 52.9   & --     & 76.4  & --    & --      \\
MiniCPM-V2.6~\cite{yao2024minicpm}        & 2348.4 & 81.5 / 79.3 & 78.0  & 60.0   & --      & 57.5    & --      & 48.1   & 3.60   & 75.2  & 87.3  & 53.6    \\
InternVL2-8B~\cite{chen2024far}           & 2210.3 & 81.7 / 81.2 & 79.5  & 54.2   & 52.3    & 62.0    & 69.2    & 45.2   & 3.33   & 75.8  & 86.9  & 52.8    \\
InternVL2.5-8B~\cite{chen2024expanding}   & 2344.1 & 84.6 / 82.6 & 83.2  & 62.8   & 58.1    & 62.8    & 73.2    & 50.1   & 3.65   & 78.4  & 90.6  & 55.7    \\
\rowcolor{gray!15}
InternVL3-8B                              & 2415.4 & 83.4 / 82.2 & 81.7  & 81.3   & 66.3    & 68.2    & 77.7    & 49.9   & 3.61   & 76.3  & 91.1  & 55.2    \\
\rowcolor{gray!15}
InternVL3-9B                              & 2372.8 & 83.4 / 82.2 & 81.7  & 76.2   & 65.4    & 66.3    & 76.3    & 51.2   & 3.47   & 75.0  & 90.4  & 55.0    \\
\rowcolor{gray!15}
InternVL3-14B                             & 2478.3 & 85.6 / 84.1 & 83.5  & 80.2   & 68.4    & 68.8    & 79.0    & 55.1   & 3.49   & 77.3  & 90.2  & 56.5    \\
\hline
InternVL-Chat-V1.5~\cite{chen2024far}     & 2194.2 & 82.2 / 82.0 & 80.3  & 61.5   & 51.5    & 57.3    & 69.7    & 50.3   & 3.11   & 75.4  & 88.4  & 54.3    \\
InternVL2-26B~\cite{chen2024far}          & 2260.7 & 83.4 / 82.0 & 81.5  & 62.1   & 57.2    & 61.2    & 71.8    & 50.7   & 3.55   & 75.6  & 88.0  & 54.5    \\
InternVL2.5-26B~\cite{chen2024expanding}  & 2373.3 & 85.4 / 85.5 & 84.2  & 65.0   & 60.8    & 66.5    & 75.2    & 55.0   & 3.70   & 79.1  & 90.6  & 57.1    \\
Cambrian-34B~\cite{tong2024cambrian}      & --     & 80.4 / 79.2 & 78.3  & 53.2   & --      & 54.2    & --      & 41.6   & --     & --    & --    & --      \\
InternVL2-40B~\cite{chen2024far}          & 2307.5 & 86.8 / 86.5 & 85.1  & 65.5   & 63.8    & 65.4    & 75.7    & 56.9   & 3.75   & 77.6  & 88.4  & 56.7    \\
InternVL2.5-38B~\cite{chen2024expanding}  & 2455.8 & 86.5 / 86.3 & 85.5  & 68.8   & 62.1    & 67.9    & 77.0    & 56.8   & 3.71   & 78.3  & 90.7  & 57.4    \\
\rowcolor{gray!15}
InternVL3-38B                             & 2523.6 & 87.6 / 86.8 & 86.9 & 83.9   & 69.6    & 71.5    & 81.5    & 57.1   & 3.77   & 77.1  & 90.6  & 57.1    \\
\hline
GPT-4V~\cite{gpt4v}                       & 1926.6 & 81.0 / 80.2 & 80.0  & 67.5   & 66.3    & 56.0    & 70.7    & 46.5   & --     & --    & --    & --      \\
GPT-4o-20240513~\cite{gpt4v}              & --     & 83.4 / 82.1 & 83.1  & 69.1   & 71.0    & 64.7    & --      & 55.0   & 4.00   & 76.6  & 86.9  & 55.6    \\
Claude-3-Opus~\cite{claude3series2024}    & 1586.8 & 63.3 / 59.2 & 60.1  & 51.7   & 55.8    & 45.7    & 55.5    & 37.8   & --     & --    & --    & --      \\
Claude-3.5-Sonnet~\cite{claude3series2024}& --     & 82.6 / 83.5 & 80.9  & 70.1   & 71.8    & 65.1    & --      & 55.5   & --     & --    & --    & --      \\
Gemini-1.5-Pro~\cite{reid2024gemini1_5}   & --     & 73.9 / 73.8 & 74.6  & 64.0   & 66.9    & 59.1    & --      & 45.6   & --     & --    & --    & --      \\
LLaVA-OneVision-72B~\cite{li2024llavaov}  & 2261.0 & 85.8 / 85.3 & 85.0  & 60.6   & --      & 65.8    & --      & 49.0   & --     & --    & --    & --      \\
Qwen2-VL-72B~\cite{wang2024qwen2vl}       & 2482.7 & 86.5 / 86.6 & 85.9  & 74.0   & 66.9    & 68.3    & 78.7    & 58.1   & --     & --    & --    & --      \\
Qwen2.5-VL-72B~\cite{bai2025qwen2}        & 2448.0 & 88.6 / 87.9 & 88.4  & 76.2   & --      & 70.8    & --      & 55.2   & --     & 79.2  & --    & --      \\
InternVL2-Llama3-76B~\cite{chen2024far}   & 2414.7 & 86.5 / 86.3 & 85.5  & 65.7   & 68.4    & 67.4    & 77.2    & 55.2   & 3.83   & 77.6  & 89.0  & 56.4    \\
InternVL2.5-78B~\cite{chen2024expanding}  & 2494.5 & 88.3 / 88.5 & 87.4  & 72.3   & 65.5    & 69.5    & 79.2    & 57.4   & 3.89   & 78.8  & 90.8  & 57.7    \\
\rowcolor{gray!15}
InternVL3-78B                             & 2549.8 & 89.0 / 88.7 & 87.7  & 81.3   & 70.0    & 72.5    & 82.0    & 59.1   & 3.85   & 79.2  & 90.3  & 58.1    \\
% \rowcolor{gray!15}
% InternVL2.5-Pro                           &        &             &       &        &         &         &         &        &        &       &       &         \\
\end{tabular}
}

\caption{\textbf{Comparison of comprehensive multimodal understanding and hallucination performance.}
Comprehensive multimodal benchmarks include MME~\cite{fu2023mme}, MMBench series~\cite{liu2023mmbench}, MMVet series~\cite{yu2023mmvet, yu2024mmvetv2}, and MMStar~\cite{chen2024mmstar}.
Hallucination benchmarks encompass HallusionBench~\cite{guan2023hallusionbench}, MMHal~\cite{sun2023aligning}, CRPE~\cite{wang2024allseeingv2}, and POPE~\cite{li2023pope}.
Part of the results are sourced from the benchmark papers and the OpenCompass leaderboard~\cite{opencompass2023}.
}
\label{tab:benchmark_multimodal_hallucination}
\end{table*}


==> table/benchmark_ocr.tex <==
\begin{table*}[t!]
\centering
{\fontsize{8}{10}\selectfont 
\renewcommand{\arraystretch}{0.95}
\setlength\tabcolsep{1.5pt}
\newcommand{\TextVQA}{\makecell{TextVQA\\(val)}}
\newcommand{\ChartQA}{\makecell{ChartQA\\(test avg)}}
\newcommand{\DocVQA}{\makecell{DocVQA\\(test)}}
\newcommand{\InfoVQA}{\makecell{InfoVQA\\(test)}}
\newcommand{\TableVQA}{\makecell{TableVQA\\Bench}}
\newcommand{\CharXiv}{\makecell{CharXiv\\(RQ / DQ)}}
\newcommand{\SEEDTP}{\makecell{SEED-2\\Plus}}
\newcommand{\VCREN}{\makecell{VCR-EN-Easy\\(EM / Jaccard)}}
\newcommand{\VCRZH}{\makecell{VCR-ZH\\(EM/Jaccard)}}
\newcommand{\OCRBench}{\makecell{OCR\\Bench}}
\newcommand{\AITD}{\makecell{AI2D\\(w / wo M)}}
\newcommand{\lsp}{--\ \ \ \ \ \ }
\newcommand{\rsp}{\ \ \ \ \ --~}
\newcommand{\TODO}{\textcolor{red}{TODO}}
\newcommand{\newicon}{\includegraphics[height=1em]{figure/new.pdf}}
\begin{tabular}{l|cccccccccc}
Model Name                                 & \AITD       & \ChartQA & \TextVQA & \DocVQA & \InfoVQA & \OCRBench & \SEEDTP & \CharXiv    & \VCREN       & Overall \\
\hline
LLaVA-OneVision-0.5B~\cite{li2024llavaov}  & 57.1 / \lsp & 61.4     & --       & 70.0    & 41.8     & 565       & --      & --          & --           & --      \\
InternVL2-1B~\cite{chen2024far}            & 64.1 / 70.5 & 72.9     & 70.5     & 81.7    & 50.9     & 754       & 54.3    & 18.1 / 30.7 & 21.5 / 48.4  & 54.9    \\
InternVL2.5-1B~\cite{chen2024expanding}    & 69.3 / 77.8 & 75.9     & 72.0     & 84.8    & 56.0     & 785       & 59.0    & 19.0 / 38.4 & 91.5 / 97.0  & 68.3    \\
\rowcolor{gray!15}
InternVL3-1B                               & 69.4 / 78.3 & 75.3     & 74.1     & 81.9    & 53.7     & 790       & 58.2    & 21.0 / 47.1 & 89.3 / 96.2  & 68.6    \\
% \hline
Qwen2-VL-2B~\cite{wang2024qwen2vl}         & 74.7 / 84.6 & 73.5     & 79.7     & 90.1    & 65.5     & 809       & 62.4    & --          & 81.5 / \lsp  & --      \\
Qwen2.5-VL-3B~\cite{bai2025qwen2_5}        & 81.6 / \lsp & 84.0     & 79.3     & 93.9    & 77.1     & 797       & 67.6    & 31.3 / 58.6 & --           & --      \\
Aquila-VL-2B~\cite{gu2024aquilavl}         & 75.0 / \lsp & 76.5     & 76.4     & 85.0    & 58.3     & 772       & 63.0    & --          & 70.0 / \lsp  & --      \\
InternVL2-2B~\cite{chen2024far}            & 74.1 / 82.3 & 76.2     & 73.4     & 86.9    & 58.9     & 784       & 60.0    & 21.0 / 40.6 & 32.9 / 59.2  & 62.0    \\
InternVL2.5-2B~\cite{chen2024expanding}    & 74.9 / 83.5 & 79.2     & 74.3     & 88.7    & 60.9     & 804       & 60.9    & 21.3 / 49.7 & 93.2 / 97.6  & 72.1    \\
\rowcolor{gray!15}
InternVL3-2B                               & 78.7 / 87.4 & 80.2     & 77.0     & 88.3    & 66.1     & 835       & 64.6    & 28.3 / 54.7 & 91.2 / 96.9  & 74.7    \\
\hline
% Phi-3.5-Vision-4B~\cite{abdin2024phi3}     & 77.8 / 87.6 & 81.8     & 72.0     & 69.3    & 36.6     & 599       & 62.2    & --          & 39.3 / 60.4  & --       \\
% Mini-InternVL-4B-V1.5~\cite{gao2024mini}   & 76.9 / 86.6 & 81.0     & 72.5     & 87.7    & 64.6     & 638       & 62.6    & --          & 19.0 / 47.8  & --       \\
% InternVL2-4B~\cite{chen2024far}            & 78.9 / 87.8 & 81.5     & 74.4     & 89.2    & 67.0     & 788       & 63.9    & 24.5 / 48.0 & 33.7 / 61.1  & 65.7     \\
% InternVL2.5-4B                             & 81.4 / 90.5 & 84.0     & 76.8     & 91.6    & 72.1     & 828       & 66.9    & 24.9 / 61.7 & 93.7 / 97.8  & 77.0     \\
% \rowcolor{gray!15}
% InternVL3-4B                               &  /          &          &          &         &          &           &         &             &              &          \\
% \hline
Ovis1.6-Gemma2-9B~\cite{lu2024ovis}        & 84.4 / \lsp & --       & --       & --      & --       & 830       & --      & --          & --           & --      \\
MiniCPM-V2.6~\cite{yao2024minicpm}         & 82.1 / \lsp & 82.4     & 80.1     & 90.8    & --       & 852       & 65.7    & 31.0 / 57.1 & 73.9 / 85.7  & --      \\
Molmo-7B-D~\cite{deitke2024molmo}          & \rsp / 93.2 & 84.1     & 81.7     & 92.2    & 72.6     & 694       & --      & --          & --           & --      \\
Qwen2-VL-7B~\cite{wang2024qwen2vl}         & 83.0 / 92.1 & 83.0     & 84.3     & 94.5    & 76.5     & 866       & 69.0    & --          & 89.7 / 93.8  & --      \\
Qwen2.5-VL-7B~\cite{bai2025qwen2_5}        & 83.9 / \lsp & 87.3     & 84.9     & 95.7    & 82.6     & 864       & 70.4    & 42.5/73.9   & --           & --      \\
InternVL2-8B~\cite{chen2024far}            & 83.8 / 91.7 & 83.3     & 77.4     & 91.6    & 74.8     & 794       & 67.5    & 31.2 / 56.1 & 37.9 / 61.5  & 69.7    \\
InternVL2.5-8B~\cite{chen2024expanding}    & 84.5 / 92.8 & 84.8     & 79.1     & 93.0    & 77.6     & 822       & 69.7    & 32.9 / 68.6 & 92.6 / 97.4  & 79.6    \\
\rowcolor{gray!15}
InternVL3-8B                               & 85.2 / 92.6 & 86.6     & 80.2     & 92.7    & 76.8     & 880       & 69.7    & 37.6 / 73.6 & 94.5 / 98.1  & 81.3    \\
\rowcolor{gray!15}
InternVL3-9B                               & 84.6 / 92.9 & 86.2     & 79.4     & 93.6    & 79.6     & 877       & 68.8    & 38.0 / 72.5 & 94.2 / 97.9  & 81.3    \\
\rowcolor{gray!15}
InternVL3-14B                              & 86.0 / 93.7 & 87.3     & 80.5     & 94.1    & 83.6     & 875       & 70.3    & 43.1 / 82.2 & 94.8 / 98.2  & 83.4    \\
\hline
InternVL-Chat-V1.5~\cite{chen2024far}      & 80.7 / 89.8 & 83.8     & 80.6     & 90.9    & 72.5     & 724       & 66.3    & 29.2 / 58.5 & 14.7 / 51.4  & 65.9    \\
InternVL2-26B~\cite{chen2024far}           & 84.5 / 92.5 & 84.9     & 82.3     & 92.9    & 75.9     & 825       & 67.6    & 33.4 / 62.4 & 74.5 / 86.7  & 76.7    \\
InternVL2.5-26B~\cite{chen2024expanding}   & 86.4 / 94.4 & 87.2     & 82.4     & 94.0    & 79.8     & 852       & 70.8    & 35.9 / 73.5 & 94.4 / 98.0  & 81.8    \\
Qwen2.5-VL-32B~\cite{bai2025qwen2_5}       & --          & --       & --       & 94.8    & 83.4     & --        & --      & --          & --           & --      \\
Cambrian-34B~\cite{tong2024cambrian}       & 79.5 / \lsp & 75.6     & 76.7     & 75.5    & 46.0     & 600       & --      & 27.3 / 59.7 & 79.7 / 89.3  & --      \\
VILA-1.5-40B~\cite{lin2024vila}            & 69.9 / \lsp & 67.2     & 73.6     & --      & --       & 460       & --      & 24.0 / 38.7 & --           & --      \\
InternVL2-40B~\cite{chen2024far}           & 86.6 / 94.5 & 86.2     & 83.0     & 93.9    & 78.7     & 837       & 69.2    & 32.3 / 66.0 & 84.7 / 92.6  & 79.3    \\
InternVL2.5-38B~\cite{chen2024expanding}   & 87.6 / 95.1 & 88.2     & 82.7     & 95.3    & 83.6     & 842       & 71.2    & 42.4 / 79.6 & 94.7 / 98.2  & 83.6    \\
\rowcolor{gray!15}
InternVL3-38B                              & 88.9 / 95.5 & 89.2     & 83.9     & 95.4    & 85.0     & 886       & 71.6    & 46.4 / 87.2 & 96.1 / 98.7  & 85.5    \\
\hline
% GPT-4o-Mini~\cite{gpt4v}                 & 77.8 / --   & --       & --       & --      & --       & 785       & --      & 34.1 / 74.9 & 83.6 / 87.8  & --      \\
GPT-4V~\cite{gpt4v}                        & 78.2 / 89.4 & 78.5     & 78.0     & 88.4    & 75.1     & 645       & 53.8    & 37.1 / 79.9 & 52.0 / 65.4  & 70.0    \\
GPT-4o-20240513~\cite{gpt4v}               & 84.6 / 94.2 & 85.7     & 77.4     & 92.8    & 79.2     & 736       & 72.0    & 47.1 / 84.5 & 91.6 / 96.4  & 81.6    \\
% Claude-3-Sonnet~\cite{claude3series2024} & 69.9 / 88.7 & 81.1     & --       & 89.5    & --       & 646       & --      & 32.2 / 73.7 & --           & --      \\
Claude-3-Opus~\cite{claude3series2024}     & 70.6 / 88.1 & 80.8     & 67.5     & 89.3    & 55.6     & 694       & 44.2    & 30.2 / 71.6 & 62.0 / 77.7  & 67.3    \\
Claude-3.5-Sonnet~\cite{claude3series2024} & 81.2 / 94.7 & 90.8     & 74.1     & 95.2    & 74.3     & 788       & 71.7    & 60.2 / 84.3 & 63.9 / 74.7  & 78.7    \\
Gemini-1.5-Pro~\cite{reid2024gemini1_5}    & 79.1 / 94.4 & 87.2     & 78.8     & 93.1    & 81.0     & 754       & --      & 43.3 / 72.0 & 62.7 / 77.7  & --      \\
% Llama3-V-70B~\cite{dubey2024llama3}      & \rsp / 93.0 & 83.2     & 83.4     & 92.2    & --       & --        & --      & --          & --           & --      \\
LLaVA-OneVision-72B~\cite{li2024llavaov}   & 85.6 / \lsp & 83.7     & 80.5     & 91.3    & 74.9     & 741       & --      & --          & --           & --      \\
NVLM-D-72B~\cite{dai2024nvlm}              & 85.2 / 94.2 & 86.0     & 82.1     & 92.6    & --       & 853       & --      & --          & --           & --      \\
Molmo-72B~\cite{deitke2024molmo}           & \rsp / 96.3 & 87.3     & 83.1     & 93.5    & 81.9     & --        & --      & --          & --           & --      \\
Qwen2-VL-72B~\cite{wang2024qwen2vl}        & 88.1 / \lsp & 88.3     & 85.5     & 96.5    & 84.5     & 877       & --      & --          & 91.3 / 94.6  & --      \\
Qwen2.5-VL-72B~\cite{bai2025qwen2_5}       & 88.7 / \lsp & 89.5     & 83.5     & 96.4    & 87.3     & 885       & 73.0    & 49.7 / 87.4 & --           & --      \\
InternVL2-Llama3-76B~\cite{chen2024far}    & 87.6 / 94.8 & 88.4     & 84.4     & 94.1    & 82.0     & 839       & 69.7    & 38.9 / 75.2 & 83.2 / 91.3  & 81.1    \\
InternVL2.5-78B~\cite{chen2024expanding}   & 89.1 / 95.7 & 88.3     & 83.4     & 95.1    & 84.1     & 854       & 71.3    & 42.4 / 82.3 & 95.7 / 94.5  & 83.9    \\
\rowcolor{gray!15}
InternVL3-78B                              & 89.7 / 96.0 & 89.7     & 84.3     & 95.4    & 86.5     & 906       & 71.9    & 46.0 / 85.1 & 96.0 / 98.6  & 85.8    \\
% \rowcolor{gray!15}
% InternVL2.5-Pro                          &             &          &          &         &          &           &         &             &              & --      \\
\end{tabular}
}
\caption{\textbf{Comparison of OCR, chart, and document understanding performance.} We evaluate OCR-related capabilities across 9 benchmarks, including AI2D~\cite{kembhavi2016ai2d}, ChartQA~\cite{masry2022chartqa}, TextVQA~\cite{singh2019textvqa}, DocVQA~\cite{mathew2021docvqa}, InfoVQA~\cite{mathew2022infographicvqa}, OCRBench~\cite{liu2023ocrbench}, SEED-2-Plus~\cite{li2024seedbench2plus}, CharXiv~\cite{wang2024charxiv}, and VCR~\cite{zhang2024vcr}.
Part of results are collected from \cite{dubey2024llama3, deitke2024molmo, claude3series2024, wang2024charxiv, zhang2024vcr} and the OpenCompass leaderboard~\cite{opencompass2023}.
}
\vspace{-0.5em}
\label{tab:benchmark_ocr}
\end{table*}


==> table/benchmark_python_coding.tex <==

% \begin{table*}[!thb]
% \centering

% \resizebox{0.9\linewidth}{!}{
% \tablestyle{10pt}{1.2}
% \begin{tabular}{l|cccc}
% \toprule
% {Models} & {HumanEval} & {HumanEval-X} & {MBPP}  & {MBPP-CN}   \\
% & {4-shot} & {5-shot} & {5-shot} & {0-shot} \\
% \multicolumn{5}{c}{\greencolor{{  $\leq 7$B Models}}} \\
% Llama2-7B   &  14.6  &  11.2  &  28.8  &  16.0  \\
% Mistral-7B-v0.1   &  27.4  &  28.5  &  47.5  &  35.0  \\
% Baichuan2-7B-Base   &  22.0  &  16.1  &  35.0  &  23.2  \\
% Qwen-7B-Chat &  36.0  &  24.4  &  33.9  &  27.0 \\
% ChatGLM3-6B-Base   &  45.1  &  38.3  &  {{68.9}}  &  {50.0}  \\
% \midrule
% InternLM2-7B   &  {56.1}  &  {39.6}  &  51.8  &  45.4  \\
% InternLM2-7B-Base   &  31.1  &  28.8  &  54.1  &  40.6  \\
% \multicolumn{5}{c}{\bluecolor{{ $13\sim 20$B Models}}} \\
% Llama2-13B   &  18.9  &  17.2  &  38.9  &  25.2  \\
% Mixtral-8x7B-v0.1   &  32.3  &  38.3  &  59.5  &  43.8  \\
% Baichuan2-13B-Base   &  23.2  &  19.5  &  44.0  &  30.6  \\
% Qwen-14B   &  30.5  &  31.0  &  52.9  &  41.0  \\
% \midrule
% InternLM2-20B   &  48.8  &  {{48.2}}  &  {63.0}  &  {{53.2}}  \\
% InternLM2-20B-Base   &  32.3  &  31.5  &  59.9  &  44.4  \\
% \bottomrule
% \end{tabular}}
% \caption{{Comparison of Base Models on Python Coding}. The model name in {bold} indicates the top performer, while an {underline} signifies the leading model within a similar parameter size group.}
% \label{tab:chat_code_results}
% \end{table*}

\begin{table*}[!t]
\centering

\resizebox{0.9\linewidth}{!}{
\tablestyle{10pt}{1.2}
\begin{tabular}{l|c|cccc|c}

\multirow{2}{*}{model name} & \multirow{2}{*}{\#param}   & {HumanEval} & {HumanEval-X} & {MBPP}  & {MBPP-CN}  & \multirow{2}{*}{avg.}  \\
& & (4-shot) & (5-shot) & (5-shot) & (0-shot) \\
% \multicolumn{6}{c}{\greencolor{{  $\leq 7$B Models}}} \\
\hline
Llama2-7B-Chat & 7B & 15.2  &  10.6  &  30.4  &  17.8 & 18.5\\
Llama2-13B-Chat & 13B & 8.5  &  12.9  &  19.8  &  22.2  & 15.9 \\

Mistral-7B-Instruct-v0.2  & 7.3B & 35.4  &  27.1  &  23.7  &  17.6 & 26.0 \\
Mixtral-8x7B-Instruct-v0.1 & 46.7B & 32.3  &  38.3  &  59.5  &  43.8 & 43.5 \\

Baichuan2-7B-Chat & 7B & 17.7  &  15.4  &  37.7  &  20.8 & 22.9  \\
Baichuan2-13B-Chat & 13B & 19.5  &  18.3  &  40.9  &  27.8 & 26.6 \\

Qwen-7B-Chat & 7B & 36.0  &  24.4  &  33.9  &  27.0 & 30.3 \\
Qwen-14B-Chat & 14B & 41.5  &  29.9  &  29.2  &  27.6 & 32.1  \\

ChatGLM3-6B & 6.2B & 53.1  &  17.6  &  {54.9}  &  38.2 & 41.0 \\
\hline
\rowcolor{gray!15}
InternLM2-Chat-7B-SFT & 7B & {61.6}  &  {{43.9}}  &  47.5  &  44.4  & 49.4 \\
\rowcolor{gray!15}
InternLM2-Chat-7B & 7B & 59.2  &  41.7  &  52.5  &  {46.4}  & {50.0} \\
\rowcolor{gray!15}
InternLM2-Chat-20B-SFT & 20B & 67.1  &  {42.0}  &  63.4  &  52.2 & 56.2  \\
\rowcolor{gray!15}
InternLM2-Chat-20B & 20B &  {{67.7}}  &  39.8  &  {{65.8}}  &  {{54.0}} & {56.8} \\
\end{tabular}}
\caption{\textbf{Comparison of chat models on python coding}.}
\label{tab:chat_code_results}
\end{table*}


==> table/benchmark_reasoning.tex <==
\begin{table}[!t]
    % \captionsetup{justification=centering}
\centering
\tablestyle{10pt}{1.2}
\begin{tabular}{l|c|ccc|c}
\multirow{2}{*}{model name} & \multirow{2}{*}{\#param} & {WinoGrande} & {HellaSwag} & {BBH} & \multirow{2}{*}{avg.} \\
& & (0-shot) & (0-shot) & (0-shot) \\
\hline
% \multicolumn{5}{c}{\purplecolor{{\ding{72}API Models}}} \\
GPT-3.5 & -- & 68.7 & 70.2 & 41.9 & 60.3\\
\hline
% \multicolumn{5}{c}{\greencolor{{$\triangle$ $\sim7B\ Models$}}} \\
Llama2-7B-Chat & 7B & 51.5 & 49.5 & 41.4 & 47.5\\
Llama2-13B-Chat & 13B & 50.8 & 57.0 & 49.7 & 52.5 \\

Mistral-7B-Instruct-v0.2 & 7.3B & 50.8 & 64.1 & 46.4 & 53.8\\
Mixtral-8x7B-Instruct-v0.1 & 46.7B & 60.9 & 80.3 & 57.3 & 66.2 \\

Baichuan2-7B-Chat & 7B & 49.9 & 36.4 & 35.9 & 40.7\\
Baichuan2-13B-Chat & 13B & 50.9 & 34.4 & 42.5 & 42.6 \\

Qwen-7B-Chat & 7B & 54.2 & 61.9 & 45.5 & 53.9 \\
Qwen-14B-Chat & 14B & 55.7 & 79.2 & 55.8 & 63.6 \\

ChatGLM3-6B & 6.2B & 61.7 & 73.1 & 56.0 & 63.6\\
\hline
\rowcolor{gray!15}
InternLM2-Chat-7B-SFT & 7B & 65.8 & {83.5} & 60.9 & {70.1} \\
\rowcolor{gray!15}
InternLM2-Chat-7B & 7B & {65.8} & 83.0 & {61.2} & 70.0 \\
\rowcolor{gray!15}
InternLM2-Chat-20B-SFT & 20B & {75.0} & {85.9} & 66.9 & 75.9\\
\rowcolor{gray!15}
InternLM2-Chat-20B & 20B & 74.8 & 85.8 & {68.3} & {76.3} \\
\end{tabular}
    \vspace{2mm}
    \caption{\textbf{Comparison of reasoning tasks.}}
    \label{tab:reasoning_result}
\end{table}


==> table/benchmark_sem_seg.tex <==
\begin{table*}[t!]
\centering
{\fontsize{8}{10}\selectfont 
\renewcommand{\arraystretch}{1.1}
\setlength\tabcolsep{5.2pt}
\begin{tabular}{l|ccc|ccc|ccc|cc}
                          & \multicolumn{3}{c|}{Linear Probing} & \multicolumn{3}{c|}{Head Tuning (UperNet)} & \multicolumn{3}{c|}{Full Tuning (UperNet)} &   &   \\

\multirow{-2}{*}{Model Name} & ADE20K & COCO & avg.                     & ADE20K & COCO & avg.                    & ADE20K & COCO & avg. & \multirow{-2}{*}{$\Delta_1$} & \multirow{-2}{*}{$\Delta_2$} \\
\hline
InternViT-6B-224px           & 47.2   & 42.8 & \cellcolor{gray!15}45.0  & 54.9   & 48.9 & \cellcolor{gray!15}51.9 & 58.9   & 51.6 & 55.3 & 6.9                          & 10.2                             \\
InternViT-6B-448px-V1.0      & 43.6   & 38.5 & \cellcolor{red!15}41.0 & 55.4   & 49.4 & \cellcolor{green!15}52.4  & 58.1   & 51.7 & 54.9 & 11.3                         & 13.9                             \\
InternViT-6B-448px-V1.2      & 40.7   & 36.1 & \cellcolor{red!15}38.4 & 55.2   & 48.8 & \cellcolor{green!15}52.0  & 58.8   & 51.7 & 55.2 & 13.6                         & 16.8                             \\
InternViT-6B-448px-V1.5      & 40.9   & 36.3 & \cellcolor{red!15}38.6 & 55.0   & 49.1 & \cellcolor{green!15}52.0  & 58.8   & 51.5 & 55.2 & 13.4                         & 16.6                             \\
InternViT-6B-448px-V2.5      & 39.4   & 35.6 & \cellcolor{red!15}37.5 & 55.4   & 49.7 & \cellcolor{green!15}52.6  & 58.6   & 51.8 & 55.2 & 15.1                         & 17.7                             \\
\end{tabular}
}
\caption{\textbf{Semantic segmentation performance across different versions of InternViT.}
The models are evaluated on ADE20K~\cite{zhou2017ade20k} and COCO-Stuff-164K~\cite{caesar2018cocostuff} using three configurations: linear probing, head tuning, and full tuning. The table shows the mIoU scores for each configuration and their averages. $\Delta_1$ represents the gap between head tuning and linear probing, while $\Delta_2$ shows the gap between full tuning and linear probing. A larger $\Delta$ value indicates a shift from simple linear features to more complex, nonlinear representations.
    }
\label{tab:benchmark_sem_seg}
\end{table*}


==> table/benchmark_spatial.tex <==
\begin{table*}[t!]
\centering
\renewcommand{\arraystretch}{0.95}
\setlength\tabcolsep{3pt}
{\fontsize{8}{10}\selectfont 
% \renewcommand{\arraystretch}{0.9}

\begin{tabular}{l|cccccccc|c}

Model Name                                        & Obj.count & Abs.Dist.& Obj.size & Room Size & Rel.Dist. & Rel.Dir.& Route Plan & Appr.Order &   Overall\\
\hline
% Baseline &   &   &    &       &     &    &      &    &    \\
% Chance Level(Random)  & --  & --  & --      & --    & 25.0   & 36.1     & 28.3    & 25.0  &  --  \\
% Chance Level(Frequency)  & 62.1  & 32.0   & 29.9      & 33.1    & 25.1   & 47.9     & 28.4    & 25.2  &  34.0  \\
% \hline
% % VSI-Bench(tiny) Perf. &   &   &    &       &     &    &      &    &    \\
% \dag Human Level & 94.3  & 47.0   & 60.4      & 45.9    & 94.7  & 95.8     & 95.8    & 100  &  79.2  \\
% \dag Gemini-1.5 Flash  & 50.8  & 33.6   & 56.5      & 45.2    & 48.0   & 39.8     & 32.7    & 59.2 &  45.7   \\
% \dag Gemini-1.5 Pro  & 49.6  & 28.8   & 58.6      & 49.4    & 46.0   & 48.1     & 42.0    & 68.0  &  48.8  \\
% \dag Gemini-2.0 Flash  & 52.4  & 30.6   & 66.7      & 31.8    & 56.0   & 46.3     & 24.5    & 55.1  &  45.4  \\
% \hline
% Propreitary Models(API) &   &   &    &       &     &    &      &    &    \\
GPT-4o~\cite{gpt4v}   & 46.2  & 5.3   & 43.8      & 38.2    & 37.0   & 41.3     & 31.5    & 28.5 &  34.0   \\
% Gemini-1.5 Flash  & 49.8  & 30.8   & 53.5      & 54.4    & 37.7   & 41.0     & 31.5    & 37.8  &  42.1  \\
Gemini-1.5 Pro~\cite{reid2024gemini1_5}  & 56.2  & 30.9   & 64.1      & 43.6    & 51.3   & 46.3     & 36.0    & 34.6  &  45.4  \\
\hline
% Open-source Models &   &   &    &       &     &    &      &    &    \\
% LongVILA-8B  & 29.1  & 9.1   & 16.7      & 0.0    & 29.6   & 30.7     & 32.5    & 25.5  &  21.6  \\
VILA-1.5-8B~\cite{lin2024vila}  & 17.4  & 21.8   & 50.3      & 18.8    & 32.1   & 34.8     & 31.0    & 24.8  &  28.9  \\
LongVA-7B~\cite{longva}  & 38.0  & 16.6   & 38.9      & 22.2   & 33.1   & 43.3     & 25.4    & 15.7  &  29.2  \\
LLaVA-NeXT-Video-7B~\cite{zhang2024llavanext}  & 48.5  & 14.0   & 47.8      & 24.2    & 43.5   & 42.4     & 34.0    & 30.6  &  35.6  \\
% LLaVA-OneVision-0.5B  & 46.1  & 28.4   & 15.4      & 28.3    & 28.9   & 36.9     & 34.5    & 5.8  &  28.0  \\
LLaVA-OneVision-7B~\cite{li2024llavaov}  & 47.7  & 20.2   & 47.4      & 12.3    & 42.5   & 35.2     & 29.4    & 24.4  &  32.4  \\
\rowcolor{gray!15}
InternVL3-8B  & 68.1  & 39.0   & 48.4      & 33.6   & 48.3   &   36.4   & 27.3    & 35.4  &  42.1  \\

% VILA-1.5-40B  & 22.4  & 24.8   & 48.7      & 22.7    & 40.5   & 25.7     & 31.5    & 32.9 &  31.2  \\
\rowcolor{gray!15}
InternVL3-38B &  71.7 & 50.2  & 46.1   & 41.7      & 53.5    & 38.6   & 28.9     & 60.7    & 48.9    \\
LLaVA-NeXT-Video-72B~\cite{zhang2024llavanext}   & 48.9  & 22.8   & 57.4      & 35.3    & 42.4   & 36.7     & 35.0    & 48.6  &  40.9  \\


LLaVA-OneVision-72B~\cite{li2024llavaov}  & 43.5  & 23.9   & 57.6      & 37.5    & 42.5   & 39.9     & 32.5    & 44.6  &  40.2  \\


\rowcolor{gray!15}
InternVL3-78B &  71.2 & 53.7  & 44.4   & 39.5      & 55.9    & 39.5   & 28.9     & 54.5    & 48.4    \\

% \rowcolor{gray!15}
% InternVL2.5-Pro                           &        &             &       &        &         &         &        &        &       &       \\
\end{tabular}
}
\caption{\textbf{Performance of InternVL3 and other models on VSI-Bench.}
}
\label{tab:vis_benchmark}
\end{table*}

==> table/benchmark_teval_cibench.tex <==

% \begin{table*}[!t]
%     \caption{{Main results of CIBench.} Tool, Exe, Num, Text, and Vis denote the tool call rate, executable rate, numeric accuracy, text score, and visualization score respectively. {bold} denotes the best score among the same model scale. \textit{Average is the mean of Num, Text, and Vis in two modes.}}
%     \label{tab:main_results}
%     \setlength{\tabcolsep}{6pt}
%     \renewcommand{\arraystretch}{1.1}
%     \centering
%     \resizebox{\textwidth}{!}{%
%     \begin{tabular}{l|cccccc|cccccc|c}
%     \toprule
%     \multirow{2}{*}{{Model}} & \multicolumn{6}{c|}{{\textsc{English}}} & \multicolumn{6}{c|}{{\textsc{Chinese}}} & \multirow{2}{*}{AVG}} \\ 
%     % \cline{2-13}
%     % & \multicolumn{2}{c}{{\textsc{Round Overall}}}
%     \addlinespace[0.3pt]
%     & \small{Tool}} & \small{Exe}} & \small{Num}} & \small{Text}} & \small{Vis}} & \small{AVG}} & \small{Tool}} & \small{Exe}} & \small{Num}} & \small{Text}} & \small{Vis}} & \small{AVG}}  \\ \midrule %
%         % \multicolumn{8}{l}{{\textasciitilde7B}}  \\ \hline
% Llama2-7B   &   44.3   &   18.7   &   0.7   &   8.0   &   2.6   &   3.8   &   46.3   &   23.5   &   9.5   &   4.0   &   11.8   &   8.4   &   6.1   \\ 
% Yi-6B   &   84.7   &   50.0   &   10.9   &   33.0   &   36.5   &   26.8   &   88.1   &   46.8   &   9.5   &   23.9   &   29.2   &   20.9   &   23.8   \\ 
% ChatGLM3-6B   &   65.9   &   41.8   &   21.1   &   25.2   &   26.3   &   24.2   &   58.0   &   36.7   &   10.9   &   27.5   &   22.9   &   20.4   &   22.3   \\ 
% DeepSeek-7B   &   90.2   &   57.0   &   11.6   &   26.6   &   44.7   &   27.6   &   77.7   &   50.4   &   11.6   &   14.0   &   40.7   &   22.1   &   24.9   \\ 
% Vicuna-7B   &   88.5   &   50.4   &   15.7   &   35.6   &   32.6   &   28.0   &   87.2   &   55.5   &   8.8   &   26.1   &   19.5   &   18.1   &   23.0   \\ 
% Qwen-7B   &   99.8   &   72.5   &   21.1   &   65.9   &   45.5   &   44.2   &   94.5   &   57.4   &   15.7   &   23.1   &   30.9   &   23.2   &   33.7   \\ 
% Qwen1.5-7B   &   98.7   &   71.2   &   25.2   &   88.1   &   41.8   &   51.7   &   98.3   &   65.7   &   15.7   &   60.1   &   37.0   &   37.6   &   44.6   \\ 
% Mistral-7B   &   99.4   &   69.3   &   31.3   &   78.7   &   48.1   &   52.7   &   98.5   &   71.0   &   19.7   &   54.2   &   42.8   &   38.9   &   45.8   \\ 
% InternLM2-7B-SFT   &   99.2   &   73.4   &   36.0   &   62.5   &   44.8   &   47.8   &   99.6   &   67.0   &   20.4   &   30.9   &   49.3   &   33.5   &   40.7   \\ 
% InternLM2-7B   &   99.2   &   68.7   &   37.4   &   53.7   &   51.8   &   47.6   &   100.0   &   67.8   &   29.2   &   48.4   &   53.2   &   43.6   &   45.6   \\ \midrule 
% Llama2-13B   &   96.4   &   65.0   &   13.6   &   23.7   &   25.5   &   20.9   &   96.4   &   73.6   &   10.9   &   27.9   &   18.2   &   19.0   &   20.0   \\ 
% Vicuna-13B   &   88.9   &   62.9   &   12.2   &   74.2   &   40.1   &   42.2   &   92.5   &   65.5   &   15.0   &   52.9   &   45.9   &   37.9   &   40.0   \\ 
% Qwen-14B   &   90.2   &   70.4   &   33.3   &   65.7   &   54.7   &   51.2   &   93.6   &   71.4   &   34.0   &   52.3   &   54.3   &   46.9   &   49.1   \\ 
% Qwen1.5-14B   &   99.8   &   86.2   &   42.9   &   85.0   &   59.6   &   62.5   &   99.8   &   89.3   &   31.3   &   72.7   &   56.4   &   53.4   &   58.0   \\ 
% Mistral-8x7B   &   99.6   &   85.1   &   25.2   &   79.7   &   51.6   &   52.2   &   99.6   &   84.5   &   19.7   &   74.2   &   55.5   &   49.8   &   51.0   \\ 
% InternLM2-20B-SFT   &   99.2   &   85.9   &   38.1   &   75.5   &   52.7   &   55.4   &   99.4   &   82.3   &   29.9   &   63.1   &   55.7   &   49.6   &   52.5   \\ 
% InternLM2-20B   &   98.5   &   84.7   &   42.9   &   80.8   &   54.9   &   59.5   &   100.0   &   87.8   &   27.2   &   44.9   &   58.5   &   43.5   &   51.5   \\ \bottomrule 
% % Yi-34B   &   81.7   &   56.1   &   30.6   &   36.2   &   47.4   &   38.1   &   89.3   &   60.0   &   22.4   &   36.9   &   43.2   &   34.2   &   36.1   \\ 
% % Llama2-70B   &   99.1   &   66.8   &   18.4   &   37.0   &   34.2   &   29.9   &   98.7   &   67.0   &   15.0   &   37.3   &   31.2   &   27.8   &   28.8   \\ 
% % DeepSeek-67B   &   99.8   &   85.5   &   39.5   &   78.5   &   66.2   &   61.4   &   99.4   &   81.0   &   37.4   &   80.6   &   61.8   &   59.9   &   60.7   \\ 
% % Qwen-72B   &   99.4   &   85.3   &   45.6   &   77.5   &   65.8   &   63.0   &   91.4   &   73.1   &   30.6   &   27.9   &   45.2   &   34.6   &   48.8   \\ \midrule 
% % GPT-4-0613   &   99.6   &   98.3   &   50.3   &   85.0   &   75.0   &   70.1   &   98.1   &   95.5   &   45.6   &   81.4   &   74.7   &   67.2   &   68.7   \\  \bottomrule
%         % \multicolumn{8}{l}{{API}}  \\ \hline
%         % GPT-4-Turbo & 71.5  & 82.6  & 50.8  & 73.1  & 81.3  & 61.7  & 70.2  \\ 
%         % ChatGLM\_Pro & 99.1  & 72.8  & 42.3  & 45.1  & 42.6 & 100.0  & 58.8   & 45.7  & 62.4  & 39.0  & 46.2  \\ 
%         % Baichuan2\_Turbo & 88.1  & 68.6  & 39.9  & 51.7  & 38.8 & 100.0  & 61.0   & 51.5  & 70.8  & 36.4  & 48.2  \\ 
%         % % Claude-2 & 99.7  & 32.9  & 37.8  & 41.1  & 26.7 & 42.3  & 45.1   & 61.0  & {78.1}  & 59.7  & 50.7  \\ 
%         % Qwen-Max & 99.6  & 87.3  & 55.5  & 67.8  & 50.5  & 99.5  & 85.7  & {72.2}  & 71.5  & 58.9  & 62.7  \\ 
%         % GPT4-Turbo & 99.8  & 97.9  & 76.0  & 78.9  & 64.0 & 99.6  & 92.5  & 70.8  & 76.5  & 67.4  & 72.3  \\ \bottomrule
%         % GPT-4-0613 & 99.7  & 98.4  & 66.8  & 75.7  & 65.5 & 99.8  & 97.8  & 70.7  & 84.2  & 73.6  & 72.8  \\ \bottomrule
% \end{tabular}
% }
% \vspace{-1em}
% \end{table*}



\begin{table*}[!t]
    \setlength{\tabcolsep}{6pt}
    \renewcommand{\arraystretch}{1.1}
    \centering
    \resizebox{0.8\textwidth}{!}{%
    \begin{tabular}{l|c|ccc|ccc}
\multirow{2}{*}{model name} & \multirow{2}{*}{\#param}  & \multicolumn{3}{c|}{{T-Eval}} & \multicolumn{3}{c}{{CIBench}}\\ 
& & \small{English} & \small{Chinese} & \small{avg.} &  \small{English} & \small{Chinese} & \small{avg.}\\ 
\hline
% \multicolumn{7}{c}{\greencolor{\textit{ $\leq 7$B Models}}} \\ 
Llama2-7B-Chat   & 7B &   37.5 & 37.0 & 37.2 &   12.2   &   10.6   &   11.4   \\ 
Llama2-13B-Chat   & 13B &  48.7 & 44.9 & 46.8 &   20.0   &   12.3   &   16.1     \\ 

% Yi-6B   &   000 & 000 & 000 &   26.8   &   20.9   &   23.8   \\ 
% DeepSeek-7B   &   000 & 000 & 000 &   27.6   &   22.1   &   24.9   \\ 
% Vicuna-7B   &   000 & 000 & 000 &   28.0   &   18.1   &   23.0   \\
% Vicuna-13B   &   000 & 000 & 000 &   42.2   &   37.9   &   40.0   \\ 

% Baichuan2-7B-Chat &   58.5 & 53.7 &  &   28.0   &   18.1   &   23.0   \\
Qwen-7B-Chat   & 7B &  57.5 & 61.1 & 59.3 &   47.8   &   29.2   &   38.5     \\ 
Qwen-14B-Chat   & 14B &  63.6 & {{68.7}} & {{66.2}}  &   54.8   &   40.8   &   47.8   \\ 

Qwen1.5-7B-Chat   & 7B &  54.5 & 50.4 & 52.5 &   44.7   &   26.9   &   35.8   \\ 
Qwen1.5-14B-Chat   & 14B &  67.6 & 63.3 & 65.4 &   57.9   &   49.7   &   53.8   \\ 

Mistral-7B-Instruct-v0.2   & 7.3B &  39.3 & 38.7 & 39.0 &   47.6   &   38.0   &   42.8   \\ 
Mistral-8x7B-Instruct-v0.1   & 46.7B & 58.6 & 58.0 & 58.3 &   42.6   &   40.3   &   41.5   \\ 

ChatGLM3-6B   & 6.2B &  62.3 & 63.6 & 63.0 &   29.4   &   17.1   &   23.2   \\ 
\hline

% \multicolumn{7}{c}{\bluecolor{\textit{ $13 \sim 20$B Models}}} \\ 
\rowcolor{gray!15}
InternLM2-Chat-7B-SFT   & 7B &  64.1 & {66.8} & 65.5 &   52.1   &   27.8   &   39.9 \\ 
\rowcolor{gray!15}
InternLM2-Chat-7B   & 7B &  {{66.1}} & 65.4 & {65.8}  &   {{57.1}}   &   {{40.7}}   &   {{48.9}}     \\ 
\rowcolor{gray!15}
InternLM2-Chat-20B-SFT   & 20B &  64.7 & 64.1 & 64.4 &   49.0   &   43.7   &   46.4   \\ 
\rowcolor{gray!15}
InternLM2-Chat-20B   &  20B & {65.6} &  62.9 & 64.3 &   {{56.0}}   &   {{54.7}}   &   {{55.4}}   \\ 
% Yi-34B   &   81.7   &   56.1   &   30.6   &   36.2   &   47.4   &   38.1   &   89.3   &   60.0   &   22.4   &   36.9   &   43.2   &   34.2   &   36.1   \\ 
% Llama2-70B   &   99.1   &   66.8   &   18.4   &   37.0   &   34.2   &   29.9   &   98.7   &   67.0   &   15.0   &   37.3   &   31.2   &   27.8   &   28.8   \\ 
% DeepSeek-67B   &   99.8   &   85.5   &   39.5   &   78.5   &   66.2   &   61.4   &   99.4   &   81.0   &   37.4   &   80.6   &   61.8   &   59.9   &   60.7   \\ 
% Qwen-72B   &   99.4   &   85.3   &   45.6   &   77.5   &   65.8   &   63.0   &   91.4   &   73.1   &   30.6   &   27.9   &   45.2   &   34.6   &   48.8   \\ \midrule 
% GPT-4-0613   &   99.6   &   98.3   &   50.3   &   85.0   &   75.0   &   70.1   &   98.1   &   95.5   &   45.6   &   81.4   &   74.7   &   67.2   &   68.7   \\  \bottomrule
        % \multicolumn{8}{l}{{API}}  \\ \hline
        % GPT-4-Turbo & 71.5  & 82.6  & 50.8  & 73.1  & 81.3  & 61.7  & 70.2  \\ 
        % ChatGLM\_Pro & 99.1  & 72.8  & 42.3  & 45.1  & 42.6 & 100.0  & 58.8   & 45.7  & 62.4  & 39.0  & 46.2  \\ 
        % Baichuan2\_Turbo & 88.1  & 68.6  & 39.9  & 51.7  & 38.8 & 100.0  & 61.0   & 51.5  & 70.8  & 36.4  & 48.2  \\ 
        % % Claude-2 & 99.7  & 32.9  & 37.8  & 41.1  & 26.7 & 42.3  & 45.1   & 61.0  & {78.1}  & 59.7  & 50.7  \\ 
        % Qwen-Max & 99.6  & 87.3  & 55.5  & 67.8  & 50.5  & 99.5  & 85.7  & {72.2}  & 71.5  & 58.9  & 62.7  \\ 
        % GPT4-Turbo & 99.8  & 97.9  & 76.0  & 78.9  & 64.0 & 99.6  & 92.5  & 70.8  & 76.5  & 67.4  & 72.3  \\ \bottomrule
        % GPT-4-0613 & 99.7  & 98.4  & 66.8  & 75.7  & 65.5 & 99.8  & 97.8  & 70.7  & 84.2  & 73.6  & 72.8  \\ \bottomrule
\end{tabular}
}
\caption{\textbf{Results on T-Eval and CIBench.}}
\label{tab:cibench_teval}
\end{table*}

==> table/benchmark_video.tex <==
\begin{table*}[t!]
\centering
\renewcommand{\arraystretch}{0.95}
\setlength\tabcolsep{3pt}
\newcommand{\VMME}{\makecell{Video-MME\\(wo / w sub)}}
\newcommand{\MVB}{\makecell{MVBench}}
\newcommand{\MMBV}{\makecell{MMBench-Video\\(val)}}
\newcommand{\MLVU}{\makecell{MLVU\\(M-Avg)}}
\newcommand{\LVB}{\makecell{LongVideoBench\\(val total)}}
\newcommand{\CG}{\makecell{CG-Bench\\(long / clue acc.)}}
\newcommand{\lsp}{--\ \ \ \ \ \ }
\newcommand{\rsp}{\ \ \ \ \ --~}
{\fontsize{8}{10}\selectfont 
\begin{tabular}{l|cccccc|c}
Model Name                                 &    \VMME    & \MVB & \MMBV & \MLVU & \LVB  & \CG         & Overall \\
\hline
InternVL2-1B~\cite{chen2024far}            & 42.9 / 45.4 & 57.5 & 1.14  & 51.6  & 43.3  & --          & --      \\
InternVL2.5-1B~\cite{chen2024expanding}    & 50.3 / 52.3 & 64.3 & 1.36  & 57.3  & 47.9  & --          & --      \\
\rowcolor{gray!15}
InternVL3-1B                               & 51.0 / 53.0 & 63.1 &  1.3  & 53.0  & 48.1  & 24.8 / 39.1 & 46.9    \\
Qwen2-VL-2B~\cite{wang2024qwen2vl}         & 55.6 / 60.4 & 63.2 & --    & --    & --    & --          & --      \\
Qwen2.5-VL-3B~\cite{bai2025qwen2_5}        & 61.5 / 67.6 & 67.0 & 1.63  & 68.2  & 43.3  & --          & --      \\
InternVL2-2B~\cite{chen2024far}            & 46.2 / 49.1 & 60.2 & 1.30  & 54.3  & 46.0  & --          & --      \\
InternVL2.5-2B~\cite{chen2024expanding}    & 51.9 / 54.1 & 68.8 & 1.44  & 61.4  & 52.0  & --          & --      \\
\rowcolor{gray!15}
InternVL3-2B                               & 58.9 / 61.4 & 70.4 & 1.42  & 64.2  & 55.4  & 30.8 / 50.7 & 54.9    \\
\hline
VideoChat2-HD~\cite{li2023videochat}       & 45.3 / 55.7 & 62.3 & 1.22  & 47.9  & --    & --          & --      \\
MiniCPM-V-2.6~\cite{yao2024minicpm}        & 60.9 / 63.6 & --   & 1.70  & --    & 54.9  & --          & --      \\
LLaVA-OneVision-7B~\cite{li2024llavaov}    & 58.2 / \lsp & 56.7 & --    & --    & --    & --          & --      \\
Qwen2-VL-7B~\cite{wang2024qwen2vl}         & 63.3 / 69.0 & 67.0 & 1.44  & --    & 55.6  & --          & --      \\
Qwen2.5-VL-7B~\cite{bai2025qwen2_5}        & 65.1 / 71.6 & 69.6 & 1.79  & 70.2  & 45.3  & --          & --      \\
InternVL2-8B~\cite{chen2024far}            & 56.3 / 59.3 & 65.8 & 1.57  & 64.0  & 54.6  & --          & --      \\
InternVL2.5-8B~\cite{chen2024expanding}    & 64.2 / 66.9 & 72.0 & 1.68  & 68.9  & 60.0  & --          & --      \\
\rowcolor{gray!15}
InternVL3-8B                               & 66.3 / 68.9 & 75.4 & 1.69  & 71.4  & 58.8  & 38.6 / 55.2 & 61.4    \\
\rowcolor{gray!15}
InternVL3-9B                               & 66.7 / 68.9 & 74.3 & 1.69  & 70.8  & 62.5  & 41.1 / 58.0 & 62.3    \\
\rowcolor{gray!15}
InternVL3-14B                              & 70.4 / 73.0 & 76.6 & 1.73  & 73.3  & 63.9  & 44.1 / 60.6 & 64.9    \\
\hline
InternVL2-26B~\cite{chen2024far}           & 57.0 / 60.2 & 67.5 & 1.67  & 64.2  & 56.1  & --          & --      \\
InternVL2.5-26B                            & 66.9 / 69.2 & 75.2 & 1.86  & 72.3  & 59.9  & --          & --      \\
Oryx-1.5-32B~\cite{liu2024oryx}            & 67.3 / 74.9 & 70.1 & 1.52  & 72.3  & --    & --          & --      \\  
Qwen2.5-VL-32B~\cite{bai2025qwen2_5}       & 70.5 / 77.9 & --   & 1.93  & --    & --    & --          & --      \\
VILA-1.5-40B~\cite{lin2024vila}            & 60.1 / 61.1 & --   & 1.61  & 56.7  & --    & --          & --      \\
InternVL2-40B~\cite{chen2024far}           & 66.1 / 68.6 & 72.0 & 1.78  & 71.0  & 60.6  & --          & --      \\
InternVL2.5-38B~\cite{chen2024expanding}   & 70.7 / 73.1 & 74.4 & 1.82  & 75.3  & 63.3  & --          & --      \\
\rowcolor{gray!15}
InternVL3-38B                              & 72.7 / 75.0 & 76.9 & 1.81  & 77.8  & 67.3  & 46.9 / 62.8 & 67.5    \\
\hline
GPT-4V/4T~\cite{openai2023gpt4}            & 59.9 / 63.3 & 43.7 & 1.53  & 49.2  & 59.1  & --          & --      \\
GPT-4o-20240513~\cite{gpt4v}               & 71.9 / 77.2 & --   & 1.63  & 64.6  & 66.7  & --          & --      \\
GPT-4o-20240806~\cite{gpt4v}               & --          & --   & 1.87  & --    & --    & 41.8 / 58.3 & --      \\
Gemini-1.5-Pro~\cite{reid2024gemini1_5}    & 75.0 / 81.3 & --   & 1.30  & --    & 64.0  & 40.1 / 56.4 & --      \\
VideoLLaMA2-72B~\cite{cheng2024videollama2}& 61.4 / 63.1 & 62.0 & --    & --    & --    & --          & --      \\
LLaVA-OneVision-72B~\cite{li2024llavaov}   & 66.2 / 69.5 & 59.4 & --    & 66.4  & 61.3  & --          & --      \\
Qwen2-VL-72B~\cite{wang2024qwen2vl}        & 71.2 / 77.8 & 73.6 & 1.70  & --    & --    & 41.3 / 56.2 & --      \\
Qwen2.5-VL-72B~\cite{bai2025qwen2_5}       & 73.3 / 79.1 & 70.4 & 2.02  & 74.6  & 60.7  & --          & --      \\
InternVL2-Llama3-76B~\cite{chen2024far}    & 64.7 / 67.8 & 69.6 & 1.71  & 69.9  & 61.1  & --          & --      \\
InternVL2.5-78B~\cite{chen2024expanding}   & 72.1 / 74.0 & 76.4 & 1.97  & 75.7  & 63.6  & 42.2 / 58.5 & 66.0    \\ 
\rowcolor{gray!15}
InternVL3-78B                              & 72.7 / 75.7 & 78.7 & 1.81  & 79.5  & 65.7  & 48.4 / 65.3 & 68.3    \\ 
% \rowcolor{gray!15}
% InternVL2.5-Pro                          &      /      &      &       &       &       &             &         \\  
\end{tabular}
}
\caption{\textbf{Comparison of video understanding performance.}
We evaluate InternVL's video understanding capabilities across 6 benchmarks.
For Video-MME~\cite{fu2024video}, MMBench-Video~\cite{fang2024mmbench}, MLVU~\cite{MLVU}, and LongVideoBench~\cite{wu2024longvideobench}, we test with four different settings: 16, 32, 48, and 64 frames, and report the maximum results. For MVBench~\cite{li2024mvbench}, we conduct testing using 16 frames. For CG-Bench~\cite{anonymous2024cgbench}, we use 32 frames.
}
\label{tab:benchmark_video}
\end{table*}

==> table/evaluation/agent.tex <==
\subsection{Tool Utilization}

\subsubsection{Datasets}

It is widely acknowledged that external tools and APIs can significantly enhance the capabilities of LLMs to tackle complex, real-world problems~\cite{DBLP:journals/corr/abs-2304-08354,DBLP:journals/corr/abs-2307-16789,DBLP:journals/corr/abs-2302-04761}. To analyze InternLM2's proficiency in tool utilization, 
we conduct experiments across several benchmark datasets: GSM8K~\cite{DBLP:journals/corr/abs-2110-14168}, MATH~\cite{DBLP:conf/nips/HendrycksBKABTS21}, the recently introduced MathBench~\cite{Anonymousmathbench}, T-Eval~\cite{chen2023t}, and the template subset of CIBench~\cite{Anonymouscibench}, all employing the ReAct protocol~\cite{DBLP:conf/iclr/YaoZYDSN023} where LLMs alternate between generating thought processes and executing actions. 


\textbf{GSM8K}, \textbf{MATH} and \textbf{MathBench} are introduced in Sec~\ref{sec:lm_reasoning_and_math}. 

\textbf{T-Eval}: T-Eval features human-verified, high-quality question instructions with corresponding step-by-step solutions. It measures an LLM's proficiency with everyday tools such as Google Search and Gaode Map across six different dimensions. 

\textbf{CIBench}: developed by our team, simulates genuine data analysis scenarios using interactive Jupyter notebooks. It encompasses multiple, consecutive tasks and covers the most commonly used Python modules in data analysis, including Pandas, Numpy, and Pytorch. This custom-made benchmark allows for a thorough assessment of an LLM's comprehensive ability in data analysis. 

% Notably, MathBench comprises 3709 questions, covering the mathematical concepts in primary, middle, and high school, allowing us to measure LLM's math problem-solving ability thoroughly. T-Eval~\cite{chen2023t} consists of human-verified high-quality question instruction and corresponding step-by-step solutions, measuring LLM's ability on daily used tools, like Google search, Gaode map, etc, from six dimensions. CIBench is constructed by ourselves to simulate authentic scenarios in data analysis, consists of interactive Jupyter notebooks, which contain multiple and consecutive tasks, and cover the most widely-used Python modules used in data analysis (e.g. Pandas, Numpy, Pytorch), benchmark LLM's ability in data analysis comprehensively. 
%The dataset details of CIBench are in the Appendix.

\subsubsection{Evaluation Results}

\paragraph{GSM8K, MATH and MathBench} We utilize the external code interpreter and follow the ReAct protocol to evaluate LLM's ability to solve coding and mathematic problems. The results, as depicted in Figure~\ref{fig:agent_gsm8k_math}, demonstrate a substantial improvement even when using the code interpreter, particularly on the MATH dataset where the enhancement is notably significant. 

% TODO: wait for results to update the text.
As depicted in Figure~\ref{fig:agent_mathbench}, regarding the recently introduced MathBench dataset, the utilization of a code interpreter results in improved performance for InternLM2's performance in most cases, and a minor decrease may be attributed to the incorrect usage of such interpreters. Moreover, notable improvements are observed within the Knowledge domain for InternLM2-20B-Chat and in the Application section for InternLM2-7B-Chat. These disparities can stem from a multitude of factors, including differences in the constitution of their respective training datasets.

% what is the difference of application and knowledge

% TODO: wait for decision on Qwen1.5
% cibench fig:prompt_of_cibench
\paragraph{T-Eval and CIBench} As depicted in Table~\ref{tab:cibench_teval}, the InternLM2 models consistently demonstrate superior or comparable performance compared to existing models across various benchmarks. Specifically, when comparing models of identical scale, InternLM2-Chat-7B emerges as the top performer on T-Eval and CIBench. Meanwhile, InternLM2-Chat-20B achieves competitive results on T-Eval while obtaining the highest scores on CIBench. Additionally, the InternLM2 series models achieve impressive results in Chinese, showcasing their proficiency in multiple languages.



% Furthermore, InternLM2-Chat observes similar results with InternLM2-Chat-SFT, which serves as compelling evidence for the robustness and effectiveness of our RLHF alignment strategy. This consistency indicates that the fine-tuning process through RLHF has successfully maintained the model's competitive edge without compromising its inherent capabilities.

% Comparing the performance of English with Chinese shows that the performance of Chinese is inferior to English, 



% \paragraph{General Tool Utilization}
% \paragraph{Code Interpreter}

\begin{figure*}[!t]
    \centering
    \includegraphics[scale=0.38]{figure/internLM2/gsm8k_math.pdf}
    \caption{Results on GSM8K (4-shot) and MATH (4-shot) with and w/o Code Interpreter.}
    \label{fig:agent_gsm8k_math}
\end{figure*}

\begin{figure*}[!t]
    \centering
    \includegraphics[scale=0.4]{figure/internLM2/mathbench.pdf}
    \caption{Results on MathBench with and without ReAct.}
    \label{fig:agent_mathbench}
\end{figure*}

\input{table/benchmark_teval_cibench}

% \paragraph{CIBench}





==> table/evaluation/coding_python_table.tex <==

\begin{table*}[!thb]
\centering
\caption{\textbf{Overall Comparison of Models on Python Coding}. 
% The model name in \textbf{bold} indicates the top performer, while an \underline{underline} signifies the leading model within a similar parameter size group.
}
% \vspace{-2mm}
\label{tab:main_results}
\resizebox{\linewidth}{!}{
\tablestyle{10pt}{1.2}
\begin{tabular}{l|ccccc}
\toprule
\textbf{Models} & \textbf{MMLU} & \textbf{CMMLU} & \textbf{C-Eval} & \textbf{AGIEval} & \textbf{GAOKAO-Bench} \\
& \textit{4-shot} & \textit{4-shot} & \textit{5-shot} & \textit{variable shots} & \textit{0-shot}\\
\hline
% \multicolumn{7}{c}{\purplecolor{\textit{\ding{72} $> 20$B}}} \\
\multicolumn{6}{c}{\purplecolor{\textit{ API Models}}} \\
GPT-3.5 &   \\
% GPT-4 & \textbf{76.3} & \textbf{82.9 }& \textbf{69.8} & \textbf{56.6} & \textbf{59.0} & \textbf{68.9} \\
% \hline
\multicolumn{6}{c}{\greencolor{\textit{  $\leq 7$B Models}}} \\
Llama2-7B-Chat &  \\
Gemma-7B-IT & \\
ChatGLM3-6B &   \\
InternLM2-Chat-Math-7B &  \\
Mistral-7B-Instruct-v0.2 & \\
Baichuan2-7B-Chat & \\
Qwen-1.5-7B-Chat &  \\
\midrule
InternLM2-Chat-7B &  \\
% \hline
\multicolumn{6}{c}{\bluecolor{\textit{ $13\sim 20$B Models}}} \\
Llama2-13B-Chat~\cite{touvron2023llama}           &\\
Mixtral-8x7B-instruct-v0.1 &\\
Qwen1.5-14B-Chat           &   \\
Baichuan2-13B-Chat         &   \\
\midrule
InternLM2-Chat-20B         &   \\
\bottomrule
\end{tabular}}
\end{table*}

==> table/evaluation/examination_table.tex <==

\newcommand\redcolor[1]{\cellcolor{gray!40!red!30}{#1}}
\newcommand\bluecolor[1]{\cellcolor[HTML]{EAE2FE}{#1}}
\newcommand\greencolor[1]{\cellcolor[HTML]{DFF5E5}{#1}}
\newcommand\yellowcolor[1]{\cellcolor[HTML]{FEF1CE}{#1}}
\newcommand\purplecolor[1]{\cellcolor[HTML]{A8B3E3}{#1}}

% 对话模型
% \begin{table*}[!t]
% \centering
% \resizebox{\linewidth}{!}{
% \tablestyle{10pt}{1.2}
% \begin{tabular}{l|c|ccccc|c}
% \multirow{2}{*}{model name} & \multirow{2}{*}{\#param} & {MMLU} & {CMMLU} & {C-Eval} & {AGIEval} & {GAOKAO} &   \multirow{2}{*}{avg.} \\
% & &{(5-shot)} & {(5-shot)} & {(5-shot)} & {(0-shot)} & {(0-shot)} &  \\
% \hline
% % \multicolumn{7}{c}{\purplecolor{{ API Models}}} \\
% GPT-3.5 & -- & 69.1 & 53.9 & 52.5 & 39.9 & 51.1 & 53.30 \\
% \hline
% % \multicolumn{7}{c}{\greencolor{{  $\leq 7$B Models}}} \\
% Llama2-7B-Chat & xxB &  48.2 & 30.7 & 34.9 & 28.5 & 19.8 &  24.4 \\
% % Gemma-7B-IT &  &  &  &  &  \\
% Mistral-7B-Instruct-v0.2 & xxB &  59.2 & 42.0 & 42.4 & 34.5 & 28.6 & 41.3 \\
% Baichuan2-7B-Chat & xxB & 50.1 &  53.4 & 53.9 & 35.3 & 37.5 & 46.0 \\
% ChatGLM3-6B & xxB & 58.0 & 57.8 & 59.1 & 44.2 & 56.3 & 55.1 \\
% Qwen-7B-Chat & xxB & 57.1 & 57.9 & 59.8 & 39.7 & \underline{62.1} & 55.3 \\
% % Qwen1.5-7B-Chat & 61.0 & \underline{68.0} & \underline{70.6} & 44.9 & \underline{69.9} \\
% \hline
% \rowcolor{gray!15}
% InternLM2-Chat-7B-SFT & xxB & \underline{63.8} & \underline{63.2} & 
% \underline{60.9} & \underline{49.0} & 57.3 & \underline{58.8} \\
% \rowcolor{gray!15}
% InternLM2-Chat-7B & xxB & 63.7 & 63.0 & 60.8 & 47.2 & 58.0 & 58.5 \\
% \hline
% % \multicolumn{7}{c}{\bluecolor{{ $13\sim 20$B Models}}} \\
% Llama2-13B-Chat & xxB & 54.1 & 33.8 & 35.0 & 30.9 & 23.2 & 35.4 \\
% Mixtral-8x7B-Instruct-v0.1 & xxB & \underline{\textbf{70.3}} & 50.6 & 54.0 & 41.7 & 42.6 & 51.8 \\
% Baichuan2-13B-Chat & xxB & 56.6 & 54.8 & 56.3 & 40.0 & 45.8 & 50.7 \\
% Qwen-14B-Chat & xxB & 66.7 &  \underline{\textbf{68.1}} & \underline{\textbf{71.5}} & 46.5 & \underline{\textbf{76.3}} & \textbf{\underline{65.8}} \\
% % Qwen1.5-14B-Chat & 67.2 & \underline{\textbf{75.1}} & \underline{\textbf{76.0}} & 50.6 & \underline{\textbf{80.3}} \\
% \hline
% \rowcolor{gray!15}
% InternLM2-Chat-20B-SFT & xxB & 66.5 & 65.3 & 63.7 & \underline{\textbf{51.2}} & 58.6 & 61.1\\
% \rowcolor{gray!15}
% InternLM2-Chat-20B & xxB & 66.5 & 65.1 & 63.0 & 50.3 & 58.3 & 60.6 \\
% \end{tabular}}

% \caption{\textbf{Comparison of chat models on comprehensive examination}. The model name in \textbf{bold} indicates the top performer, while an \underline{underline} signifies the leading model within a similar parameter size group.}
% % \vspace{-2mm}
% \label{tab:exam_chat_results}
% \end{table*}


\begin{table*}[!t]
\centering
\resizebox{\linewidth}{!}{
\tablestyle{10pt}{1.2}
\begin{tabular}{l|c|ccccc|c}
\multirow{2}{*}{model name} & \multirow{2}{*}{\#param} & {MMLU} & {CMMLU} & {C-Eval} & {AGIEval} & {GAOKAO} &   \multirow{2}{*}{avg.} \\
& &{(5-shot)} & {(5-shot)} & {(5-shot)} & {(0-shot)} & {(0-shot)} &  \\
\hline
% \multicolumn{7}{c}{\purplecolor{{ API Models}}} \\
GPT-3.5 & -- & 69.1 & 53.9 & 52.5 & 39.9 & 51.1 & 53.3 \\
\hline
% \multicolumn{7}{c}{\greencolor{{  $\leq 7$B Models}}} \\
Llama2-7B-Chat & 7B &  48.2 & 30.7 & 34.9 & 28.5 & 19.8 &  24.4 \\
Llama2-13B-Chat & 13B & 54.1 & 33.8 & 35.0 & 30.9 & 23.2 & 35.4 \\

% Gemma-7B-IT &  &  &  &  &  \\
Mistral-7B-Instruct-v0.2 & 7.3B &  59.2 & 42.0 & 42.4 & 34.5 & 28.6 & 41.3 \\
Mixtral-8x7B-Instruct-v0.1 & 46.7B & {{70.3}} & 50.6 & 54.0 & 41.7 & 42.6 & 51.8 \\
Baichuan2-7B-Chat & 7B & 50.1 &  53.4 & 53.9 & 35.3 & 37.5 & 46.0 \\
Baichuan2-13B-Chat & 13B & 56.6 & 54.8 & 56.3 & 40.0 & 45.8 & 50.7 \\

Qwen-7B-Chat & 7B & 57.1 & 57.9 & 59.8 & 39.7 & {62.1} & 55.3 \\
Qwen-14B-Chat & 14B & 66.7 &  {{68.1}} & {{71.5}} & 46.5 & {{76.3}} & {{65.8}} \\
ChatGLM3-6B & 6.2B & 58.0 & 57.8 & 59.1 & 44.2 & 56.3 & 55.1 \\
% Qwen1.5-7B-Chat & 61.0 & \underline{68.0} & \underline{70.6} & 44.9 & \underline{69.9} \\
% \multicolumn{7}{c}{\bluecolor{{ $13\sim 20$B Models}}} \\
% Qwen1.5-14B-Chat & 67.2 & \underline{\textbf{75.1}} & \underline{\textbf{76.0}} & 50.6 & \underline{\textbf{80.3}} \\
\hline
\rowcolor{gray!15}
InternLM2-Chat-7B-SFT & 7B & {63.8} & {63.2} & 
{60.9} & {49.0} & 57.3 & {58.8} \\
\rowcolor{gray!15}
InternLM2-Chat-7B & 7B & 63.7 & 63.0 & 60.8 & 47.2 & 58.0 & 58.5 \\
\rowcolor{gray!15}
InternLM2-Chat-20B-SFT & 20B & 66.5 & 65.3 & 63.7 & {{51.2}} & 58.6 & 61.1\\
\rowcolor{gray!15}
InternLM2-Chat-20B & 20B & 66.5 & 65.1 & 63.0 & 50.3 & 58.3 & 60.6 \\
\end{tabular}}
\caption{\textbf{Comparison of chat models on comprehensive examination}. We evaluate model's comprehensive examination capability across 5 benchmarks, including MMLU~\cite{hendrycks2020measuring}, CMMLU~\cite{li2023cmmlu}, C-Eval~\cite{huang2023ceval}, AGIEval~\cite{zhong2023agieval} and GAOKAO-Bench~\cite{Zhang2023EvaluatingTP}.
\textcolor{red}{TODO cy: param 保留一位的都是在源技术文档里明确找出的参数量，baichuan2和qwen即使原技术文档也还是整数}
}
% TODO cy: 保留一位的都是在源技术文档里明确找出的参数量，baichuan2和qwen即使原技术文档也还是整数

% \vspace{-2mm}
\label{tab:exam_chat_results}
\end{table*}


==> table/evaluation/language_table_1.tex <==
\begin{table*}[!t]
\centering

\resizebox{\linewidth}{!}{
\tablestyle{10pt}{1.2}
\begin{tabular}{l|c|ccccc|c}
\multirow{2}{*}{model name} & \multirow{2}{*}{\#param} & {TriviaQA} & {NaturalQuestions} & {C3} & {RACE-High} & {FLORES} &  \multirow{2}{*}{avg.} \\
& & {(4-shot)} & {(5-shot)} & {(5-shot)} & {(0-shot)} & {(0-shot)}\\
\hline
% \multicolumn{7}{c}{\purplecolor{{\ding{72} $> 20$B}}} \\
% \multicolumn{7}{c}{\purplecolor{{ API Models}}} \\
GPT-3.5 & -- & 69.1 & 53.9 & 52.5 & 39.9 & 51.1 & 53.3 \\
\hline
% \multicolumn{7}{c}{\greencolor{{  $\leq 7$B Models}}} \\
Llama2-7B-Chat & 7B & 46.8 & 19.6 & 51.7 & 3.0 & 5.3 & 25.3 \\
Llama2-13B-Chat                 & 13B & 54.4 & 25.2 & 56.9 & 19.2 & 6.6 & 32.5\\
% Gemma-7B-IT &  &  &  &  &  \\
Mistral-7B-Instruct-v0.2        & 7.3B & 35.0 & 8.1  & 66.9 & 71.2 & 12.8 & 38.8 \\
Mixtral-8x7B-Instruct-v0.1      & 46.7B & 57.7 & 22.5 & 82.1 & 81.4 & 17.2 & 52.2\\
Baichuan2-7B-Chat               & 7B & 37.6 & 12.8 & 78.5 & 67.5 & 11.0 & 41.5\\
Baichuan2-13B-Chat              & 13B & 40.3 & 12.7 & 84.4 & 73.2 & 12.4 & 44.6 \\
Qwen-7B-Chat                    & 7B & 46.1 & 18.6 & 84.4 & 74.8 & 12.9 & 47.4\\
Qwen-14B-Chat                   & 14B & 54.5 & 22.9 & 91.5 & 84.7 & 17.3 & 54.2 \\
% Qwen1.5-7B-Chat & 44.6 & 12.7 & 88.6 & 82.3 & 12.2 \\
ChatGLM3-6B                     & 6.2B & 38.1 & 14.0 & 79.3 & 79.1 & 9.7 & 44.0\\
% \hline
% \multicolumn{7}{c}{\bluecolor{{ $13\sim 20$B Models}}} \\
% Qwen1.5-14B-Chat & 54.9 & 15.3 & 93.3 & 86.4 & 15.4 \\
\hline
\rowcolor{gray!15}
InternLM2-Chat-7B-SFT           & 7B &  {51.4} & {24.5} & {91.7} & {85.2} & {15.5} & {53.7} \\
\rowcolor{gray!15}
InternLM2-Chat-7B               & 7B &  50.8 & 24.1 & 91.5 & 85.1 & 15.2 & 53.3 \\
\rowcolor{gray!15}
InternLM2-Chat-20B-SFT          & 20B &  55.5 & {{27.8}} & 93.5 & {{87.3}} & 17.0 & {{56.2}} \\
\rowcolor{gray!15}
InternLM2-Chat-20B              & 20B &  53.9 & 25.9 & {{93.5}} & 87.1 & 16.9 & 55.5 \\
\end{tabular}}
\caption{\textbf{Comparison of chat models on language \& knowledge}. }
% \vspace{-2mm}
\label{tab:language_chat_results}
\end{table*}


==> table/evaluation/long_context_subsub.tex <==

\subsubsection{Datasets}

% \paragraph{Long-context Understanding and Reasoning. }
We mainly evaluate the long-context modeling capability of InternLM2 on the following two benchmarks: L-Eval~\cite{DBLP:journals/corr/abs-2307-11088} and LongBench~\cite{DBLP:journals/corr/abs-2308-14508}. 

\noindent \textbf{L-Eval~\cite{DBLP:journals/corr/abs-2307-11088}: }
L-Eval is a long-context benchmark consisting of 18 subtasks\footnote{
We adopt the first version of L-Eval, corresponding to \href{https://arxiv.org/abs/2307.11088v1}{https://arxiv.org/abs/2307.11088v1}}, 
including texts from various fields such as law, economy, and technology.
L-Eval consists of 411 documents and over 2000 test cases, with an average document length of 7217 words. 
Subtasks in this dataset can be categorized into two major classes:
5 close-ended tasks and 13 open-ended categories. 
Closed-ended tasks are evaluated using exact matching based accuracies,
while open-ended tasks adopt the Rouge score as the metric. 

\noindent \textbf{LongBench~\cite{DBLP:journals/corr/abs-2308-14508}: }
LongBench is a long-context benchmark consisting of 21 subtasks with a total of 4750 test cases. 
It is the first bilingual long-context benchmark, with an average English text length of 6711 words and an average Chinese text length of 13386 characters. 
The 21 subtasks are divided into 6 types, providing a more comprehensive evaluation of the model's capabilities in various aspects.

\textbf{Needle-in-the-Haystack: }
``Needle-in-the-Haystack" is a single-needle retrieval task, which is designed to test the Large Language Models' (LLMs) ability to recall a single piece of key information. This is done by inserting a crucial piece of information into a Haystack text of a target length\footnote{Text token length calculations use the GPT-4 tokenizer} at various positions and then querying the model about this key information at the end of the prompt. This method precisely visualizes LLMs' recall capabilities at different positions within long texts of varying lengths. We design a Chinese Haystack following the original idea, and utilize the Skywork/ChineseDomainModelingEval dataset released by \cite{wei2023skywork}, ensuring diversity and quality in the sources of Chinese texts. This dataset covers a wide range of fields from finance to technology, offering high-quality, up-to-date Chinese articles and providing a stable benchmark for assessing different models' abilities to handle domain-specific long texts. For this experiment, we leverage the LMDeploy\footnote{\href{https://github.com/InternLM/lmdeploy}{https://github.com/InternLM/lmdeploy}} \cite{2023lmdeploy} inference engine to accelerate the inference process. 


\subsubsection{Evaluation Results }
We report the evaluation results of InternLM2 on long-context benchmarks in Table~\ref{tab:longtext_chat_results}.
All variants of InternLM2 have demonstrated strong long-context modeling performance across two benchmarks.
InternLM2-Chat-20B-SFT achieves the best performance on L-Eval and outperforms its counterparts by a considerable margin. 
On LongBench, InternLM2-Chat-7B-SFT outperforms other $\leq 7$B Models models across 4 out of 6 subtask categories. 
It obtains a 48.1 overall score, which is only slightly inferior to the 48.4 overall score of ChatGLM3-6B. 
Meanwhile, we noticed that for InternLM2, different parameter sizes do not lead to significant difference in long-context performance, which will be further investigated. 


\input{table/benchmark_long_context_lm}

\begin{figure*}[!t]
    \centering
    \includegraphics[scale=0.4]{figure/internLM2/InternLM2-7B-200K_Needle_In_A_Haystack_Test.pdf}
    \caption{Results on Needle in the Haystack(Chinese).}
    \label{fig:needle_bench}
\end{figure*}



The results of ``Needle-in-the-Haystack" is presented in Figure \ref{fig:needle_bench}, which effectively demonstrate InternLM2's capability for long-context modeling.

==> table/evaluation/math_table_2.tex <==
% \begin{table*}[!thb]
% \centering
% \caption{{Comparison of Base Models on Reasoning\&Math}. Models are categorized by their parameter size and type, highlighting top performers in each category with {bold} for overall leaders and {underline} for leaders within their parameter group.}
% \vspace{-2mm}
% \label{tab:enhanced_model_results}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{lcccccccc}
% \hline
% {Models/Datasets} & {WinoGrande} & {HellaSwag} & {BBH} & {GSM-8K} & {MATH} & {TheoremQA} & {MathBench-CN}& {MathBench-EN}\\
% & {0-shot} & {0-shot} & {0-shot} & {4-shot} & {4-shot}& {0-shot} & {0-shot\&8-shot}& {0-shot\&8-shot}\\
% \hline
% \multicolumn{8}{c}{\purplecolor{{\ding{72}API Models}}} \\
% GPT-3.5 & 68.7 & 70.2 & 41.9 & 24.6 & 5.5 & 1.6 & - \\
% \multicolumn{8}{c}{\greencolor{{$\triangle$ $\sim7B Models$}}} \\
% ChatGLM3-6B & 61.7 & 73.1 & 56.0 & 53.8 & 20.4 & 9.3 & - \\
% Llama2-7B-Chat & 51.5 & 49.5 & 41.4 & 28.4 & 4.1 & 0.3 & - \\
% Baichuan2-7B-Chat & 49.9 & 36.4 & 35.9 & 32.4 & 5.7 & 2.4 & - \\
% Mistral-7B-Instruct-v0.2 & 50.8 & 64.1 & 46.4 & 48.3 & 8.6 & 2.3 & - \\
% Qwen-7B-Chat & 54.2 & 61.9 & 45.5 & 44.1 & 12.0 & 5.8 & - \\
% Qwen1.5-7B-Chat & 55.5 & 66.4 & 32.5 & 56.9 & 9.3 & 5.4 & - \\
% InternLM2-Chat-7B-SFT & 65.8 & {83.5} & 60.9 & 68.8 & 13.0 & {11.3} & - \\
% InternLM2-Chat-7B & {65.8} & 83.0 & {61.2} & {70.7} & {23.0} & 9.5 & 34.3 \\
% \multicolumn{8}{c}{\bluecolor{{$\heartsuit$ $\sim20B Models$}}} \\
% Llama2-13B-Chat & 50.8 & 57.0 & 49.7 & 43.1 & 5.2 & 1.1 & - \\
% Baichuan2-13B-Chat & 50.9 & 34.4 & 42.5 & 56.0 & 4.3 & 3.4 & 24.1 \\
% Mixtral-8x7B-Instruct-v0.1 & 60.9 & 80.3 & 57.3 & 71.7 & 22.5 & 9.6 & 32.1 \\
% Qwen-14B-Chat & 55.7 & 79.2 & 55.8 & 57.7 & 27.6 & 8.1 & - \\
% Qwen1.5-14B-Chat & 65.6 & 76.9 & 49.6 & 63.5 & 24.0 & 10.5 & 47.4 \\
% InternLM2-Chat-20B-SFT &{75.0} & {85.9} & 66.9 & 77.1 & 20.1 & 13.6 & 48.1 \\
% InternLM2-Chat-20B & 74.8 & 85.8 & {68.3} & {79.6} & {31.9} & {14.1} & {48.0} \\
% \hline
% \end{tabular}}
% \end{table*}

% \begin{table*}[!thb]
% \centering
% \caption{{Base Models Comparison on Reasoning Tasks: WinoGrande, HellaSwag, BBH}. Models are categorized by their parameter size and type, highlighting top performers in each category with {bold} for overall leaders and {underline} for leaders within their parameter group.}
% \vspace{-2mm}
% \label{tab:chat_reasoning_result}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{lccc}
% \hline
% {Models/Datasets} & {WinoGrande} & {HellaSwag} & {BBH} \\
% & {0-shot} & {0-shot} & {0-shot} \\
% \hline
% \multicolumn{4}{c}{\purplecolor{{\ding{72}API Models}}} \\
% GPT-3.5 & 68.7 & 70.2 & 41.9 \\
% \multicolumn{4}{c}{\greencolor{{$\triangle$ $\sim7B Models$}}} \\
% ChatGLM3-6B & 61.7 & 73.1 & 56.0 \\
% Llama2-7B-Chat & 51.5 & 49.5 & 41.4 \\
% Baichuan2-7B-Chat & 49.9 & 36.4 & 35.9 \\
% Mistral-7B-Instruct-v0.2 & 50.8 & 64.1 & 46.4 \\
% Qwen-7B-Chat & 54.2 & 61.9 & 45.5 \\
% Qwen1.5-7B-Chat & 55.5 & 66.4 & 32.5 \\
% InternLM2-Chat-7B-SFT & 65.8 & {83.5} & 60.9 \\
% InternLM2-Chat-7B & {65.8} & 83.0 & {61.2} \\
% \multicolumn{4}{c}{\bluecolor{{$\heartsuit$ $\sim20B Models$}}} \\
% Llama2-13B-Chat & 50.8 & 57.0 & 49.7 \\
% Baichuan2-13B-Chat & 50.9 & 34.4 & 42.5 \\
% Mixtral-8x7B-Instruct-v0.1 & 60.9 & 80.3 & 57.3 \\
% Qwen-14B-Chat & 55.7 & 79.2 & 55.8 \\
% Qwen1.5-14B-Chat & 65.6 & 76.9 & 49.6 \\
% InternLM2-Chat-20B-SFT & {75.0} & {85.9} & 66.9 \\
% InternLM2-Chat-20B & 74.8 & 85.8 & {68.3} \\
% \hline
% \end{tabular}}
% \end{table*}


% \begin{table*}[!thb]
% \centering
% \caption{{Base Models Comparison on Math \& Advanced Reasoning Tasks: GSM-8K, MATH, TheoremQA, MathBench-CN, MathBench-EN}. Models are categorized by their parameter size and type, highlighting top performers in each category with {bold} for overall leaders and {underline} for leaders within their parameter group.}
% \vspace{-2mm}
% \label{tab:base_math_result}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{lccccc}
% \hline
% {Models/Datasets} & {GSM-8K} & {MATH} & {TheoremQA} & {MathBench-CN}& {MathBench-EN}\\
% & {4-shot} & {4-shot}& {0-shot} & {0-shot\&8-shot}& {0-shot\&8-shot}\\
% \hline
% \multicolumn{6}{c}{\purplecolor{{\ding{72}API Models}}} \\
% GPT-3.5 & 24.6 & 5.5 & 1.6 & - \\
% \multicolumn{6}{c}{\greencolor{{$\triangle$ $\sim7B Models$}}} \\
% ChatGLM3-6B & 53.8 & 20.4 & 9.3 & - \\
% Llama2-7B-Chat & 28.4 & 4.1 & 0.3 & - \\
% Baichuan2-7B-Chat & 32.4 & 5.7 & 2.4 & - \\
% Mistral-7B-Instruct-v0.2 & 48.3 & 8.6 & 2.3 & - \\
% Qwen-7B-Chat & 44.1 & 12.0 & 5.8 & - \\
% Qwen1.5-7B-Chat & 56.9 & 9.3 & 5.4 & - \\
% InternLM2-Chat-7B-SFT & 68.8 & 13.0 & {11.3} & - \\
% InternLM2-Chat-7B & {70.7} & {23.0} & 9.5 & 34.3 \\
% \multicolumn{6}{c}{\bluecolor{{$\heartsuit$ $\sim20B Models$}}} \\
% Llama2-13B-Chat & 43.1 & 5.2 & 1.1 & - \\
% Baichuan2-13B-Chat & 56.0 & 4.3 & 3.4 & 24.1 \\
% Mixtral-8x7B-Instruct-v0.1 & 71.7 & 22.5 & 9.6 & 32.1 \\
% Qwen-14B-Chat & 57.7 & 27.6 & 8.1 & - \\
% Qwen1.5-14B-Chat & 63.5 & 24.0 & 10.5 & 47.4 \\
% InternLM2-Chat-20B-SFT & 77.1 & 20.1 & 13.6 & 48.1 \\
% InternLM2-Chat-20B & {79.6} & {31.9} & {14.1} & {48.0} \\
% \hline
% \end{tabular}}
% \end{table*}


\begin{table*}[!t]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|c|ccccc|c}
\multirow{2}{*}{model name} & \multirow{2}{*}{\#param}  & {GSM8K} & {MATH} & {TheoremQA} & {MathBench-CN}& {MathBench-EN} & \multirow{2}{*}{avg.} \\
& & (4-shot) & (4-shot) & (0-shot) & (0-shot\&8-shot) & (0-shot\&8-shot) & \\
\hline
% \multicolumn{7}{c}{\purplecolor{{\ding{72}API Models}}} \\
GPT-3.5 & -- & 78.2 & 28.0 & 9.1 & 26.4 & 42.5 & 36.8\\
\hline
% \multicolumn{7}{c}{\greencolor{{$\triangle$ $\sim7B\ Models$}}} \\
Llama2-7B-Chat & 7B & 28.4 & 4.1 & 0.3 & 3.3 & 7.7 & 8.8 \\
Llama2-13B-Chat & 13B & 43.1 & 5.2 & 1.1 & 6.7 & 15.7 & 14.4\\

Mistral-7B-Instruct-v0.2 & 7.3B & 48.3 & 8.6 & 2.3 & 14.5 & 28.3 & 20.4\\
Mixtral-8x7B-Instruct-v0.1 & 46.7B & 71.7 & 22.5 & 9.6 & 27.2 & 44.3 & 35.1 \\

Baichuan2-7B-Chat & 7B & 32.4 & 5.7 & 2.4 & 16.9 & 17.8  & 15.0\\
Baichuan2-13B-Chat & 13B & 56.0 & 4.3 & 3.4 & 28.3 & 29.1 & 24.2\\

Qwen-7B-Chat & 7B & 44.1 & 12.0 & 5.8 & 31.2 & 29.0 & 24.4 \\
Qwen-14B-Chat & 14B & 57.7 & 27.6 & 8.1 & 47.1 & 40.6 & 36.2 \\

ChatGLM3-6B & 6.2B & 53.8 & 20.4 & 9.3 & 18.2 & 21.7 & 24.7 \\
% Qwen1.5-7B-Chat & 56.9 & 9.3 & 5.4 & 38.0 & 34.2 \\
% \multicolumn{7}{c}{\bluecolor{{$\heartsuit$ $\sim20B\  Models$}}} \\
% Qwen1.5-14B-Chat & 63.5 & 24.0 & 10.5 & {52.0} & {50.8} \\
\hline
\rowcolor{gray!15}
InternLM2-Chat-7B-SFT & 7B & 68.8 & 23.2 & {11.3} & {43.1} & 40.1 & {37.3} \\
\rowcolor{gray!15}
InternLM2-Chat-7B & 7B & {70.7} & {23.6} & 9.5 & 38.0 & {42.3} & 36.8 \\
\rowcolor{gray!15}
InternLM2-Chat-20B-SFT & 20B & 77.1 & 31.9 & 13.6 & 47.5 & {50.6} & 44.1 \\
\rowcolor{gray!15}
InternLM2-Chat-20B & 20B & {79.6} & {32.4} & {14.1} & {48.0} & 48.5 & {44.5} \\
\end{tabular}}
\caption{\textbf{Comparison of chat models on math tasks}. }
\vspace{-2mm}
\label{tab:chat_math_result}
\end{table*}





==> table/finetuning_datasets.tex <==
\begin{table*}[t!]
\centering
{
\renewcommand{\arraystretch}{0.97}
\fontsize{8}{10}\selectfont 
\setlength\tabcolsep{3.5pt}
\begin{tabular}{l|l}
Task &  Dataset \\
\hline
\multicolumn{2}{l}{\emph{Type: Single-Image Datasets}} \\
                              & TextCaps (en)~\cite{sidorov2020textcaps}, 
                              ShareGPT4o (en \& zh)~\cite{chen2024far}, 
                              InternVL-SA-1B-Caption (en \& zh)~\cite{chen2023internvl}, \\
\multirow{-2}{*}{Captioning}
                              & NewYorkerCaptionContest (en)~\cite{hessel2023androids},
                              MMInstruct (en \& zh)~\cite{liu2024mminstruct}  \\
\rowcolor{gray!15}
                              & VQAv2 (en)~\cite{goyal2017vqav2}, 
                              GQA (en)~\cite{hudson2019gqa}, 
                              OKVQA (en)~\cite{marino2019okvqa}, 
                              Visual7W (en)~\cite{zhu2016visual7w}, 
                              MMInstruct (en \& zh)~\cite{liu2024mminstruct}, \\
\rowcolor{gray!15}
\multirow{-2}{*}{General QA}
                              &  VSR (en)~\cite{liu2023vsr},
                              FSC147 (en)~\cite{ranjan2021learning},
                              Objects365-YorN (en)~\cite{shao2019objects365}, 
                              Hateful-Memes (en)~\cite{kiela2020hateful} \\
                              & GeoQA+ (en)~\cite{cao2022geoqa_plus}, 
                              CLEVR-Math (en)~\cite{lindstrom2022clevrmath}, 
                              Super-CLEVR (en)~\cite{li2023superclevr},
                              MapQA (en)~\cite{chang2022mapqa}, 
                              MAVIS (en)~\cite{zhang2024mavis}, \\ 
                              & Geometry3K (en)~\cite{lu2021geometry3k}, 
                              TallyQA (en)~\cite{acharya2019tallyqa}, 
                              MetaMath (en)~\cite{yu2023metamath}, 
                              GEOS (en)~\cite{seo2015solving}, 
                              UniGeo (en)~\cite{chen2022unigeo}, \\
\multirow{-3}{*}{Mathematics} 
                              & 
                              GeomVerse (en)~\cite{kazemi2023geomverse}, 
                              CMM-Math (zh)~\cite{liu2024cmmmath}  \\
                              
\rowcolor{gray!15}
                              & ChartQA (en)~\cite{masry2022chartqa}, 
                              MMTab (en)~\cite{zheng2024multimodal}, 
                              PlotQA (en)~\cite{methani2020plotqa}, 
                              FigureQA (en)~\cite{kahou2017figureqa}, 
                              VisText (en)~\cite{tang2023vistext},  \\
\rowcolor{gray!15}
                              & LRV-Instruction (en)~\cite{liu2023lrv-instruction}, 
                              ArxivQA (en)~\cite{li2024multimodal}, 
                              TabMWP (en)~\cite{lu2022tablemwp}, 
                              MMC-Inst (en)~\cite{liu2023mmc},
                              DVQA (en)~\cite{kafle2018dvqa},\\
\rowcolor{gray!15}
                              & UniChart (en)~\cite{masry2023unichart}, 
                              SimChart9K (en)~\cite{xia2023structchart}, 
                              Chart2Text (en)~\cite{obeid2020chart}, 
                              FinTabNet (zh)~\cite{zheng2021global},
                              SciTSR (zh)~\cite{chi2019complicated}, \\
\rowcolor{gray!15}
\multirow{-4}{*}{Chart}
                              & \textcolor{gray}{Synthetic Chart2Markdown (en)}  \\
                              & 
                              OCRVQA (en)~\cite{mishra2019ocrvqa}, 
                              InfoVQA (en)~\cite{mathew2022infographicvqa}, 
                              TextVQA (en)~\cite{singh2019textvqa}, 
                              ArT (en \& zh)~\cite{chng2019art}, 
                              HME100K (en)~\cite{yuan2022syntax},  \\ 
                              & COCO-Text (en)~\cite{veit2016coco}, 
                              CTW (zh)~\cite{yuan2019ctw}, 
                              LSVT (zh)~\cite{sun2019lsvt}, 
                              RCTW-17 (zh)~\cite{shi2017rctw17}, 
                              VCR (en \& zh)~\cite{zhang2024vcr}, \\ 
                              & EST-VQA (en \& zh)~\cite{wang2020general}, 
                              ST-VQA (en)~\cite{biten2019stvqa}, 
                              EATEN (zh)~\cite{guo2019eaten}, 
                              LLaVAR (en)~\cite{zhang2023llavar}, 
                              CASIA (zh)~\cite{liu2020casia},  \\
                              & Chinese-OCR (zh)~\cite{chinese-ocr}, 
                              CyrillicHandwriting (ru)~\cite{cyrillic}, 
                              IAM (en)~\cite{marti2002iam}, 
                              NAF (en)~\cite{davis2019deep}, 
                              POIE (en)~\cite{kuang2023visual}, \\
                              & ReCTs (zh)~\cite{zhang2019rects}, 
                              MTWI (zh)~\cite{he2018icpr2018}, 
                              TextOCR (en)~\cite{singh2021textocr}, 
                              SROIE (en)~\cite{huang2019icdar2019}, 
                              \textcolor{gray}{Synthetic Arxiv OCR (en)}, \\
                              & MTVQA (ko \& ja \& it \& ru \& de \& fr \& th \& ar \& vi)~\cite{tang2024mtvqa}, 
                              \textcolor{gray}{Synthetic Image2Latex (en)}, 
                              \\ 
\multirow{-7}{*}{OCR}         & \textcolor{gray}{Synthetic Handwritten OCR (zh)}, 
                              \textcolor{gray}{Synthetic Infographic2Markdown (en \& zh)} \\
\rowcolor{gray!15}
                              & KVQA (en)~\cite{shah2019kvqa}, 
                              A-OKVQA (en)~\cite{schwenk2022aokvqa}, 
                              ViQuAE (en)~\cite{lerner2022viquae}, 
                              iNaturalist2018 (en)~\cite{van2018inaturalist},
                              MovieNet (en)~\cite{huang2020movienet}, \\
\rowcolor{gray!15}
\multirow{-2}{*}{Knowledge} 
                              & ART500K (en)~\cite{mao2017deepart}, 
                              KonIQ-10K (en)~\cite{hosu2020koniq},
                              \textcolor{gray}{Synthetic Multidisciplinary Knowledge / QA (en \& zh)} \\
Document
                              & DocVQA (en)~\cite{clark2017docqa}, 
                              Docmatix (en)~\cite{2024docmatrix}, 
                              DocReason25K (en)~\cite{hu2024mplug_docowl_1_5}, 
                              Sujet-Finance-QA-Vision (en)~\cite{sujet-finance} \\
\rowcolor{gray!15}
                              & RefCOCO/+/g (en)~\cite{yu2016refcoco,mao2016generation}, 
                              GPT4Gen-RD-BoxCoT (en)~\cite{chen2023shikra}, 
                              All-Seeing-V2 (en)~\cite{wang2024allseeingv2}, \\
\rowcolor{gray!15}
\multirow{-2}{*}{Grounding}   
                              & V3Det (en \& zh)~\cite{wang2023v3det}, 
                              DsLMF (en)~\cite{yang2023open}, 
                              COCO-ReM (en \& zh)~\cite{singh2025benchmarking}, 
                              TolokaVQA (en)~\cite{ustalov2023toloka} \\
\multirow{-1}{*}{Science}     & AI2D (en)~\cite{kembhavi2016ai2d}, 
                              ScienceQA (en)~\cite{lu2022scienceqa}, 
                              TQA (en)~\cite{kembhavi2017tqa}, 
                              ChemVLM Data (en \& zh)~\cite{li2024chemvlm} \\
\rowcolor{gray!15}
                              & ALLaVA (en \& zh)~\cite{chen2024allava}, 
                              Viet-ShareGPT4o (vi)~\cite{doan2024vintern}, 
                              Cambrain-GPT4o (en)~\cite{tong2024cambrian} , 
                              RLAIF-V (en)~\cite{yu2024rlaifv}, \\ 
\rowcolor{gray!15}
                              & Laion-GPT4V (en)~\cite{laion_gpt4v_dataset}, 
                              TextOCR-GPT4V (en)~\cite{textocr_gpt4v_dataset}, 
                              WildVision-GPT4o (en)~\cite{lu2024wildvision}, \\
\rowcolor{gray!15}
\multirow{-3}{*}{Conversation}& \textcolor{gray}{Synthetic Real-World Conversations (en \& zh)}  \\
                              & PMC-VQA (en)~\cite{zhang2023pmc}, 
                              VQA-RAD (en)~\cite{lau2018dataset}, 
                              ImageCLEF (en)~\cite{garcia2015overview}, 
                              PMC (en)~\cite{wu2023towards}, 
                              SLAKE (en \& zh)~\cite{liu2021slake}, \\
                              & GMAI-VL (en \& zh)~\cite{li2024gmai},
                              VQA-Med (en)~\cite{ben2019vqa},
                              Medical-Diff-VQA (en)~\cite{hu2023medical},
                              PathVQA (en)~\cite{he2020pathvqa}, \\
\multirow{-3}{*}{Medical}
                              & PMC-CaseReport (en)~\cite{pmccase}\\
\rowcolor{gray!15}
                             & Screen2Words (en)~\cite{wang2021screen2words}, 
                              WebSight (en)~\cite{laurenccon2024unlocking},
                              Widget-Caption (en)~\cite{li2020widget},
                              RICOSCA (en)~\cite{deka2017rico}, \\
\rowcolor{gray!15}
                              & Seeclick (en)~\cite{cheng2024seeclick},
                              ScreenQA (en)~\cite{hsiao2022screenqa},
                              AMEX (en)~\cite{chai2024amex},
                              AITW (en)~\cite{rawles2024androidinthewild},
                              Odyssey (en)~\cite{lu2024gui}, \\
\rowcolor{gray!15}
\multirow{-3}{*}{GUI}
                              & UIBert (en)~\cite{bai2021uibert},
                              AndroidControl (en)~\cite{lieffects},
                              Mind2Web (en)~\cite{deng2024mind2web},
                              OmniACT (en)~\cite{kapoor2025omniact}, 
                              WaveUI (en)~\cite{agentsea_wave_ui} \\
\hline
\multicolumn{2}{l}{\emph{Type: Multi-Image Datasets}}    \\
                              & Img-Diff (en)~\cite{jiao2024img}, 
                              Birds-to-Words (en)~\cite{jiang2024mantis}, 
                              Spot-the-Diff (en)~\cite{jiang2024mantis}, 
                              MultiVQA (en)~\cite{jiang2024mantis}, 
                              NLVR2 (en)~\cite{suhr2018corpus}, \\ 
\multirow{-2}{*}{General QA}   
                              & ContrastiveCaption (en)~\cite{jiang2024mantis}, 
                              DreamSim (en)~\cite{jiang2024mantis}, 
                              InternVL-SA-1B-Caption (en \& zh)~\cite{chen2023internvl} \\ 
\rowcolor{gray!15}
Document   
                              & MP-DocVQA (en)~\cite{tito2023hier}, 
                              MP-Docmatix (en)~\cite{2024docmatrix} \\
\hline
\multicolumn{2}{l}{\emph{Type: Video Datasets}}    \\
                              & Vript (en \& zh)~\cite{yang2024vript},
                              OpenVid (en)~\cite{nan2024openvid},
                              Mementos (en)~\cite{wang2024mementos}, 
                              ShareGPT4o-Video (en \& zh)~\cite{chen2024far}, \\ 
\multirow{-2}{*}{Captioning} 
                              & 
                              ShareGPT4Video (en \& zh)~\cite{chen2024sharegpt4video},
                              VideoGPT+ (en)~\cite{Maaz2024VideoGPT+} \\
\rowcolor{gray!15}
                              & VideoChat2-IT (en \& zh)~\cite{li2023videochat,li2024mvbench}, 
                              EgoTaskQA (en)~\cite{jia2022egotaskqa}, 
                              NTU RGB+D (en)~\cite{liu2020ntu},
                              CLEVRER (en)~\cite{yi2019clevrer}, \\                              
\rowcolor{gray!15}
                              & LLaVA-Video (en)~\cite{zhang2024video}, 
                              FineVideo (en)~\cite{FineVideo}, 
                              PerceptionTest (en)~\cite{patraucean2024perception},
                              HiREST (en)~\cite{zala2023hierarchical},
                              STAR (en)~\cite{wu2024star},
                              \\
\rowcolor{gray!15}
\multirow{-3}{*}{General QA} 
                             & EgoSchema (en)~\cite{mangalam2023egoschema},
                             ScanQA (en)~\cite{azuma2022scanqa},
                             LSMDC (en)~\cite{rohrbach2015dataset}  \\ 
GUI 
                             & GUI-World (en)~\cite{chen2024gui}  \\

\hline
\multicolumn{2}{l}{\emph{Type: Text Datasets}}    \\


                              & UltraFeedback (en)~\cite{cui2023ultrafeedback}, 
                              UltraChat (en)~\cite{ding2023enhancing}, 
                              Unnatural-Instructions (en)~\cite{honovich2022unnatural}, 
                              NoRobots (en)~\cite{no_robots}, \\
                              & MOSS (en)~\cite{sun2023moss}, 
                              LIMA (en)~\cite{zhou2024lima},  
                              SlimOrca (en)~\cite{SlimOrca}, 
                              WizardLM-Evol-Instruct-70K (en)~\cite{xu2024wizardlm}, \\
                              & Llama-3-Magpie-Pro (en)~\cite{xu2024magpie}, 
                              Magpie-Qwen2-Pro (en \& zh)~\cite{xu2024magpie}, 
                              KOpen-HQ-Hermes-2.5-60K (ko)~\cite{MarkrAI_KOpen_HQ_Hermes_2.5_60K},  \\
                              & Firefly (zh)~\cite{Firefly}, 
                              Dolly (en)~\cite{conover2023free}, 
                              OpenAI-Summarize-TLDR (en)~\cite{CarperAI_openai_summarize_tldr},
                              Know-Saraswati-CoT (en)~\cite{knowrohit07_know_saraswati_cot}, \\
\multirow{-5}{*}{General QA} 
                              &  
                              FLAN (en)~\cite{wei2021finetuned}, 
                              FLANv2 (en \& zh)~\cite{chung2024scaling} \\

\rowcolor{gray!15}
                              & Code-Feedback (en)~\cite{opencodeinterpreter}, 
                              Glaive-Code-Assistant (en)~\cite{glaive_code_assistant_v3}, 
                              XCoder-80K (en)~\cite{wang2024xcoder80k},
                              LeetCode (en \& zh), \\
\rowcolor{gray!15}
\multirow{-2}{*}{Code}        
                              & Evol-Instruct-Code (en)~\cite{luo2023wizardcoder}, 
                              InternLM2-Code (en \& zh)~\cite{cai2024internlm2} \\

\multirow{2}{*}{Long Context}
                              & Long-Instruction-with-Paraphrasing (en \& zh)~\cite{yu2023paraphrasing}, 
                              LongCite (en \& zh)~\cite{zhang2024longcite}, 
                              LongQLoRA (en)~\cite{yang2023longqlora}, \\ & 
                              LongAlpaca (en)~\cite{long-alpaca}  \\

\rowcolor{gray!15}
                              & GSM8K-Socratic (en)~\cite{cobbe2021training}, 
                              NuminaMath-CoT/TIR (en)~\cite{li2024numinamath}, 
                              Orca-Math (en)~\cite{mitra2024orcamath}, 
                              MathQA (en)~\cite{amini2019mathqa},  \\
\rowcolor{gray!15}
\multirow{-2}{*}{Mathematics}
                              & InfinityMATH (en)~\cite{zhang2024inifinitymath},
                              InternLM2-Math (en \& zh)~\cite{cai2024internlm2} \\  

Knowledge
                              & \textcolor{gray}{Synthetic Multidisciplinary Knowledge / QA (en)} \\

\end{tabular}
\caption{
\textbf{Summary of the fine-tuning data mixture of InternVL 2.5.}
We expanded our fine-tuning data mixture through extensive collection of open-source datasets and self-synthesized data. This mixture is predominantly in English (en) and Chinese (zh), with smaller portions in other languages, including Korean (ko), Japanese (ja), Italian (it), Russian (ru), German (de), French (fr), Thai (th), Arabic (ar), and Vietnamese (vi).
}
\label{tab:finetuning_datasets}
}
\end{table*}


==> table/language_model_comparison.tex <==
\begin{table*}[!t]
\centering
\small
\renewcommand{\arraystretch}{0.95}
\setlength\tabcolsep{5pt}
{\fontsize{8}{10}\selectfont 
% \renewcommand{\arraystretch}{0.9}

\newcommand{\QwenOne}{\rotatebox{90}{\makecell{Qwen2.5-0.5B Chat}}}
\newcommand{\QwenTwo}{\rotatebox{90}{\makecell{Qwen2.5-1.5B Chat}}}
\newcommand{\QwenThree}{\rotatebox{90}{\makecell{Qwen2.5-7B Chat}}}
\newcommand{\QwenFour}{\rotatebox{90}{\makecell{Qwen2.5-14B Chat}}}
\newcommand{\QwenFive}{\rotatebox{90}{\makecell{Qwen2.5-32B Chat}}}
\newcommand{\QwenSix}{\rotatebox{90}{\makecell{Qwen2.5-72B Chat}}}

\newcommand{\InternVLThreeOne}{\rotatebox{90}{\makecell{InternVL3-1B}}}
\newcommand{\InternVLThreeTwo}{\rotatebox{90}{\makecell{InternVL3-2B}}}
\newcommand{\InternVLThreeThree}{\rotatebox{90}{\makecell{InternVL3-8B}}}
\newcommand{\InternVLThreeFour}{\rotatebox{90}{\makecell{InternVL3-9B}}}
\newcommand{\InternVLThreeFive}{\rotatebox{90}{\makecell{InternVL3-14B}}}
\newcommand{\InternVLThreeSix}{\rotatebox{90}{\makecell{InternVL3-38B}}}
\newcommand{\InternVLThreeSeven}{\rotatebox{90}{\makecell{InternVL3-78B}}}

% \begin{tabular}{l|rr|rr|rr|rr|rr|rr}
% Dataset                                                                & \QwenOne & \InternVLThreeOne & \QwenTwo & \InternVLThreeTwo & \QwenThree & \InternVLThreeThree & \QwenFour & \InternVLThreeFive & \QwenFive & \InternVLThreeSix & \QwenSix & \InternVLThreeSeven \\
% \midrule
% \begin{tabular}[c]{@{}l@{}}MMLU\\ 4d595a\end{tabular}             & 46.4         & 49.8         & 61.8         & 64.8         & 74.2       & 77.3         & 79.5        & 82.1          & 83.3        & 85.4          & 84.4        & 86.9          \\
% \begin{tabular}[c]{@{}l@{}}CMMLU\\ c13365\end{tabular}            & 47.2         & 56.7         & 62.9         & 72.2         & 78.8       & 84.4         & 82.6        & 85.8          & 85.8        & 88.7          & 87.4        & 89.9          \\
% \begin{tabular}[c]{@{}l@{}}C-Eval\\ 2daf24\end{tabular}           & 53.5         & 59.0         & 66.2         & 73.3         & 77.8       & 84.5         & 81.4        & 85.6          & 86.5        & 89.2          & 88.1        & 89.5          \\
% \begin{tabular}[c]{@{}l@{}}GAOKAO\\ 4c31db\end{tabular}           & 30.9         & 46.6         & 53.7         & 67.7         & 81.3       & 89.5         & 86.9        & 91.2          & 90.8        & 93.5          & 91.0        & 93.1          \\
% \midrule
% \begin{tabular}[c]{@{}l@{}}TriviaQA\\ 2121ce\end{tabular}         & 24.2         & 21.5         & 39.8         & 41.2         & 55.8       & 51.5         & 65.1        & 67.4          & 65.8        & 70.1          & 74.0        & 74.7          \\
% \begin{tabular}[c]{@{}l@{}}NaturalQuestions\\ 3dcea1\end{tabular} & 8.2          & 8.5          & 15.2         & 15.9         & 17.9       & 28.2         & 19.7        & 31.4          & 19.7        & 31.0          & 23.8        & 39.0          \\
% \begin{tabular}[c]{@{}l@{}}C3\\ 8c358f\end{tabular}               & 35.2         & 66.3         & 81.2         & 84.7         & 90.8       & 95.1         & 92.1        & 96.3          & 92.3        & 97.4          & 96.1        & 97.6          \\
% \begin{tabular}[c]{@{}l@{}}RACE-High\\ 69ee4f\end{tabular}        & 51.5         & 68.8         & 76.0         & 84.6         & 86.8       & 90.8         & 89.6        & 93.0          & 91.5        & 94.2          & 91.7        & 94.2          \\
% \midrule
% \begin{tabular}[c]{@{}l@{}}WinoGrande\\ b36770\end{tabular}       & 47.2         & 52.9         & 56.5         & 61.9         & 71.5       & 78.1         & 79.1        & 84.3          & 83.8        & 86.7          & 83.9        & 87.8          \\
% \begin{tabular}[c]{@{}l@{}}HellaSwag\\ e42710\end{tabular}        & 39.3         & 47.0         & 62.0         & 73.8         & 85.4       & 90.2         & 90.5        & 93.0          & 92.1        & 95.5          & 92.7        & 95.6          \\
% \begin{tabular}[c]{@{}l@{}}BBH\\ 5b92b0\end{tabular}              & 21.5         & 34.5         & 39.7         & 52.0         & 65.7       & 77.4         & 73.0        & 82.5          & 85.5        & 87.7          & 85.4        & 85.2          \\
% \midrule
% \begin{tabular}[c]{@{}l@{}}GSM8K\\ 1d7fe4\end{tabular}            & 39.0         & 47.2         & 61.6         & 72.5         & 80.1       & 83.1         & 82.4        & 88.4          & 84.7        & 89.7          & 88.2        & 90.5          \\
% \begin{tabular}[c]{@{}l@{}}MATH\\ 393424\end{tabular}             & 27.8         & 32.7         & 49.3         & 57.3         & 72.6       & 72.2         & 73.7        & 76.3          & 81.1        & 65.1          & 81.4        & 78.9          \\
% \begin{tabular}[c]{@{}l@{}}TheoremQA\\ 6f0af8\end{tabular}        & 12.3         & 12.9         & 14.4         & 15.6         & 20.1       & 25.5         & 18.5        & 24.1          & 21.9        & 18.9          & 22.9        & 30.4          \\
% \midrule
% \begin{tabular}[c]{@{}l@{}}HumanEval\\ 8e312c\end{tabular}        & 27.4         & 39.0         & 51.8         & 62.8         & 82.3       & 78.1         & 81.1        & 78.1          & 89.0        & 87.8          & 87.2        & 82.3          \\
% \begin{tabular}[c]{@{}l@{}}MBPP\\ a447ff\end{tabular}             & 38.5         & 47.5         & 51.4         & 60.7         & 74.3       & 69.3         & 76.7        & 75.1          & 83.7        & 77.4          & 86.8        & 76.7          \\
% \begin{tabular}[c]{@{}l@{}}MBPP-CN\\ 9114d5\end{tabular}          & 19.6         & 30.6         & 34.4         & 45.8         & 64.4       & 64.4         & 75.4        & 67.2          & 77.8        & 75.4          & 76.0        & 76.0          \\
% \midrule
% Avg.                                                                   & 33.5         & 42.4         & 51.6         & 59.2         & 69.4       & 72.9         & 73.4        & 76.6          & 77.4        & 78.4          & 78.9        & 80.5         
% \end{tabular}

\begin{tabular}{ll|rr|rr|rr|rr|rr|rr}
% Dataset          & Split       & Qwen2.5-0.5B & InternVL3-1B & Qwen2.5-1.5B & InternVL3-2B & Qwen2.5-7B & InternVL3-8B & Qwen2.5-14B & InternVL3-14B & Qwen2.5-32B & InternVL3-38B & Qwen2.5-72B & InternVL3-78B \\
Dataset                         &  Version                                       & \QwenOne & \InternVLThreeOne & \QwenTwo & \InternVLThreeTwo & \QwenThree & \InternVLThreeThree & \QwenFour & \InternVLThreeFive & \QwenFive & \InternVLThreeSix & \QwenSix & \InternVLThreeSeven \\
\midrule
MMLU             & 4d595a & 46.4         & 49.8         & 61.8         & 64.8         & 74.2       & 77.3         & 79.5        & 82.1          & 83.3        & 85.4          & 84.4        & 86.9          \\
CMMLU            & c13365 & 47.2         & 56.7         & 62.9         & 72.2         & 78.8       & 84.4         & 82.6        & 85.8          & 85.8        & 88.7          & 87.4        & 89.9          \\
C-Eval           & 2daf24 & 53.5         & 59.0         & 66.2         & 73.3         & 77.8       & 84.5         & 81.4        & 85.6          & 86.5        & 89.2          & 88.1        & 89.5          \\
GAOKAO           & 4c31db & 30.9         & 46.6         & 53.7         & 67.7         & 81.3       & 89.5         & 86.9        & 91.2          & 90.8        & 93.5          & 91.0        & 93.1          \\
\midrule
TriviaQA         & 2121ce & 24.2         & 21.5         & 39.8         & 41.2         & 55.8       & 51.5         & 65.1        & 67.4          & 65.8        & 70.1          & 74.0        & 74.7          \\
NaturalQuestions & 3dcea1 & 8.2          & 8.5          & 15.2         & 15.9         & 17.9       & 28.2         & 19.7        & 31.4          & 19.7        & 31.0          & 23.8        & 39.0          \\
C3               & 8c358f & 35.2         & 66.3         & 81.2         & 84.7         & 90.8       & 95.1         & 92.1        & 96.3          & 92.3        & 97.4          & 96.1        & 97.6          \\
RACE-High        & 69ee4f & 51.5         & 68.8         & 76.0         & 84.6         & 86.8       & 90.8         & 89.6        & 93.0          & 91.5        & 94.2          & 91.7        & 94.2          \\
\midrule
WinoGrande       & b36770 & 47.2         & 52.9         & 56.5         & 61.9         & 71.5       & 78.1         & 79.1        & 84.3          & 83.8        & 86.7          & 83.9        & 87.8          \\
HellaSwag        & e42710 & 39.3         & 47.0         & 62.0         & 73.8         & 85.4       & 90.2         & 90.5        & 93.0          & 92.1        & 95.5          & 92.7        & 95.6          \\
BBH              & 5b92b0 & 21.5         & 34.5         & 39.7         & 52.0         & 65.7       & 77.4         & 73.0        & 82.5          & 85.5        & 87.7          & 85.4        & 85.2          \\
\midrule
GSM8K            & 1d7fe4 & 39.0         & 47.2         & 61.6         & 72.5         & 80.1       & 83.1         & 82.4        & 88.4          & 84.7        & 89.7          & 88.2        & 90.5          \\
MATH             & 393424 & 27.8         & 32.7         & 49.3         & 57.3         & 72.6       & 72.2         & 73.7        & 76.3          & 81.1        & 72.2          & 81.4        & 78.9          \\
TheoremQA        & 6f0af8 & 12.3         & 12.9         & 14.4         & 15.6         & 20.1       & 25.5         & 18.5        & 24.1          & 21.9        & 18.9          & 22.9        & 30.4          \\
\midrule
HumanEval        & 8e312c & 27.4         & 39.0         & 51.8         & 62.8         & 82.3       & 78.1         & 81.1        & 78.1          & 89.0        & 87.8          & 87.2        & 82.3          \\
MBPP             & a447ff & 38.5         & 47.5         & 51.4         & 60.7         & 74.3       & 69.3         & 76.7        & 75.1          & 83.7        & 77.4          & 86.8        & 76.7          \\
MBPP-CN          & 9114d5 & 19.6         & 30.6         & 34.4         & 45.8         & 64.4       & 64.4         & 75.4        & 67.2          & 77.8        & 75.4          & 76.0        & 76.0          \\
\midrule
Overall             & -           & 33.5         & 42.4         & 51.6         & 59.2         & 69.4       & 72.9         & 73.4        & 76.6          & 77.4        & 78.9          & 78.9        & 80.5         
\end{tabular}
}
\caption{\textbf{Comparison of language model performance across multiple benchmarks.} These results were obtained using the OpenCompass toolkit. We compare InternVL3 with  Qwen2.5 Chat models, whose corresponding pre-trained base models are employed as the initialization of the language component in InternVL3.  Please note that the evaluation scores of the Qwen2.5 series may differ from those officially reported, as we have adopted the prompt versions provided in the table across all datasets for OpenCompass evaluation.}

\label{tab:language_model_comparison}
\end{table*}


==> table/multi-modal_benchmark.tex <==
\begin{table*}[t!]
\scriptsize
\centering
\setlength\tabcolsep{0.9pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{l|c|c|ccccc|ccccccccc|c}
                                        & open-   &       & \multicolumn{5}{c|}{OCR-related  Benchmarks} & \multicolumn{9}{c|}{General Multimodal Benchmarks}  & \multicolumn{1}{c}{Math}\\

\multirow{-2}{*}{model} & source & \multirow{-2}{*}{\#param} & DocVQA        & ChartQA       & InfoVQA       & TextVQA       & OCRBench     & MME           & RWQA        & AI2D          & MMMU          & MMB-EN/CN                     & CCB           & MMVet         & SEED           & HallB         & MathVista \\
\hline
GPT-4V-1106~\cite{openai2023gpt4}    &   \no                & $-$ & 88.4          & 78.5	         & $-$           & 78.0          & 645          & 1926.6        &61.4          & 78.2          & 56.8          & 77.0 / 74.4                   & 46.5          & \textbf{67.6} & 71.6          & 46.5          &  49.9     \\ 
Gemini Ultra 1.0~\cite{team2023gemini} & \no           & $-$ & 90.9          & 80.8          & \textbf{80.3} & \textbf{82.3} & $-$          & $-$           &$-$           & 79.5          & \textbf{59.4} & $-$ / $-$                     & $-$           & $-$           & $-$           & $-$           &  53.0     \\
Gemini Pro 1.0~\cite{team2023gemini} & \no             & $-$ & 88.1          & 74.1          & 75.2          & 74.6          & 659          & 1933.4        &$-$           & 73.9          & 47.9          & 73.6 / 74.3                   & 52.5          & 64.3          & 70.7          & 45.2          &  45.2     \\
Gemini Pro 1.5~\cite{reid2024gemini1_5} & \no          & $-$ & 86.5          & 81.3          & 72.7          & 73.5          & $-$          & $-$           &67.5          & 80.3          & 58.5          & $-$ / $-$                     & $-$           & $-$           & $-$           & $-$           &  52.1     \\
Qwen-VL-Max~\cite{bai2023qwenvl} &   \no               & $-$ & \textbf{93.1} & 79.8	         & 73.4          & $-$           & 723          &\textbf{2433.6}&$-$           & 79.3          & 51.3          & 77.6 / 75.7                   & 63.5          & 66.6          & $-$           & 41.2          &  51.0     \\
Qwen-VL-Plus~\cite{bai2023qwenvl} &  \no               & $-$ & 91.4          & 78.1          & $-$           & $-$           & 694          & 2183.4        &$-$           & 75.9          & 45.2          & 67.0 / 70.7                   & 55.1          & 61.1          & 72.7          & 40.6          &  43.3     \\
Claude-3 Opus~\cite{claude3series2024} & \no           & $-$ & 89.3          & 80.8          & $-$           & $-$           & 694          & 1586.8        &49.8          & 88.1          & \textbf{59.4} & 63.3 / 59.2                   & 26.3          & 58.1          & $-$           & 37.8          &  50.5     \\
Claude-3 Sonnet~\cite{claude3series2024} & \no         & $-$ & 89.5          & 81.1          & $-$           & $-$	         & 646          & 1625.9        &51.9          & \textbf{88.7} & 53.1          & 67.8 / 64.2                   & 27.8          & $-$           & $-$           & 41.3          &  47.9     \\
Claude-3 Haiku~\cite{claude3series2024} & \no          & $-$ & 88.8          & 81.7          & $-$           & $-$           & 658          & 1453.2        &$-$           & 86.7          & 50.2          & 60.7 / 57.2                   & 24.5          & $-$           & $-$           & 39.2          &  46.4     \\
HPT Pro~\cite{hptpro2024}  &    \no                    & $-$ & $-$           & $-$           & $-$           & $-$           & $-$          & $-$           &$-$           & $-$           & 52.0          & 77.5 / 76.7                   & $-$           & $-$           & 73.1          & $-$           &  $-$      \\
MM1~\cite{mckinzie2024mm1}     &    \no                & 30B & $-$           & $-$           & $-$           & 73.5          & $-$          & 2069.0        &$-$           & $-$           & 44.7          & 75.1 / $-$~~~~                & $-$           & 48.7          & 72.1          & $-$           &  39.4	   \\
Step-1V~\cite{step1v2023}  &      \no                  & 100B& $-$           & $-$           & $-$           & $-$           & 625          & 2206.4        &$-$           & 79.2          & 49.9          & 80.7 / 79.9                   & \textbf{71.2} & 63.3          & 70.3	       & 48.4          &  44.8     \\
Grok-1.5V~\cite{xai2024grokv}   &   \no                & $-$ & 85.6          & 76.1          & $-$           & 78.1          & $-$          & $-$           &\textbf{68.7} & 88.3          & $-$           & $-$ / $-$                     & $-$           & $-$           & $-$           & $-$           &  52.8     \\
\hline
Text-Monkey~\cite{liu2024textmonkey} & \yes            & 10B & 66.7          & 59.9          & 28.6          & 64.3          & 561          & $-$           &$-$           & $-$           & $-$           & $-$ / $-$                     & $-$           & $-$           & $-$           & $-$           &  $-$      \\
DocOwl-1.5~\cite{hu2024mplug_docowl_1_5}  & \yes       & 8B  & 82.2          & 70.2          & 50.7          & 68.6          & 599          & $-$           &$-$           & $-$           & $-$           & $-$ / $-$                     & $-$           & $-$           & $-$           & $-$           &  $-$      \\
Mini-Gemini~\cite{li2024miniGemini} & \yes             & 35B & $-$           & $-$           & $-$           & ~~74.1*       & $-$          & 2141.0        &$-$           & $-$           & 48.0          & 80.6 / $-$~~~~                & $-$           & 59.3          & $-$           & $-$           &  43.3     \\
LLaVA-NeXT~\cite{liu2024llavanext}  & \yes             & 35B & 84.0          & 68.7          & 51.5          & ~~69.5*       & 574          & 2028.0        &$-$           & 74.9          & 51.1          & 81.1 / 79.0                   & 49.2          & 57.4          & 75.9	       & 34.8          &  46.5     \\
\rowcolor{gray!15}
InternVL 1.2 (ours)         &   \yes                   & 40B & 57.7          & 68.0          & 39.5          & ~~72.5*       & 569          & 2175.4        &67.5          & 79.0          & 51.6          & 82.2 / 81.2                   & 59.2          & 48.9          & 75.6          & 47.6          &  47.7     \\
\rowcolor{gray!15}
InternVL 1.5 (ours)       &     \yes                   & 26B & 90.9          & \textbf{83.8} & 72.5          & 80.6          & \textbf{724} & 2187.8        &66.0          & 80.7          & 45.2          & \textbf{82.2} / \textbf{82.0} & 69.8          & 62.8          & \textbf{76.0} & \textbf{49.3} &  \textbf{53.5} \\
% \hline

\end{tabular}
\caption{\textbf{Comparison with SoTA models on 16 multimodal benchmarks.}
% InternVL 1.5 achieves performance comparable to state-of-the-art MLLMs.
OCR-related benchmarks include: DocVQA test \cite{mathew2021docvqa}, ChartQA test \cite{masry2022chartqa}, InfographicVQA test \cite{mathew2022infographicvqa}, TextVQA val~\cite{singh2019textvqa}, and OCRBench~\cite{liu2023ocrbench}.
General multimodal benchmarks encompass: MME~\cite{fu2023mme}, RealWorldQA~\cite{xai2024grokv}, AI2D test~\cite{kembhavi2016ai2d}, MMMU val~\cite{yue2023mmmu}, MMBench-EN/CN test~\cite{liu2023mmbench}, CCBench dev~\cite{liu2023mmbench}, MMVet~\cite{yu2023mmvet}, SEED Image~\cite{li2023seed}, and HallusionBench~\cite{guan2023hallusionbench}. 
Additionally, the math dataset includes MathVista testmini~\cite{lu2023mathvista}.
* denotes that Rosetta OCR tokens are used in the testing of TextVQA.
The MME results we report are the sum of the perception and cognition scores.
The results of OCRBench, MMBench, CCBench, and HallusionBench are collected from the OpenCompass leaderboard~\cite{opencompass2023}.
}
\label{tab:sota_results}
\end{table*}

==> table/overall_compare.tex <==
\begin{table*}[t!]
\centering
{\fontsize{8}{10}\selectfont 
\renewcommand{\arraystretch}{0.94}
\setlength\tabcolsep{3.9pt}
\newcommand{\MMMU}{\makecell{MMMU\\(val)}}
\newcommand{\MMMUT}{\makecell{MMMU\\(test)}}
\newcommand{\MMMUPRO}{\makecell{MMMU-Pro\\(std10 / vision / overall)}}
\newcommand{\MathVista}{\makecell{MathVista\\(mini)}}
\newcommand{\MathVision}{\makecell{MATH-Vision\\(mini / full)}}
\newcommand{\MathVe}{\makecell{MathVerse\\(mini)}}
\newcommand{\MMMATH}{\makecell{MM-MATH\\(mini)}}
\newcommand{\Olympiad}{\makecell{Olympiad\\Bench}}
\newcommand{\TODO}{\textcolor{red}{TODO}}
\newcommand{\lsp}{--\ \ \ \ \ \ }
\newcommand{\rsp}{\ \ \ \ \ --~}
\begin{tabular}{l|cccc|ccc}
Model Name                                 &  \makecell{GPT-4o\\20240513}      &  \makecell{Claude-3.5\\Sonnet} &  \makecell{Step-1o } & \makecell{Gemini-2.5-Pro } & \makecell{InternVL2.5 \\78B } & \makecell{Qwen2.5-VL \\ 72B  } &  \makecell{InternVL3 \\78B } \\
\hline
\rowcolor{gray!15}
GPT-4o-20240513 \\
Claude-3.5-Sonnet  \\
\rowcolor{gray!15}
GLM-4v-Plus-20250111 \\
Step-1o \\ 
\rowcolor{gray!15}
Gemini-2.5-Pro \\ 
% Gemini-1.5-Pro \\ 
Qwen2.5-VL 72B \\
\rowcolor{gray!15}
InternVL2.5 78B \\
InternVL3 78B \\ 

\end{tabular}
}
\caption{\textbf{Performance of InternVL 3 and other advanced MLLMs.}
}
\label{tab:overall_compare}
\end{table*}

==> table/pretraining_datasets.tex <==
\begin{table*}[t!]
{\fontsize{8}{10}\selectfont 
    \centering
    \setlength{\tabcolsep}{3mm} 
    \renewcommand{\arraystretch}{0.95}
    \begin{tabular}{l|l}
         Task & Dataset \\
         \hline
\multicolumn{2}{l}{\emph{Type: Single/Multi-Image Datasets}} \\
                            & FaceCaption~\cite{dai202415m},
                            COCO-Caption~\cite{singh2025benchmarking},
                            OpenImages-Caption~\cite{kuznetsova2020openimage},
                            Objects365-Caption~\cite{shao2019objects365},
                            TextCap~\cite{sidorov2020textcaps},
                            \\
                            &Laion-ZH~\cite{schuhmann2022laion5b},
                            Laion-EN~\cite{schuhmann2022laion5b}, 
                            Laion-COCO~\cite{schuhmann2022laioncoco},
                            LLaVAR~\cite{zhang2023llavar}, 
                            InternVL-SA-1B-Caption~\cite{kirillov2023segment}, 
                            \\
\multirow{-2}{*}{Captioning}& 
                            MMInstruct~\cite{liu2024mminstruct},
                            GRIT-Caption~\cite{peng2023kosmos2},
                            ShareGPT4V~\cite{chen2023sharegpt4v},
                            LVIS-Instruct-4V~\cite{wang2023lvisinstruct4v},
                            ShareCaptioner~\cite{chen2023sharegpt4v},
                            \\
                            &
                            OmniCorpus~\cite{li2024omnicorpus},
                            ShareGPT4o~\cite{chen2024far}
                            \\

\rowcolor{gray!15}          
                            & GQA~\cite{hudson2019gqa},
                            OKVQA~\cite{marino2019okvqa},
                            A-OKVQA~\cite{schwenk2022aokvqa},
                            Visual7W~\cite{zhu2016visual7w},
                            VisText~\cite{tang2023vistext},
                            VSR~\cite{liu2023vsr},
                            TallyQA~\cite{acharya2019tallyqa},
                            \\
\rowcolor{gray!15}
\multirow{-2}{*}{General QA}   
                            & 
                            Objects365-YorN~\cite{shao2019objects365},
                            IconQA~\cite{lu2021iconqa},
                            Stanford40~\cite{yao2011human},
                            VisDial~\cite{das2017visdial},
                            VQAv2~\cite{goyal2017vqav2}, 
                            Hateful-Memes~\cite{kiela2020hateful} \\


                            & MAVIS~\cite{zhang2024mavis},
                            GeomVerse~\cite{kazemi2023geomverse},
                            % CLEVR-Math~\cite{lindstrom2022clevrmath}, 
                            MetaMath-Rendered~\cite{yu2023metamath}, 
                            MapQA~\cite{chang2022mapqa}, 
                            GeoQA+~\cite{cao2022geoqa_plus},
                            Geometry3K~\cite{lu2021geometry3k}, \\
\multirow{-2}{*}{Mathematics}
                            & UniGeo~\cite{chen2022unigeo},
                            GEOS~\cite{seo2015solving},
                            CLEVR-Math~\cite{lindstrom2022clevrmath}  \\

\rowcolor{gray!15}
                            & 
                            ChartQA~\cite{masry2022chartqa}, 
                            PlotQA~\cite{methani2020plotqa},
                            FigureQA~\cite{kahou2017figureqa},
                            LRV-Instruction~\cite{liu2023lrv-instruction}, 
                            ArxivQA~\cite{li2024multimodal},
                            MMC-Inst~\cite{liu2023mmc}, \\
\rowcolor{gray!15}
                            & TabMWP~\cite{lu2022tablemwp},
                            DVQA~\cite{kafle2018dvqa},
                            UniChart~\cite{masry2023unichart}, 
                            SimChart9K~\cite{xia2023structchart},
                            Chart2Text~\cite{obeid2020chart},
                            FinTabNet~\cite{zheng2021global}, \\
\rowcolor{gray!15}
\multirow{-3}{*}{Chart}                            
                            & SciTSR~\cite{chi2019complicated},
                            \textcolor{gray}{Synthetic Chart2Markdown}
                            \\
                            & 
                            LaionCOCO-OCR~\cite{schuhmann2022laioncoco}, 
                            Wukong-OCR~\cite{gu2022wukong},  
                            ParsynthOCR~\cite{hezarai_parsynth_ocr_200k},
                            SynthDoG-EN~\cite{kim2022synthdog},
                            SynthDoG-ZH~\cite{kim2022synthdog},
                            \\
                            & 
                            SynthDoG-RU~\cite{kim2022synthdog},
                            SynthDoG-JP~\cite{kim2022synthdog},
                            SynthDoG-KO~\cite{kim2022synthdog},
                            IAM~\cite{marti2002iam},
                            EST-VQA~\cite{wang2020general},
                            ST-VQA~\cite{biten2019stvqa}, \\
                            &
                            NAF~\cite{davis2019deep}, 
                            InfoVQA~\cite{mathew2022infographicvqa}, 
                            HME100K~\cite{yuan2022syntax},
                            OCRVQA~\cite{mishra2019ocrvqa}, 
                            SROIE~\cite{huang2019icdar2019},
                            POIE~\cite{kuang2023visual},
                            CTW~\cite{yuan2019ctw}, \\
                            & SynthText~\cite{gupta2016synthtext},
                            ArT~\cite{chng2019art}, 
                            LSVT~\cite{sun2019lsvt}, 
                            RCTW-17~\cite{shi2017rctw17}, 
                            ReCTs~\cite{zhang2019rects},
                            MTWI~\cite{he2018icpr2018}, 
                            TextVQA~\cite{singh2019textvqa}, \\
                            & CASIA~\cite{liu2020casia},
                            TextOCR~\cite{singh2021textocr}, 
                            Chinese-OCR~\cite{chinese-ocr}, 
                            EATEN~\cite{guo2019eaten},
                            COCO-Text~\cite{veit2016coco},
                            \textcolor{gray}{Synthetic Arxiv OCR},
                             \\
\multirow{-5}{*}{OCR} 
                            & 
                            \textcolor{gray}{Synthetic Image2Latex}, 
                            \textcolor{gray}{Synthetic Handwritten OCR}, 
                            \textcolor{gray}{Synthetic Infographic2Markdown} 
                            \\


\rowcolor{gray!15}
                            & KVQA~\cite{shah2019kvqa},
                            A-OKVQA~\cite{schwenk2022aokvqa},
                            ViQuAE~\cite{lerner2022viquae}, 
                            iNaturalist2018~\cite{van2018inaturalist}, 
                            MovieNet~\cite{huang2020movienet},
                            ART500K~\cite{mao2017deepart}, 
                            \\      
\rowcolor{gray!15}
                            & 
                            KonIQ-10K~\cite{hosu2020koniq},
                            IconQA~\cite{lu2021iconqa}, 
                            VisualMRC~\cite{tanaka2021visualmrc},
                            ChemVLM Data~\cite{li2024chemvlm},
                            ScienceQA~\cite{lu2022scienceqa},
                            AI2D~\cite{kembhavi2016ai2d}, \\
\rowcolor{gray!15}
\multirow{-3}{*}{Knowledge}
                            &
                            TQA~\cite{kembhavi2017tqa},
                            Wikipedia-QA~\cite{he2023wanjuan}, 
                            \textcolor{gray}{Synthetic Multidisciplinary Knowledge / QA} \\
                            & Objects365~\cite{shao2019objects365},
                            GRIT~\cite{you2023ferret}, 
                            RefCOCO~\cite{yu2016refcoco},
                            GPT4Gen-RD-BoxCoT~\cite{chen2023shikra},
                            All-Seeing-V1~\cite{wang2023allseeing}, \\
\multirow{-2}{*}{Grounding}
                            & 
                            All-Seeing-V2~\cite{wang2024allseeingv2},
                            V3Det~\cite{wang2023v3det},
                            TolokaVQA~\cite{ustalov2023toloka} \\

\rowcolor{gray!15}
Document
                            & DocReason25K~\cite{hu2024mplug_docowl_1_5},
                            DocVQA~\cite{mathew2021docvqa},
                            Docmatix~\cite{2024docmatrix}, 
                            \textcolor{gray}{Synthetic Arxiv QA} \\

                            & ALLaVA~\cite{chen2024allava},
                            SVIT~\cite{zhao2023svit},
                            Cambrain-GPT4o~\cite{tong2024cambrian},
                            TextOCR-GPT4V~\cite{textocr_gpt4v_dataset}, 
                            MMDU~\cite{liu2024mmdu}, \\
\multirow{-2}{*}{Conversation}
                            &
                            \textcolor{gray}{Synthetic Real-World Conversations}
                            \\

\rowcolor{gray!15}
                            & PMC-VQA~\cite{zhang2023pmc},
                            VQA-RAD~\cite{lau2018dataset},
                            ImageCLEF~\cite{garcia2015overview},
                            SLAKE~\cite{liu2021slake}, 
                            Medical-Diff-VQA~\cite{hu2023medical},\\
\rowcolor{gray!15}
\multirow{-2}{*}{Medical}
                            & PMC-CaseReport~\cite{pmccase},
                            GMAI-VL (subset)~\cite{li2024gmai}\\

GUI
% Infographic
                            & Screen2Words~\cite{wang2021screen2words},
                            WebSight~\cite{laurenccon2024unlocking} \\

\hline
\multicolumn{2}{l}{\emph{Type: Video Datasets}} \\

\rowcolor{gray!15}
Captioning                  & Mementos~\cite{wang2024mementos},
                            ShareGPT4Video~\cite{chen2024sharegpt4video},
                            VideoGPT+~\cite{Maaz2024VideoGPT+},
                            ShareGPT4o-Video~\cite{chen2024far} \\
                            
General QA                  & VideoChat2-IT~\cite{li2024mvbench},
                            EgoTaskQA~\cite{jia2022egotaskqa},
                            NTU RGB+D~\cite{liu2020ntu},
                            CLEVRER~\cite{yi2019clevrer},
                            STAR~\cite{wu2024star}, 
                            LSMDC~\cite{rohrbach2015dataset} \\
    \end{tabular}
    \caption{\textbf{Summary of the pre-training data mixture of InternVL 2.5.}
    Notably, we exclusively use conversaiton-format instruction data, and at this stage, only the MLP or both MLP and ViT parameters are trainable, allowing the incorporation of both low-quality and high-quality data.
    } 
\label{tab:pretraining_datasets}
}
\end{table*}


% 没找到的
% % japanese_ocr
% % image_textualization
% % diagram_image_to_text_gpt4o
% % chrome_writting
% mmmu\_data
% * xueersi\_\*
% % latex10k_qa_20240805
% % pixel_art_instruction_gpt4o_filtered
% 爬虫 crawler\_data2
% crawler\_data
% gaokao/文件夹里面的
% ocr\_st/文件夹
% % mmmu_tiku_gpt4o_20240626_18k_filtered
% % reflux_20240510_to_20240621_gpt4o_filtered
% % mmmu_baidu_image_caption_gpt4o_filtered
% % EdrawSVG_Caption_13K_v1
% % coco_clothes_zh_20240402

% CAR-A_20240621

% safety_20240619
% study_com_image_20240619
% reflow_gpt4o_correct_shanghai_0510_To_0523_filtered
% reflow_gpt4o_correct_shanghai_0212_To_0510_filtered

% Pathology_VQA
% medical_longanswer_*
% SenseChat_Vision_0429_To_0517_gpt4o_filtered st的？
% GPT4o_LongCaption_20240819_90k_v1.0_reformat
% GPT4o_LongCaption_20240819_v1.0_reformat
% llavar\_inhous不管
% AndroidUI_longcaption_0312to0327_20240409_v1 这个是private？
% ocr/pdf60k_cn_v1.0_woBox.jsonl
% synth_handwrite_small_500k_v1.0.jsonl
% irregular_layout_v1.0_woBox.jsonl
% industry_research_report_woBox_v1.0.jsonl
% EdrawSVG2PNG
% charts2500_qa_v1.jsonl
% ocr-st/eastmoney3k_qa_20240621_v1.jsonl
% ccbench_inhouse_20240401_v2
% inhouse没有
% ctrip_food_qa_zh_20240624_gpt4o_filtered
% ctrip_food_longcap_zh_20240624_gpt4o_filtered
% ctrip_insight_gpt4v_zh_20240402
% douban_movie_qa_zh_gpt4o_20240625_filtered
% douban_movie_longcap_gpt4o_20240624_filtered
% coco_poetry_zh_20240402
% vqa_rad_en_20240402
% pic_math2k/images 合成数据
% Baidu_Baike_500k_zh_20240402_filtered_v2
% chart_data_with_markdown.jsonl


==> table/stage12_data.tex <==
\begin{table}[t]
    \scriptsize
    \centering
    \renewcommand\arraystretch{1.0} % Line spacing
    \setlength{\tabcolsep}{1.1mm}    % table col width
    \begin{tabular}{l|cc|cc|cc}
          & \multicolumn{2}{c|}{characteristics} & \multicolumn{2}{c|}{stage 1}  & \multicolumn{2}{c}{stage 2} \\
         \multirow{-2}{*}{dataset} & language & original & cleaned & remain  & cleaned & remain \\
         \hline
         LAION-en~\cite{schuhmann2022laion5b}  & \multirow{6}{*}{English} & 2.3B & 1.94B & 84.3\% &  91M & 4.0\% \\
         LAION-COCO~\cite{schuhmann2022laioncoco}  &  & 663M     & 550M   & 83.0\% & 550M & 83.0\% \\
         COYO~\cite{byeon2022coyo}        &  & 747M     & 535M   & 71.6\% & 200M & 26.8\% \\
         CC12M~\cite{changpinyo2021cc12m}       &  & 12.4M      & 11.1M  & 89.5\% & 11.1M  & 89.5\% \\
         CC3M~\cite{sharma2018cc3m}        &  & 3.0M       & 2.6M   & 86.7\% & 2.6M   & 86.7\%  \\
         SBU~\cite{ordonez2011sbu}
         &  & 1.0M & 1.0M & 100\% & 1.0M & 100\% \\
         
         \rowcolor{gray!15}
         Wukong~\cite{gu2022wukong}& \multirow{1}{*}{Chinese} & 100M  & 69.4M & 69.4\% & 69.4M & 69.4\% \\
         
         LAION-multi~\cite{schuhmann2022laion5b} & \multirow{1}{*}{Multi} & 2.2B  & 1.87B & 85.0\% & 100M & 4.5\%\\
         \hline
          Total      &  Multi & 6.03B     & 4.98B    & 82.6\% & 1.03B & 17.0\%\\
    \end{tabular}
    \vspace{-0.5em}
    \caption{\textbf{Details of the training data for \modelname in stage 1 and stage 2.}
    Among them, LAION-en~\cite{schuhmann2022laion5b}, LAION-multi~\cite{schuhmann2022laion5b}, COYO~\cite{byeon2022coyo}, and Wukong~\cite{gu2022wukong} are web-scale image-text pairs data.
    LAION-COCO~\cite{schuhmann2022laioncoco} is a synthetic dataset with high-quality captions from LAION-en. CC12M~\cite{changpinyo2021cc12m}, CC3M~\cite{sharma2018cc3m}, SBU~\cite{ordonez2011sbu} are academic caption datasets. ``Multi" means multilingual.
    } 
    \vspace{-0.5em}
    \label{tab:stage1_data}
    % \vspace{-0.5em}
\end{table}

==> table/train_hyperparam.tex <==
\begin{table*}[t!]
\centering
{\fontsize{8}{10}\selectfont 
\newcommand{\Pretrain}{\makecell{Pre-train\\Mixture}}
\newcommand{\Finetune}{\makecell{Fine-tune\\Mixture}}
\renewcommand{\arraystretch}{1.0}
{\setlength\tabcolsep{2.8pt}
\begin{tabular}{l|cc|cc|cc|ccc}
\multirow{2}{*}{Settings}         & \multicolumn{2}{c|}{InternVL2.5-1B} & \multicolumn{2}{c|}{InternVL2.5-2B} & \multicolumn{2}{c|}{InternVL2.5-4B} & \multicolumn{3}{c}{InternVL2.5-8B}       \\
                                  & Stage 1    & Stage 2                & Stage 1          & Stage 2          & Stage 1          & Stage 2          & Stage 1     & Stage 1.5    & Stage 2     \\
\hline
Dataset                           & \Pretrain  & \Finetune              & \Pretrain        & \Finetune        & \Pretrain        & \Finetune        & \Pretrain   & \Pretrain    & \Finetune   \\
Trainable                         & MLP        & Full Model             & MLP              & Full Model       & MLP              & Full Model       & MLP         & ViT+MLP      & Full Model  \\
% Packed Dataset                  & \yes       & \yes                   & \yes             & \yes             & \yes             & \yes             & \yes        & \yes         & \yes        \\
Packed Batch Size                 & 512        & 512                    & 512              & 512              & 512              & 512              & 512         & 1024         & 512         \\
Learning Rate                     & 2e-4       & 4e-5                   & 2e-4             & 4e-5             & 2e-4             & 4e-5             & 2e-4        & 1e-5         & 4e-5        \\
Context Length                    & 16384      & 16384                  & 16384            & 16384            & 16384            & 16384            & 16384       & 16384        & 16384       \\
% Length Threshold                & 16384      & 16384                  & 16384            & 16384            & 16384            & 16384            & 16384       & 16384        & 16384       \\
Image Tile Threshold              & 48         & 48                     & 48               & 48               & 48               & 48               & 48          & 48           & 48          \\
ViT Drop Path                     & 0.0        & 0.1                    & 0.0              & 0.1              & 0.0              & 0.1              & 0.0         & 0.1          & 0.1         \\
Weight Decay                      & 0.01       & 0.01                   & 0.01             & 0.01             & 0.01             & 0.01             & 0.05        & 0.05         & 0.05        \\
Training Epochs                   & --         & 4                      & --               & 4                & --               & 2                & --          & --           & 1           \\
\hline
Training Tokens                   & $\sim$191B & $\sim$176B             & $\sim$277B       & $\sim$176B       & $\sim$164B        & $\sim$88B        & $\sim$22B   & $\sim$76B    & $\sim$44B  \\
\end{tabular}
}

\bigskip

{
\setlength\tabcolsep{8pt}
\begin{tabular}{l|ccc|cc|cc}
\multirow{2}{*}{Settings}         & \multicolumn{3}{c|}{InternVL2.5-26B}   & \multicolumn{2}{c|}{InternVL2.5-38B} & \multicolumn{2}{c}{InternVL2.5-78B} \\
                                  & Stage 1    & Stage 1.5    & Stage 2    & Stage 1          & Stage 2           & Stage 1          & Stage 2          \\
\hline
Dataset                           & \Pretrain  & \Pretrain    & \Finetune  & \Pretrain        & \Finetune         & \Pretrain        & \Finetune        \\
Trainable                         & MLP        & ViT+MLP      & Full Model & MLP              & Full Model        & MLP              & Full Model       \\
% Packed Dataset                  & \yes       & \yes         & \yes       & \yes             & \yes              & \yes             & \yes             \\
Packed Batch Size                 & 512        & 1024         & 512        & 512              & 512               & 512              & 512              \\
Learning Rate                     & 2e-4       & 1e-5         & 2e-5       & 2e-4             & 2e-5              & 2e-4             & 2e-5             \\
Context Length                    & 16384      & 16384        & 16384      & 16384            & 16384             & 16384            & 16384            \\
% Length Threshold                & 16384      & 16384        & 16384      & 16384            & 16384             & 16384            & 16384            \\
Image Tile Threshold              & 48         & 48           & 48         & 48               & 48                & 48               & 48               \\
ViT Drop Path                     & 0.0        & 0.4          & 0.4        & 0.0              & 0.4               & 0.0              & 0.4              \\
Weight Decay                      & 0.05       & 0.05         & 0.05       & 0.05             & 0.05              & 0.05             & 0.05             \\
Training Epochs                   & --         & --           & 1          & --               & 1                 & --               & 1                \\
\hline
Training Tokens                   & $\sim$31B  & $\sim$146B   & $\sim$44B  & $\sim$107B       & $\sim$44B         & $\sim$76B        & $\sim$44B        \\
\end{tabular}
}
}
\caption{\textbf{Training configurations and hyperparameters for InternVL 2.5.} 
This table presents the training setups for various scales of InternVL 2.5 models. 
The configurations are carefully optimized to ensure efficient scaling and performance across different parameter sizes and training stages.
Notably, Qwen2-VL~\cite{wang2024qwen2vl} processed a cumulative total of 1.4T tokens, while our InternVL2.5-78B is trained on just $\sim$120B tokens.
}
\label{tab:train_hyperparameter}
\end{table*}


==> table/v2pe.tex <==
\begin{table*}[t!]
\scriptsize
\centering
{\fontsize{8}{10}\selectfont 
\renewcommand{\arraystretch}{0.95}
\setlength\tabcolsep{2.6pt}
\begin{tabular}{c|lccccccccccccc}
\toprule
\multirow{2}{*}{V2PE}       & \multirow{2}{*}{\( \delta \)} & TextVQA        & VizWiz        & ChartQA       & DocVQA        & AI2D          & InfoVQA       & GQA           & SQA-I         & \multirow{2}{*}{POPE} & Tiny           & MMMU          & SEED v1       & \multirow{2}{*}{Overall} \\
                            &                               & val            & val           & test avg      & val           & test          & val           & test          & test          &                       & LVLM           & val           & image         &         \\

\midrule
\no               & --                            & 78.4           & 61.7          & 81.4          & 89.4          & 81.1          & 69.4          & 60.8          & 94.4          & 87.9                  & 348.5          & 52.6          & 75.6          & 75.2    \\
\midrule
\multirow{5}{*}{\yes} & 1/256                         & 78.0           & 61.7          & 81.2          & 88.5          & 81.0          & 67.7          & 61.0          & 94.4          & 88.3                  & 345.3          & 52.9          & 75.9          & 75.0    \\
                            & 1/64                          & 78.3           & 62.0          & 81.7          & 89.4          & 81.3          & 69.6          & 60.9          & 94.7          & 88.3                  & 345.7          & 52.3          & 76.1          & 75.3    \\
                            & 1/16                          & 78.7           & 62.1          & 81.7          & 90.4          & 81.6          & 70.4          & 61.1          & \textbf{95.0} & 88.2                  & 345.0          & \textbf{53.3} & 76.1          & 75.6    \\
                            & 1/4                           & \textbf{ 79.0} & \textbf{62.2} & \textbf{82.4} & \textbf{91.0} & \textbf{81.8} & \textbf{71.7} & \textbf{61.2} & 94.9          & 88.1                  & 345.8          & 52.6          & \textbf{76.2} & 75.9    \\
                            & 1/1                           & 78.7           & 61.7          & 82.2          & 90.2          & 81.7          & 71.4          & 61.2          & 94.6          & \textbf{ 88.5}        & \textbf{347.2} & 52.4          & 76.1          & 75.7    \\ 
\bottomrule
\end{tabular}}
\caption{\textbf{Performance of the pre-trained InternVL3-8B model on multimodal benchmarks with different positional encoding strategies.} When employing V2PE, the impact of different positional increment values \( \delta \) is systematically evaluated.
}
\label{v2pe_eff}
\end{table*}
